Berk-Nash Rationalizability

We introduce Berk--Nash rationalizability, a set-valued counterpart to Berk--Nash equilibrium for environments in which agents may hold misspecified models. A set of behaviors is self-justified if every behavior in the set is optimal under beliefs fitted to data generated within the set. Berk--Nash rationalizability is the largest self-justified set and reduces to standard rationalizability under correct specification and identification. We provide a learning foundation allowing Bayesian agents to learn from different, selectively sampled histories: almost surely, the limit set of play is self-justified. Conversely, under identification, any compact self-justified set can arise as the limit set with arbitrarily high probability. We illustrate how the concept yields informative predictions that are robust across learning procedures, without committing to a specific dynamic or assuming convergence.

==> other.tex <==
\section{Other}

\subsection{OLD. Positive support refinement}
A further refinement is useful in finite action spaces. Assume for the remainder of this subsection involving \(\Gamma^{CS+}\) that \(\mathbb A\) is finite. The refinement requires the action profile being justified to receive positive probability under the common sample distribution.

For \(S\subseteq\mathbb A\), define the \emph{positive-frequency common-sample} operator
\[
\Gamma^{CS+}(S)
:=
\left\{
a\in\mathbb A:
\exists\,\sigma\in\Delta S
\text{ s.t. }
\sigma(a)>0
\text{ and }
\forall i\in I,\ 
\exists\,\mu^i\in\Delta\Theta^{m,i}(\sigma)
\text{ with }
a^i\in F^i\bigl(\mu^i,\sigma^{-i}\bigr)
\right\}.
\]
A set \(S\subseteq\mathbb A\) is \emph{positive-frequency common-sample self-justified} if \(S\subseteq\Gamma^{CS+}(S)\). Let
\[
\mathcal S^{CS+}
:=
\{S\subseteq\mathbb A:S\subseteq\Gamma^{CS+}(S)\}
\]
denote the collection of positive-frequency common-sample self-justified sets. An action profile \(a\in\mathbb A\) is \emph{positive-frequency common-sample Berk--Nash rationalizable} if it belongs to some positive-frequency common-sample self-justified set. Equivalently,
\[
\mathcal B^{CS+}
:=
\bigcup_{S\in\mathcal S^{CS+}}S
\]
is the set of positive-frequency common-sample Berk--Nash rationalizable profiles.

This refinement is appropriate when one wants to justify not only actions that can occur infinitely often, but actions that can occur with nonvanishing frequency. The requirement \(\sigma(a)>0\) says that the same common sample distribution that justifies the players' beliefs and forecasts also assigns positive probability to the action profile being justified. Thus \(a\) is not merely compatible with the sample; it appears in the sample with positive probability.

Like \(\Gamma^{CS}\), the operator \(\Gamma^{CS+}\) need not be product-valued. The same distribution \(\sigma\) must jointly justify all players' components and must also assign positive probability to the profile \(a\) being justified.

The following result collects the inclusion relations among the baseline concept and the two refinements. All statements involving \(\Gamma^{CS+}\), \(\mathcal S^{CS+}\), and \(\mathcal B^{CS+}\) are understood under the finite-action restriction introduced above.

\begin{proposition}[Refinement hierarchy]\label{prop:refinement-hierarchy}
For every \(S\subseteq\mathbb A\),
\[
\Gamma^{CS+}(S)\subseteq\Gamma^{CS}(S)\subseteq\Gamma(S).
\]
Consequently,
\[
\mathcal S^{CS+}\subseteq\mathcal S^{CS}\subseteq\mathcal S
\qquad\text{and}\qquad
\mathcal B^{CS+}\subseteq\mathcal B^{CS}\subseteq\mathcal B.
\]
\end{proposition}
\begin{proof}
Fix \(S\subseteq\mathbb A\) and \(a\in\Gamma^{CS}(S)\). Then there exists a single \(\sigma\in\Delta S\) such that, for every player \(i\), there exists \(\mu^i\in\Delta\Theta^{m,i}(\sigma)\) with \(a^i\in F^i(\mu^i,\sigma^{-i})\). In the baseline definition, player \(i\) is allowed to use a player-specific selected sample \(\sigma^i\in\Delta S\). Taking \(\sigma^i=\sigma\) for every \(i\), the same witnesses show that \(a\in\Gamma(S)\). Hence \(\Gamma^{CS}(S)\subseteq\Gamma(S)\).

Now assume \(\mathbb A\) is finite and take \(a\in\Gamma^{CS+}(S)\). Then there exists \(\sigma\in\Delta S\) such that \(\sigma(a)>0\) and, for every player \(i\), there exists \(\mu^i\in\Delta\Theta^{m,i}(\sigma)\) with \(a^i\in F^i(\mu^i,\sigma^{-i})\). Dropping the additional requirement \(\sigma(a)>0\), the same witnesses show that \(a\in\Gamma^{CS}(S)\). Hence \(\Gamma^{CS+}(S)\subseteq\Gamma^{CS}(S)\).

If \(S\in\mathcal S^{CS+}\), then \(S\subseteq\Gamma^{CS+}(S)\subseteq\Gamma^{CS}(S)\), so \(S\in\mathcal S^{CS}\). Similarly, if \(S\in\mathcal S^{CS}\), then \(S\subseteq\Gamma^{CS}(S)\subseteq\Gamma(S)\), so \(S\in\mathcal S\). Thus \(\mathcal S^{CS+}\subseteq\mathcal S^{CS}\subseteq\mathcal S\). Taking unions over these collections gives \(\mathcal B^{CS+}\subseteq\mathcal B^{CS}\subseteq\mathcal B\).
\end{proof}

The inclusion \(\mathcal B^{CS}\subseteq\mathcal B\) can be strict in general because the baseline concept allows different players to justify their actions using different selected samples, while the common-sample concept requires a single sample distribution to justify all players' actions simultaneously. The following benchmark shows, however, that in correctly specified and identified two-player games, this additional restriction has no bite at the level of rationalizable profiles.

\begin{proposition}[Two-player correct-model benchmark]\label{prop:CS-two-player-equivalence}
Suppose the game is correctly specified and identified, and suppose \(|I|=2\). Then
\[
\mathcal B^{CS}=\mathcal B.
\]
\end{proposition}

\begin{proof}
By Proposition \ref{prop:refinement-hierarchy}, \(\mathcal B^{CS}\subseteq\mathcal B\). We prove the reverse inclusion.

Under correct specification and identification, each player's best-fitting model is the true model, independently of the sample distribution. Hence player \(i\)'s optimality condition depends only on the marginal distribution over her opponent's actions. Now let \(S=S^1\times S^2\) be a product set. We claim that \(\Gamma(S)\subseteq\Gamma^{CS}(S)\). Take \(a\in\Gamma(S)\). Then, for player \(1\), there is some selected sample \(\sigma^1\in\Delta S\) whose marginal on \(\mathbb A^2\), denoted \((\sigma^1)^2\), makes \(a^1\) optimal. Similarly, for player \(2\), there is some selected sample \(\sigma^2\in\Delta S\) whose marginal on \(\mathbb A^1\), denoted \((\sigma^2)^1\), makes \(a^2\) optimal. Since there are two players and \(S\) is a product set, the product distribution
\[
\bar\sigma:=(\sigma^2)^1\otimes(\sigma^1)^2
\]
belongs to \(\Delta S\). Its marginal over player \(2\)'s action is \((\sigma^1)^2\), and its marginal over player \(1\)'s action is \((\sigma^2)^1\). Therefore the same distribution \(\bar\sigma\) justifies both \(a^1\) and \(a^2\), so \(a\in\Gamma^{CS}(S)\).

As shown in Theorem \ref{theo:characterization}, \(\mathcal B\) is a product fixed point of \(\Gamma\). Applying the claim to \(S=\mathcal B\), we get
\[
\mathcal B=\Gamma(\mathcal B)\subseteq\Gamma^{CS}(\mathcal B).
\]
Thus \(\mathcal B\in\mathcal S^{CS}\), and therefore \(\mathcal B\subseteq\mathcal B^{CS}\). Combining this with \(\mathcal B^{CS}\subseteq\mathcal B\) gives \(\mathcal B^{CS}=\mathcal B\).
\end{proof}


\subsection{OLD. Common sample refinement}

The definition above allows each player \(i\) to justify her action using a player-specific selected sample \(\sigma^i\in\Delta S\). A stronger requirement is that all players' justifications be based on the same distribution over action profiles.

For \(S\subseteq\mathbb A\), define the \emph{common-sample} operator
\[
\Gamma^{CS}(S)
:=
\left\{
a\in\mathbb A:
\exists\,\sigma\in\Delta S
\text{ such that }
\forall i\in I,\ 
\exists\,\mu^i\in\Delta\Theta^{m,i}(\sigma)
\text{ with }
a^i\in F^i\bigl(\mu^i,\sigma^{-i}\bigr)
\right\}.
\]
A set \(S\subseteq\mathbb A\) is \emph{common-sample self-justified} if it is nonempty and compact, and $S\subseteq\Gamma^{CS}(S)$. Let
\[
\mathcal S^{CS}
:=
\{S\subseteq\mathbb A:S\text{ is nonempty and compact, and }S\subseteq\Gamma^{CS}(S)\}
\]
denote the collection of common-sample self-justified sets. An action profile \(a\in\mathbb A\) is \emph{common-sample Berk--Nash rationalizable} if it belongs to some common-sample self-justified set. Equivalently,
\[
\mathcal B^{CS}
:=
\bigcup_{S\in\mathcal S^{CS}}S
\]
is the set of common-sample Berk--Nash rationalizable profiles. As with \(\Gamma\), the compactness requirement does not affect the induced set of common-sample Berk--Nash rationalizable profiles. %If an arbitrary set \(S\subseteq\mathbb A\) satisfies \(S\subseteq\Gamma^{CS}(S)\), then its closure also satisfies \(\overline S\subseteq\Gamma^{CS}(\overline S)\). The argument is the same as before: \(\Gamma^{CS}\) is monotone, and the same compactness and closed-graph arguments used in Lemmas \ref{lem:basic-properties} and \ref{lem:Gamma-regular} imply that \(\Gamma^{CS}\) maps nonempty closed sets to nonempty closed sets.

The interpretation is that each profile \(a\) must be justified by a single sample distribution \(\sigma\) supported on \(S\). The same \(\sigma\) disciplines every player's belief about the best-fitting models and every player's forecast of opponents' behavior. Players may still have different subjective models and different limiting beliefs \(\mu^i\), but these beliefs and forecasts must be based on common evidence.

The common-sample rationalizable set admits the same existence and iterative characterization as \(\mathcal B\), except for the product-set conclusion. That is, the analogue of Theorem \ref{theo:characterization} holds for \(\Gamma^{CS}\): starting from \(C^0=\mathbb A\) and iterating \(C^{k+1}=\Gamma^{CS}(C^k)\), we obtain
\[
\mathcal B^{CS}=\bigcap_{k=0}^{\infty}C^k,
\]
and \(\mathcal B^{CS}\) is nonempty, compact, and the largest fixed point of \(\Gamma^{CS}\). Unlike \(\Gamma\), however, \(\Gamma^{CS}\) need not be product-valued. For each fixed \(\sigma\in\Delta S\), the profiles justified by \(\sigma\) form a product set. But \(\Gamma^{CS}(S)\) is the union of these product sets over all \(\sigma\in\Delta S\), and a union of product sets need not be a product set.


\begin{proposition}[Refinement hierarchy]\label{prop:refinement-hierarchy}
For every \(S\subseteq\mathbb A\), $\Gamma^{CS}(S)\subseteq\Gamma(S)$. Consequently,
$\mathcal S^{CS}\subseteq\mathcal S$ and $\mathcal B^{CS+}\subseteq\mathcal B^{CS}\subseteq\mathcal B$.
\end{proposition}
\begin{proof}
Fix \(S\subseteq\mathbb A\) and \(a\in\Gamma^{CS}(S)\). Then there exists a single \(\sigma\in\Delta S\) such that, for every player \(i\), there exists \(\mu^i\in\Delta\Theta^{m,i}(\sigma)\) with \(a^i\in F^i(\mu^i,\sigma^{-i})\). In the baseline definition, player \(i\) is allowed to use a player-specific selected sample \(\sigma^i\in\Delta S\). Taking \(\sigma^i=\sigma\) for every \(i\), the same witnesses show that \(a\in\Gamma(S)\). Hence \(\Gamma^{CS}(S)\subseteq\Gamma(S)\).

If \(S\in\mathcal S^{CS}\), then \(S\subseteq\Gamma^{CS}(S)\subseteq\Gamma(S)\), so \(S\in\mathcal S\). Thus \(\mathcal S^{CS}\subseteq\mathcal S\). Taking unions over these collections gives \(\mathcal B^{CS}\subseteq\mathcal B\).
\end{proof}

The inclusion \(\mathcal B^{CS}\subseteq\mathcal B\) can be strict in general because the baseline concept allows different players to justify their actions using different selected samples, while the common-sample concept requires a single sample distribution to justify all players' actions simultaneously. The following benchmark shows, however, that in correctly specified and identified two-player games, this additional restriction has no bite at the level of rationalizable profiles.

\begin{proposition}[Two-player correct-model benchmark]\label{prop:CS-two-player-equivalence}
Suppose the game is correctly specified and identified, and suppose \(|I|=2\). Then
\[
\mathcal B^{CS}=\mathcal B.
\]
\end{proposition}

\begin{proof}
By Proposition \ref{prop:refinement-hierarchy}, \(\mathcal B^{CS}\subseteq\mathcal B\). We prove the reverse inclusion.

Under correct specification and identification, each player's best-fitting model is the true model, independently of the sample distribution. Hence player \(i\)'s optimality condition depends only on the marginal distribution over her opponent's actions. Now let \(S=S^1\times S^2\) be a product set. We claim that \(\Gamma(S)\subseteq\Gamma^{CS}(S)\). Take \(a\in\Gamma(S)\). Then, for player \(1\), there is some selected sample \(\sigma^1\in\Delta S\) whose marginal on \(\mathbb A^2\), denoted \((\sigma^1)^2\), makes \(a^1\) optimal. Similarly, for player \(2\), there is some selected sample \(\sigma^2\in\Delta S\) whose marginal on \(\mathbb A^1\), denoted \((\sigma^2)^1\), makes \(a^2\) optimal. Since there are two players and \(S\) is a product set, the product distribution
\[
\bar\sigma:=(\sigma^2)^1\otimes(\sigma^1)^2
\]
belongs to \(\Delta S\). Its marginal over player \(2\)'s action is \((\sigma^1)^2\), and its marginal over player \(1\)'s action is \((\sigma^2)^1\). Therefore the same distribution \(\bar\sigma\) justifies both \(a^1\) and \(a^2\), so \(a\in\Gamma^{CS}(S)\).

As shown in Theorem \ref{theo:characterization}, \(\mathcal B\) is a product fixed point of \(\Gamma\). Applying the claim to \(S=\mathcal B\), we get
\[
\mathcal B=\Gamma(\mathcal B)\subseteq\Gamma^{CS}(\mathcal B).
\]
Thus \(\mathcal B\in\mathcal S^{CS}\), and therefore \(\mathcal B\subseteq\mathcal B^{CS}\). Combining this with \(\mathcal B^{CS}\subseteq\mathcal B\) gives \(\mathcal B^{CS}=\mathcal B\).
\end{proof}

\subsection{OLD A general learning environment}

We now describe a general class of stochastic processes underlying the learning results. Time is discrete, $t=1,2,\ldots$. Let $\mathbb Y=\times_{i\in I}\mathbb Y^i$, and let $Q(\cdot\mid a)\in\Delta\mathbb Y$ be a joint consequence kernel whose $i$th marginal is $Q^i(\cdot\mid a)$ for every player $i$. No independence across players' consequences is required.

Let
\[
\Omega=
\bigl(\mathbb A\times\{0,1\}^I\times\mathbb Y\bigr)^{\mathbb N}
\]
be the space of infinite histories, endowed with the product Borel $\sigma$-algebra $\mathcal F$. A realization is written
\[
\omega=(a_1,J_1,y_1,a_2,J_2,y_2,\ldots),
\]
where $J_t=(J_t^i)_{i\in I}\in\{0,1\}^I$ records which players retain the period-$t$ observation. After period $t$, the cumulative history is
\[
h_t=(a_1,J_1,y_1,\ldots,a_t,J_t,y_t).
\]

An action rule is an arbitrary sequence of measurable stochastic kernels
\[
\alpha_t(\cdot\mid h_{t-1})\in\Delta\mathbb A.
\]
Thus actions may depend arbitrarily on the entire past and may be randomized. At this stage, the action rule is unrestricted beyond measurability and non-anticipation; in particular, actions need not be functions of the selected sample or the posterior belief. Behavioral restrictions linking actions to beliefs and forecasts are imposed below.

After $a_t$ is chosen, but before $y_t$ is realized, the sampling decision $J_t$ is drawn according to an arbitrary measurable stochastic kernel
\[
\lambda_t(\cdot\mid h_{t-1},a_t)\in\Delta\{0,1\}^I.
\]
Selection may therefore depend on the entire past and on the current action profile, but not on the current consequence.

Conditional on $(h_{t-1},a_t,J_t)$, the consequence vector is drawn from $Q(\cdot\mid a_t)$. Hence the one-period transition kernel is
\[
\alpha_t(da_t\mid h_{t-1})
\lambda_t(dJ_t\mid h_{t-1},a_t)
Q(dy_t\mid a_t).
\]
These kernels induce a unique probability measure $\mathbf P$ on
$(\Omega,\mathcal F)$. In particular, for every player $i$ and every Borel set $B\subseteq\mathbb Y^i$,
\[
\mathbf P(y_t^i\in B\mid h_{t-1},a_t,J_t)
=
Q^i(B\mid a_t).
\]

For each player $i$, the selected sample available at date $t$ is
\[
H_t^i=\{\tau<t:J_\tau^i=1\}.
\]
Selection is permanent: once $J_\tau^i$ is realized, observation $\tau$ either belongs to every subsequent sample or to none of them. We assume
\[
|H_t^i|\to\infty
\qquad \mathbf P\text{-a.s.}
\]
for every player $i$. The selected sample induces the empirical distribution
\[
\hat\sigma_t^i
=
\frac{1}{|H_t^i|}
\sum_{\tau\in H_t^i}\delta_{a_\tau},
\]
whenever $H_t^i\neq\varnothing$. The full-history case corresponds to
$J_\tau^i=1$ for every $i$ and $\tau$.

Player $i$ starts from a full-support prior
$\mu_0^i\in\Delta\Theta^i$ and updates using only the selected observations. Thus, for every Borel set $B\subseteq\Theta^i$,
\[
\mu_t^i(B)
=
\frac{
\int_B
\prod_{\tau\in H_t^i}
q_\theta^i(y_\tau^i\mid a_\tau)
\,\mu_0^i(d\theta)
}{
\int_{\Theta^i}
\prod_{\tau\in H_t^i}
q_\theta^i(y_\tau^i\mid a_\tau)
\,\mu_0^i(d\theta)
},
\]
with $\mu_t^i=\mu_0^i$ when $H_t^i=\varnothing$.

We call any process satisfying the preceding timing, sampling, persistence, and Bayesian-updating conditions an \emph{admissible learning process}.

\begin{lemma}[Asymptotic beliefs]\label{lemm:Berk-selected}
For every admissible learning process, with $\mathbf P$-probability one, the following holds simultaneously for every player $i$. If, along some subsequence $(t_k)_k$, $\hat\sigma_{t_k}^i\Rightarrow\sigma^i\in\Delta\mathbb A$, then for every closed set $E\subseteq\Theta^i$ with $E\cap\Theta^{m,i}(\sigma^i)=\varnothing$, there exist constants $C>0$, $\rho>0$, and an integer $K$ such that
\begin{equation}\label{eq:exponential}
\mu_{t_k}^i(E)
\leq
C\exp\{-\rho |H_{t_k}^i|\}.
\end{equation}
for all $k\geq K$. In particular, if also $\mu_{t_k}^i\Rightarrow\mu^i$, then $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$.
\end{lemma}

\begin{proof}
See the Supplemental Appendix.
\end{proof}

Lemma~\ref{lemm:Berk-selected} says that along any subsequence for which player $i$'s selected empirical distribution converges, posterior probability assigned to any closed set of models separated from the best-fitting models for the limiting selected data vanishes exponentially fast.\footnote{The exponential rate is not needed for the sequel.} Consequently, every limiting posterior belief is supported on $\Theta^{m,i}(\sigma^i)$. The result builds on \citet{berk1966limiting}'s analysis of misspecified Bayesian learning and its extensions to endogenous data, including \citet{esponda2016berk} and \citet{esponda2021asymptotic}. Relative to those results, the lemma allows inference to be based on a selected subsequence of realized observations and allows for a compact action space.

Importantly, Lemma~\ref{lemm:Berk-selected} places no optimality restriction on the action rule. Actions may be generated by any history-dependent and randomized procedure. The action and sampling rules matter because, together with the true consequence kernels, they determine the probability measure $\mathbf P$ and the selected empirical distributions $\hat\sigma_t^i$. The key statistical restriction is non-anticipation: the current action and the decision whether to retain its observation are determined before the corresponding consequence is realized. Under this restriction, selected log-likelihood contributions retain a martingale-difference structure under the joint probability law, so the required uniform strong law can be established directly. Thus the result is portable across action rules: once an action-and-sampling process satisfies the above timing and persistence conditions, posterior concentration is governed by the limiting empirical distribution of the selected actions. The Supplemental Appendix provides the details.\footnote{Our persistent-sampling restriction is convenient for the martingale strong-law argument. More general, non-monotone stochastic sampling schemes can also be analyzed under additional structure; for example, \cite{fudenberg2024selective} use conditional concentration and Borel--Cantelli arguments to study selective-memory rules in which the recalled sample can change across dates.}

\subsection{OLD Sustaining Self-Justified Sets}

We next establish a partial converse to the limit-result above. While the previous subsection showed that long-run behavior under a specfic form of learning must be self-justified, the result below shows that, under identification, every compact self-justified set can be sustained as the long-run range of behavior by a suitable learning process with asymptotically optimal behavior.


Throughout this subsection,
assume that the game is identified: for every player \(i\) and every
\(\sigma\in\Delta\mathbb A\), the set \(\Theta^{m,i}(\sigma)\) is a singleton.
We write its unique element as
\[
\theta^i(\sigma),
\qquad
\Theta^{m,i}(\sigma)=\{\theta^i(\sigma)\}.
\]

For \(\varepsilon\geq 0\), define the \(\varepsilon\)-optimal action
correspondence
\[
F^i_\varepsilon(\mu^i,\beta^{-i})
:=
\left\{
a^i\in\mathbb A^i:
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\beta^{-i},\theta^i)\,\mu^i(d\theta^i)
-
\int_{\Theta^i}U^i(a^i,\beta^{-i},\theta^i)\,\mu^i(d\theta^i)
\leq \varepsilon
\right\}.
\]
Thus \(F^i_0=F^i\).

A \emph{learning rule} specifies, for each player \(i\), a full-support prior
\(\mu_0^i\), a selected-sample rule
\[
H_t^i(a_1,\ldots,a_{t-1})\subseteq\{1,\ldots,t-1\},
\]
a posterior \(\mu_t^i\) obtained by Bayesian updating from the selected sample,
the empirical forecast
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i},
\]
and an action rule \(g_t^i\) that maps player \(i\)'s date-\(t\) information into
an action \(a_t^i\).

A learning rule is \emph{asymptotically optimal} if there exists a deterministic
sequence \(\varepsilon_t\downarrow0\) such that, for every date \(t\), every
player \(i\), and every history at which the rule is evaluated,
\[
g_t^i\in F^i_{\varepsilon_t}(\mu_t^i,\tilde\sigma_t^{-i}).
\]
Thus asymptotic optimality is a restriction on the rule itself, not merely a
property verified ex post along the realized path.

\begin{theorem}[Sustaining self-justified sets]\label{theo:sustain-self-justified}
Suppose the game is identified. Let \(S\subseteq\mathbb A\) be a nonempty compact
self-justified set. Then, for every \(\alpha>0\), there exist a learning rule and
a deterministic sequence \(\varepsilon_t\downarrow0\) such that:

\begin{enumerate}
\item the learning rule is asymptotically optimal with tolerance
\((\varepsilon_t)_t\);

\item the action process generated by the rule satisfies
\[
\mathbf P\bigl(L(a^\infty)=S\bigr)>1-\alpha.
\]
\end{enumerate}
\end{theorem}
\begin{proof}
See the Appendix.
\end{proof}

The result follows the logic of \cite{fudenberg1993learning}'s learning foundation for Nash equilibrium. Their key insight is that any Nash equilibrium can be sustained by behavior that is not exactly optimal after every finite history, but is asymptotically optimal. \cite{esponda2016berk} extend this argument to Berk--Nash equilibrium, allowing for misspecified models. Theorem \ref{theo:sustain-self-justified} uses the same basic learning mechanism, but changes the object being sustained. Instead of sustaining a singleton steady state, the target is a compact set \(S\) of possible long-run actions. The proof therefore constructs a path whose limit set is \(S\), and specifies selected histories so that different dates and players can use different samples from that same long-run range.

The compactness restriction comes from the conclusion of the theorem. Since \(\mathbb A\) is compact, the set of limit points of any action path is nonempty and compact. Thus only compact sets can literally be sustained as \(L(a^\infty)\). This restriction does not affect the set of Berk--Nash rationalizable profiles: if a profile belongs to some self-justified set \(S\), then it also belongs to the compact self-justified set \(\overline S\), the closure of \(S\).\footnote{By monotonicity, \(S\subseteq\overline S\) implies \(\Gamma(S)\subseteq\Gamma(\overline S)\). Thus, if \(S\subseteq\Gamma(S)\), then \(S\subseteq\Gamma(\overline S)\). Since \(\Gamma(\overline S)\) is closed, it contains \(\overline S\).}

The idea of the proof is as follows. Since \(S\) is self-justified, each profile \(a\in S\) can be justified by some selected sample drawn from \(S\). The construction therefore chooses a target path whose limit set is \(S\), and specifies sampling rules so that, when the target path calls for action profile \(a\), each player selects past observations whose empirical distribution is close to one that justifies her component \(a^i\). In this way, different parts of the long-run range \(S\) may be supported by different selected samples from the same range.

Identification is used to ensure that selected samples determine limiting beliefs. If the selected empirical distribution is close to \(\sigma\), Bayesian learning drives beliefs close to the unique best-fitting model \(\theta^i(\sigma)\). Without identification, beliefs may fail to converge, or may converge to a belief that does not justify the prescribed action.

Finally, the action rule follows the target path whenever the prescribed action is \(\varepsilon_t\)-optimal, and otherwise plays an exact best response. The sequence \(\varepsilon_t\downarrow0\) is chosen slowly enough that, with probability arbitrarily close to one, the prescribed action is \(\varepsilon_t\)-optimal at every date along the target path. On this event, the realized path coincides with the target path, so its set of limit points is exactly \(S\).

The construction has a selected-history interpretation. The path generates a compact long-run range \(S\), but beliefs at a given date are based on a selected or weighted sample from that range rather than on the full empirical history. Different dates, or different players, may use different samples, so different actions in \(S\) can be supported by different empirical distributions over the same long-run range. This is natural in a repeated-population interpretation, where later generations inherit data from earlier play but need not use all of it.

The result should not be read as selecting which self-justified set will arise in a particular learning environment. That selection may depend on the learning rule, the sampling procedure, initial conditions, and early consequence realizations. The theorem is instead a possibility result: under identification, no compact self-justified set is ruled out on learning grounds alone. With appropriate selected-sample learning and asymptotically optimal behavior, any such set can arise as the long-run range with probability arbitrarily close to one.

XXXXXXX  OLD XXXXXXX

\subsection{OLD Limit Behavior under Learning}

We now describe a class of learning dynamics whose long-run behavior is captured by self-justification and Berk--Nash rationalizability. Time is discrete, \(t=1,2,\ldots\). At each date \(t\), players choose an action profile \(a_t\in\mathbb A\). Consequences are then drawn according to the true kernels: for each player \(i\), \(y_t^i\sim Q^i(\cdot\mid a_t)\). Action profiles are publicly observed, and player \(i\) observes her own realized consequence \(y_t^i\).

Each player \(i\) starts with a full-support prior \(\mu_0^i\in\Delta\Theta^i\). At date \(t\), player \(i\) selects a set of past periods
\[
H_t^i\subseteq\{1,\ldots,t-1\}.
\]
We impose a non-anticipatory and persistent sampling rule. For each player \(i\) and period \(\tau\), after the action \(a_\tau\) is determined but without using the realized consequence \(y_\tau^i\), the player determines whether observation \(\tau\) will be included in her selected sample. This decision may depend on the action history \(a_1,\ldots,a_\tau\) and on exogenous randomization independent of consequence shocks, but not on \(y_\tau^i\) or on any later endogenous variable that may contain information about \(y_\tau^i\). Let \(I_\tau^i\in\{0,1\}\) denote this selection decision.

The selected sample available at date \(t\) is therefore
\[
H_t^i=\{\tau<t:I_\tau^i=1\}.
\]
Thus selection is made once for each observation: if \(I_\tau^i=1\), observation \(\tau\) is retained in all subsequent samples, while if \(I_\tau^i=0\), it is never used. We assume moreover that
\[
|H_t^i|\to\infty
\]
along every infinite action path, so that each player eventually accumulates arbitrarily many selected observations.\footnote{\cite{fudenberg2024selective} also studies permanent retention as a special case, but allows recall probabilities to depend on realized outcomes in order to model memory bias. We instead require selection to be independent of consequences, so that selection changes which observations are used without distorting the conditional outcome distribution given actions.}


%\footnote{The restriction that \(H_t^i\) is determined by the action history rules out selection rules that condition directly on realized consequence shocks. Such rules could generate biased selected samples; for example, a player could select only periods in which a given action happened to generate unusually favorable outcomes. The asymptotic-belief lemma below requires that, conditional on the selected action profiles, the selected consequences are generated according to the true kernels.}

The selected sample induces player \(i\)'s empirical distribution over action profiles,
\[
\hat\sigma_t^i
=
\frac{1}{|H_t^i|}
\sum_{\tau\in H_t^i}\delta_{a_\tau},
\]
for all \(t\) such that \(H_t^i\neq\varnothing\). The superscript \(i\) indicates that this distribution is player-specific: different players may select different subsets of past periods and therefore may base their learning on different empirical distributions. The benchmark full-history case is
\[
H_t^i=\{1,\ldots,t-1\}
\quad\text{for every }i,
\]
in which case \(\hat\sigma_t^i\) is the same for all players and coincides with the usual empirical distribution of past play.

Player \(i\)'s posterior at date \(t\) is the Bayesian posterior obtained from her prior and the selected observations \(\{(a_\tau,y_\tau^i):\tau\in H_t^i\}\). Thus, for every Borel set \(B\subseteq\Theta^i\),
\[
\mu_t^i(B)
=
\frac{
\int_B
\prod_{\tau\in H_t^i}
q_\theta^i(y_\tau^i\mid a_\tau)
\,\mu_0^i(d\theta)
}{
\int_{\Theta^i}
\prod_{\tau\in H_t^i}
q_\theta^i(y_\tau^i\mid a_\tau)
\,\mu_0^i(d\theta)
},
\]
whenever \(H_t^i\neq\varnothing\); for finite initial dates with \(H_t^i=\varnothing\), let \(\mu_t^i=\mu_0^i\).

Player \(i\) also forms a forecast
\[
\tilde\sigma_t^{-i}\in\Delta\mathbb A^{-i}
\]
over opponents' actions. For any distribution \(\sigma\in\Delta\mathbb A\), let \(\sigma^{-i}\in\Delta\mathbb A^{-i}\) denote its marginal on opponents' action profiles. Thus, if \(\sigma^i\in\Delta\mathbb A\) is a distribution over full action profiles associated with player \(i\)'s selected sample, then \((\sigma^i)^{-i}\) denotes its marginal over opponents' actions. We require forecasts to be asymptotically consistent with the selected sample in the following sense: for every realized action path, every player \(i\), and every subsequence \((t_k)_k\),
\begin{equation}\label{eq:forecast-consistency}
\hat\sigma_{t_k}^i\Rightarrow\sigma^i
\quad\Longrightarrow\quad
\tilde\sigma_{t_k}^{-i}\Rightarrow(\sigma^i)^{-i}.
\end{equation}
In words, whenever player \(i\)'s selected empirical distribution over full action profiles converges along a subsequence, her forecast of opponents' behavior must converge to the opponents' marginal of that same limiting distribution.

The simplest example is the empirical forecast
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i},
\]
where player \(i\) forecasts opponents' behavior using the marginal empirical distribution from her own selected sample. This forecast satisfies condition \eqref{eq:forecast-consistency} immediately.\footnote{Condition \eqref{eq:forecast-consistency} also allows finite-date smoothing and initial conditions, provided their effect vanishes asymptotically. For example, forecasts may mix the selected empirical marginal with an initial full-support forecast using a weight that converges to zero. Weighted samples can be handled similarly by replacing selected sets with sampling weights and imposing the usual no-dominant-observation condition. Finally, the separated presentation of model learning and forecasts is also a reduced form for a joint Bayesian model over consequences and opponents' play when the distribution of opponents' play is governed by flexible nuisance parameters that are variation independent of \(\theta^i\). If the subjective model imposes cross-restrictions between \(\theta^i\) and the feasible distributions of opponents' actions, the relevant limiting object would instead involve a joint KL problem.}

For \(\varepsilon\geq 0\), define the \(\varepsilon\)-optimal action correspondence
\[
F^i_\varepsilon(\mu^i,\beta^{-i})
:=
\left\{
a^i\in\mathbb A^i:
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\beta^{-i},\theta^i)\,\mu^i(d\theta^i)
-
\int_{\Theta^i}U^i(a^i,\beta^{-i},\theta^i)\,\mu^i(d\theta^i)
\leq \varepsilon
\right\}.
\]
Thus \(F^i_0=F^i\).
At date \(t\), player \(i\) chooses an asymptotically myopic action. That is, there exists a deterministic sequence \(\varepsilon_t\downarrow0\) such that, for every date \(t\), every player \(i\), and every history at which the rule is evaluated,
\[
a_t^i\in F_{\varepsilon_t}^i(\mu_t^i,\tilde\sigma_t^{-i}).
\]
A learning environment satisfying these conditions is called a \emph{game with Bayesian players, selected samples, consistent forecasts, and asymptotically myopic behavior}.



The formulation is intentionally permissive, and several further extensions could be incorporated without changing the logic of the result. Exact best responses are not required; it is enough that payoff losses vanish asymptotically. Nor does the result depend on a particular adjustment process, such as fictitious play or best-response dynamics, or on players using the full history. We present the model using selected subsets of past observations for simplicity, but the same argument could allow weighted samples, provided the effective sample size grows and no single observation has asymptotically dominant weight; random sample-selection rules, provided selection of each observation is based only on information available before its consequence is realized and on exogenous randomization independent of consequence shocks; and smoothed forecasts or finite-date prior adjustments, provided their effect vanishes asymptotically. The key restrictions are that selected samples grow large, forecasts are asymptotically consistent with those samples, and sample selection is non-anticipatory with respect to consequence realizations. This last restriction prevents selection from favoring observations with unusually favorable or unfavorable consequences, whether directly or indirectly through later endogenous behavior, which would generally distort the conditional distribution of selected consequences away from the true kernels.

The Bayesian-updating assumption determines the particular notion of model fit used in the solution concept. Given the subjective likelihoods, Bayesian updating under misspecification leads asymptotically to models that minimize the KL divergence from the data-generating process. Other updating rules could be studied in the same spirit, but the definition of the best-fitting-model correspondence would have to be modified accordingly.


\paragraph{Probability space.}
Let \(\mathbb Y=\times_{i\in I}\mathbb Y^i\). The data-generating process, the selected-sample rules, the forecasting rules, the players' action rules, and any exogenous randomization used by these rules are defined on an underlying probability space \((\Omega,\mathcal F,\mathbf P)\). They generate stochastic processes \((a_t,y_t)_{t\geq1}\), together with the selected samples \(H_t^i\), posterior beliefs \(\mu_t^i\), and forecasts \(\tilde\sigma_t^{-i}\).

The following lemma characterizes asymptotic posterior beliefs along convergent subsequences of selected empirical distributions.

\begin{lemma}[Asymptotic beliefs]\label{lemm:Berk-selected}
With $\mathbf P$-probability one, the following holds simultaneously for every player $i$. Suppose that, for some subsequence $(t_k)_k$,
\[
\hat\sigma_{t_k}^i\Rightarrow\sigma^i\in\Delta\mathbb A.
\]
Then, for every closed set $E\subseteq\Theta^i$ such that
\[
E\cap\Theta^{m,i}(\sigma^i)=\varnothing,
\]
there exist constants $C>0$, $\rho>0$, and an integer $K$ such that, for all $k\geq K$,
\begin{equation}\label{eq:exponential}
\mu_{t_k}^i(E)
\leq
C\exp\{-\rho |H_{t_k}^i|\}.
\end{equation}
In particular, if
\[
\mu_{t_k}^i\Rightarrow\mu^i,
\]
then
\[
\mu^i\in\Delta\Theta^{m,i}(\sigma^i).
\]
\end{lemma}
\begin{proof}
See the Supplemental Appendix.
\end{proof}

Lemma \ref{lemm:Berk-selected} says that along any subsequence for which player \(i\)'s selected empirical distribution converges, posterior probability assigned to any closed set of models that is separated from the best-fitting models for the limiting selected data vanishes exponentially fast.\footnote{The exponential rate is not needed for the sequel.} Consequently, every limiting posterior belief is supported on \(\Theta^{m,i}(\sigma^i)\). The result builds on \citet{berk1966limiting}'s analysis of misspecified Bayesian learning and its extensions to endogenous data, including \citet{esponda2016berk} and \citet{esponda2021asymptotic}. Relative to those results, the lemma allows the data used for inference to be a selected subsequence of the realized observations and allows for a compact action space. Under our non-anticipatory persistent-sampling assumption, the selected likelihood contributions retain a martingale-difference structure, so the required uniform strong law can be established directly under the joint probability law. The Supplemental Appendix provides the details.\footnote{Our persistent-sampling restriction is convenient for the martingale strong-law argument. More general, non-monotone stochastic sampling schemes can also be analyzed under additional structure; for example, \cite{fudenberg2024selective} use conditional concentration and Borel--Cantelli arguments to study selective-memory rules in which the recalled sample can change across dates.}


Let \(L(a^\infty)\) denote the set of limit action profiles of the realized action path \(a^\infty\). That is,
\[
L(a^\infty)
=
\left\{
a\in\mathbb A:
\exists\, t_k\to\infty
\text{ such that }
a_{t_k}\to a
\right\}.
\]
When \(\mathbb A\) is finite, \(a\in L(a^\infty)\) if and only if \(a\) is played infinitely often along the path. 

The next lemma records a purely topological property of limit sets. It does not use the learning assumptions introduced above; it follows only from compactness of the action space. This is the reason self-justified sets were defined in the previous section to be compact: if such sets are meant to represent long-run ranges of behavior, they should have the same basic topological property as the limit set of an action path.

\begin{lemma}\label{lem:limit-set-compact}
For every action path \(a^\infty\in\mathbb A^{\mathbb N}\), the set \(L(a^\infty)\) is nonempty and compact.
\end{lemma}

\begin{proof}
For each \(T\geq1\), let
\[
K_T:=\overline{\{a_t:t\geq T\}}.
\]
Since \(\mathbb A\) is compact, each \(K_T\) is nonempty and compact. Moreover, the sequence \((K_T)_T\) is decreasing. Hence \(\bigcap_{T=1}^{\infty}K_T\) is nonempty and compact. This intersection is exactly \(L(a^\infty)\): a point belongs to every tail closure if and only if it is the limit of a subsequence of the path. Therefore \(L(a^\infty)\) is nonempty and compact.
\end{proof}

The next result shows that the learning environment just described generates only self-justified long-run behavior.

\begin{theorem}[Limit behavior is self-justified]\label{theo:limit-self-justified}
Consider a game with Bayesian players, selected samples, consistent forecasts, and asymptotically myopic behavior. With probability one, \(L(a^\infty)\) is self-justified; that is, \(L(a^\infty)\) is nonempty and compact, and $L(a^\infty)\subseteq \Gamma\bigl(L(a^\infty)\bigr)$. Consequently, every limit action profile is Berk--Nash rationalizable.
\end{theorem}

\begin{proof}
Fix a realization in the $\mathbf P$-probability-one event on which Lemma \ref{lemm:Berk-selected} holds simultaneously for every player. Let \(L=L(a^\infty)\). By Lemma \ref{lem:limit-set-compact}, \(L\) is nonempty and compact. Pick any \(a\in L\). Then there exists a subsequence \((t_k)_k\) such that $a_{t_k}\to a$. By compactness, passing to a further subsequence if necessary, for every player \(i\),
\[
\hat\sigma_{t_k}^i\Rightarrow\sigma^i\in\Delta\mathbb A,
\qquad
\mu_{t_k}^i\Rightarrow\mu^i\in\Delta\Theta^i.
\]

We first show that each \(\sigma^i\) is supported on \(L\). If \(x\notin L\), then there is an open neighborhood \(U\) of \(x\) that is visited only finitely many times by the action path. Since \(|H_t^i|\to\infty\), $\hat\sigma_t^i(U)\to0$. Therefore any weak limit of \((\hat\sigma_t^i)_t\) assigns probability zero to such a neighborhood \(U\). Hence \(\operatorname{supp}(\sigma^i)\subseteq L\) for every $i$. By Lemma \ref{lemm:Berk-selected}, $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$ for every $i$.

By forecast consistency, condition \eqref{eq:forecast-consistency}, \(\tilde\sigma_{t_k}^{-i}\Rightarrow(\sigma^i)^{-i}\) for every \(i\). Since \(a_{t_k}^i\in F^i_{\varepsilon_{t_k}}(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})\), \(\varepsilon_{t_k}\to0\), and the correspondence \((\varepsilon,\mu^i,\beta^{-i})\mapsto F^i_\varepsilon(\mu^i,\beta^{-i})\) has a closed graph (see Lemma \ref{lem:basic-properties}(ii) in the Appendix), it follows that \(a^i\in F^i(\mu^i,(\sigma^i)^{-i})\) for every \(i\).

Thus, for each player \(i\), there exists \(\sigma^i\in\Delta L\) and \(\mu^i\in\Delta\Theta^{m,i}(\sigma^i)\) such that $a^i\in F^i(\mu^i,(\sigma^i)^{-i})$. By the definition of \(\Gamma\), \(a\in\Gamma(L)\). Since \(a\in L\) was arbitrary, \(L\subseteq\Gamma(L)\). Since \(L\) is nonempty and compact, \(L\in\mathcal S\), and hence every \(a\in L\) belongs to \(\mathcal B=\bigcup_{S\in\mathcal S}S\). Thus every limit action profile is Berk--Nash rationalizable.
\end{proof}


The intuition is as follows. Take any action profile \(a\) that is a limit point of play. Along a subsequence with \(a_t\to a\), each player's selected empirical distribution has a further subsequential limit \(\sigma^i\). Because selected observations are drawn from the realized path, any such limiting selected sample is supported on the set \(L(a^\infty)\) of limit action profiles. The asymptotic-belief lemma implies that player \(i\)'s limiting posterior is supported on the models that best fit \(\sigma^i\), and forecast consistency implies that the limiting forecast is \((\sigma^i)^{-i}\). Since actions are asymptotically optimal and \(\varepsilon_t\to0\), the closed-graph property of the correspondence \((\varepsilon,\mu^i,\sigma^{-i})\mapsto F^i_\varepsilon(\mu^i,\sigma^{-i})\) implies that the limiting action \(a^i\) is exactly optimal under this limiting belief and forecast. Thus each component of \(a\) is justified by a selected sample drawn from \(L(a^\infty)\), which gives the inclusion \(L(a^\infty)\subseteq\Gamma(L(a^\infty))\). Together with compactness of \(L(a^\infty)\), this means that the limit set is self-justified.

\paragraph{Learning foundation for the common-sample refinement.}
The learning foundation above mirrors the original solution concept: different players may base their posteriors and forecasts on different selected samples from the realized history. This is why a limit profile may be justified by player-specific sample distributions \(\sigma^i\). The common-sample refinement introduced earlier imposes a stronger requirement: the components of a profile must be justified using a single distribution over action profiles. We now show that this refinement has the corresponding learning foundation when players draw on the same selected sample from the history.

Under the non-anticipatory persistent-sampling rule imposed above, suppose further that the selection decision is common across players: for every period \(\tau\), $I_\tau^i=I_\tau$ for every $i\in I$. Hence the selected sample is common, $H_t^i=H_t$ for every $i\in I$. Write
\[
\hat\sigma_t=\frac{1}{|H_t|}\sum_{\tau\in H_t}\delta_{a_\tau}
\]
for the common selected empirical distribution. Suppose also that forecasts are consistent with this common sample: whenever \(\hat\sigma_{t_k}\Rightarrow\sigma\), we have
\begin{equation} \label{commonconsistency}
\tilde\sigma_{t_k}^{-i}\Rightarrow\sigma^{-i}
\qquad\text{for every }i\in I.
\end{equation}

\begin{theorem}[Learning foundation for common-sample self-justification]\label{theo:common-sample-foundation}
Consider a game with Bayesian players, common selected samples, forecasts consistent with the common sample, and asymptotically myopic behavior. With probability one, With probability one, \(L(a^\infty)\) is common-sample self-justified; that is, \(L(a^\infty)\) is nonempty and compact, and $L(a^\infty)\subseteq \Gamma^{CS}\bigl(L(a^\infty)\bigr)$. Consequently, every limit action profile is common-sample Berk--Nash rationalizable.
\end{theorem}
\begin{proof}
The proof is identical to that of Theorem \ref{theo:limit-self-justified}, except that the common selected sample yields a single subsequential limit \(\sigma\in\Delta L(a^\infty)\) for all players, rather than player-specific limits \(\sigma^i\). Hence the same \(\sigma\) justifies every component of the limit profile, which gives \(L(a^\infty)\subseteq\Gamma^{CS}(L(a^\infty))\).
\end{proof}

%The proof is a straightforward modification of the proof of Theorem \ref{theo:limit-self-justified}. The only substantive change is that, under common selected samples, the subsequential selected-sample limit is the same for all players. Thus, along a subsequence with \(a_t\to a\), we obtain a single distribution \(\sigma\in\Delta L(a^\infty)\), rather than player-specific distributions \(\sigma^i\). Lemma \ref{lemm:Berk-selected} then implies that each player's limiting belief is supported on the models that best fit this same \(\sigma\), and forecast consistency gives the limiting forecast \(\sigma^{-i}\). Since actions are asymptotically optimal and \(\varepsilon_t\to0\), the closed-graph property of the correspondence \((\varepsilon,\mu^i,\beta^{-i})\mapsto F^i_\varepsilon(\mu^i,\beta^{-i})\) implies that \(a^i\) is optimal under this limiting belief and forecast for every player \(i\). Therefore the same sample distribution \(\sigma\) justifies all components of \(a\), which is exactly the defining requirement of \(\Gamma^{CS}\).


\paragraph{OUT, SUPPLEMENTAL APPENDIX FOR FINITE GAMES XXX Learning foundation for the positive-frequency common-sample refinement.}
We now give a learning foundation for the positive-frequency common-sample refinement. This refinement is most transparent when \(\mathbb A\) is finite, because then positive frequency has a direct meaning: a profile is played with positive empirical frequency along some arbitrarily late histories. To obtain this foundation, we impose a stronger sampling requirement than in Theorem \ref{theo:common-sample-foundation}: players do not merely use a common selected sample, but the full public history.

Assume that \(\mathbb A\) is finite. Suppose that players use the full public history as their common sample: for every player \(i\) and every date \(t\ge 2\),
\[
H_t^i=\{1,\ldots,t-1\}.
\]
Thus the common selected empirical distribution is
\[
\hat\sigma_t=\frac{1}{t-1}\sum_{\tau<t}\delta_{a_\tau}.
\]
Suppose also that forecasts are consistent with this common sample, in the sense of condition \eqref{commonconsistency}.
Define the positive-frequency limit set by
\[
L^+(a^\infty)
=
\left\{
a\in\mathbb A:
\limsup_{t\to\infty}\hat\sigma_t(a)>0
\right\}.
\]
Thus \(L^+(a^\infty)\) is the set of profiles whose accumulated empirical frequency is bounded away from zero along arbitrarily late histories. These profiles need not have a limiting frequency, and their frequency need not stay bounded away from zero at all late dates; they need only be statistically visible along some subsequence of histories.

\begin{theorem}[Learning foundation for positive-frequency common-sample self-justification]\label{theo:positive-frequency-common-sample-foundation}
Consider a finite game with Bayesian players, full public-history common samples, and forecasts consistent with the common sample. With probability one,
\[
L^+(a^\infty)
\subseteq
\Gamma^{CS+}\bigl(L^+(a^\infty)\bigr).
\]
Consequently, every action profile played with positive limsup frequency is positive-frequency common-sample Berk--Nash rationalizable.
\end{theorem}

\begin{proof}
Work on the probability-one event used in the proof of Theorem \ref{theo:common-sample-foundation}. Let \(L^+=L^+(a^\infty)\), and fix \(a\in L^+\). By definition of \(L^+\), there exist \(\eta>0\) and dates \(n_k\to\infty\) such that \(\hat\sigma_{n_k}(a)>\eta\) for every \(k\). For each \(k\), let \(t_k<n_k\) be the last date before \(n_k\) at which \(a\) is played. Then \(a_{t_k}=a\), and \(t_k\to\infty\). Write \(M_t(a)=\sum_{\tau<t}\mathbf 1\{a_\tau=a\}\), so that \(\hat\sigma_t(a)=M_t(a)/(t-1)\). Since \(t_k\) is the last date before \(n_k\) at which \(a\) is played, \(M_{n_k}(a)=M_{t_k}(a)+1\). Hence \(M_{t_k}(a)=M_{n_k}(a)-1>\eta(n_k-1)-1\). Since \(t_k<n_k\), it follows that, for all sufficiently large \(k\), \(\hat\sigma_{t_k}(a)=M_{t_k}(a)/(t_k-1)>\eta/2\).

Passing to a further subsequence if necessary, compactness of the finite simplex and of the belief spaces implies that \(\hat\sigma_{t_k}\to\sigma\) for some \(\sigma\in\Delta\mathbb A\), and \(\mu_{t_k}^i\Rightarrow\mu^i\in\Delta\Theta^i\) for every \(i\in I\). Since \(\hat\sigma_{t_k}(a)>\eta/2\) along this subsequence, \(\sigma(a)>0\). We next show that \(\sigma\in\Delta L^+\). If \(b\in\mathbb A\) and \(\sigma(b)>0\), then \(\hat\sigma_{t_k}(b)\to\sigma(b)>0\), so \(\limsup_t\hat\sigma_t(b)>0\), and therefore \(b\in L^+\). Thus \(\sigma\) assigns probability only to profiles in \(L^+\), so \(\sigma\in\Delta L^+\).

Now apply the same learning argument as in Theorem \ref{theo:common-sample-foundation}. Since players use the full public history, the selected empirical distribution is common and converges along the chosen subsequence to \(\sigma\). By Lemma \ref{lemm:Berk-selected}, \(\mu^i\in\Delta\Theta^{m,i}(\sigma)\) for every \(i\in I\). By forecast consistency, condition \eqref{commonconsistency}, \(\tilde\sigma_{t_k}^{-i}\Rightarrow\sigma^{-i}\) for every \(i\in I\). Since \(a_{t_k}=a\), we have \(a_{t_k}^i=a^i\) for every \(i\) and every \(k\). The optimality condition gives \(a^i\in F^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})\) for every \(i\in I\) and every \(k\). Since \(F^i\) has a closed graph, it follows that \(a^i\in F^i(\mu^i,\sigma^{-i})\) for every \(i\in I\). Thus there exists a single distribution \(\sigma\in\Delta L^+\) such that \(\sigma(a)>0\) and, for every player \(i\), there exists \(\mu^i\in\Delta\Theta^{m,i}(\sigma)\) with \(a^i\in F^i(\mu^i,\sigma^{-i})\). By the definition of \(\Gamma^{CS+}\), this means that \(a\in\Gamma^{CS+}(L^+)\). Since \(a\in L^+\) was arbitrary, \(L^+(a^\infty)\subseteq\Gamma^{CS+}(L^+(a^\infty))\).
\end{proof}

The intuition is that positive limsup frequency lets us synchronize the dates at which a profile is played with the empirical distribution that justifies it. If \(a\) has positive limsup frequency, then along arbitrarily late histories the accumulated frequency of \(a\) is bounded away from zero. Taking the last play of \(a\) before such a history gives dates \(t_k\) at which the current profile is exactly \(a\), while the empirical frequency of \(a\) is still bounded away from zero. Any limiting empirical distribution along these dates therefore assigns positive probability to \(a\). This is precisely the additional requirement in \(\Gamma^{CS+}\).

This argument uses finiteness in an important way. In a general compact action space, a profile may be approached through neighborhoods that receive positive limsup empirical probability, but the relevant mass may come from different nearby profiles or different subsequences. There need not be dates at which current play converges to \(a\) and the empirical distribution along those same dates converges to a measure that assigns positive probability to every neighborhood of \(a\). Thus the positive-frequency common-sample foundation is stated here for finite action spaces.




\subsection{Demian old proof properties}



\begin{lemma}
\label{lem:continuity-correspondences}
For each $i\in I$, the following statements hold:
\begin{enumerate}
    \item The best-response correspondence,
   $F^i:    \Delta \Theta^i \times\Delta \mathbb A^{-i}
        \rightrightarrows \mathbb A^i $, is nonempty-valued, compact-valued, and upper hemicontinuous.

    \item The correspondence of KL minimizers,
$ \Theta^{m,i}:
        \Delta \mathbb A^{i} \rightrightarrows\Theta^i$,    is nonempty-valued, compact-valued, and upper hemicontinuous.
\end{enumerate}
\end{lemma}

\begin{proof}
Fix $i\in I$.

\medskip
\noindent
\textit{Part (i).}
Define
\begin{align}
    \overline U^i(a^i,\theta^i,a^{-i})
    :=
    \int_{Y^i}
    \pi^i(a^i,y^i)
    q^i_{\theta^i}(y^i\mid a^i,a^{-i})
    \nu^i(dy^i).
    \label{eq:Ubar}
\end{align}
By Assumption \ref{ass:game}(XXX), for $\nu^i$-a.e.\ $y^i$, the integrand in
\eqref{eq:Ubar} is continuous in
$(a^i,\theta^i,a^{-i})$.
Moreover, by Assumptions~\ref{ass:game}(XXX)
\begin{align*}
    \left|
        \pi^i(a^i,y^i)
        q^i_{\theta^i}(y^i\mid a^i,a^{-i})
    \right|
    \leq
    h_\pi^i(y^i)
    M^i(y^i)
    q^i(y^i\mid a^i,a^{-i}) \leq
    h_\pi^i(y^i)
    M^i(y^i)
    r^i(y^i),
\end{align*}
and $\int_{Y^i}
    h_\pi^i(y^i)
    M^i(y^i)
    r^i(y^i)
    \nu^i(dy^i)
    <\infty$. 
The Dominated Convergence Theorem therefore implies that
$\overline U^i$ is jointly continuous. The same envelope also implies
that $\overline U^i$ is uniformly bounded.

For
$(\mu^i,\sigma^{-i})
\in
\Delta \Theta^i \times\Delta \mathbb A^{-i} $ ,
define
\begin{align}
    V^i(a^i,\mu^i,\sigma^{-i})
    :=
    \int_{\Theta^i}
    \int_{\mathbb A^{-i}}
    \overline U^i(a^i,\theta^i,a^{-i})
    \sigma^{-i}(da^{-i})
    \mu^i(d\theta^i).
    \label{eq:V}
\end{align}
We claim that $V^i$ is jointly continuous when the spaces of
probability measures are endowed with the weak topology.

Indeed, suppose
\[
    a_n^i\to a^i,
    \qquad
    \mu_n^i\Rightarrow\mu^i,
    \qquad
    \sigma_n^{-i}\Rightarrow\sigma^{-i}.
\]
Because $\Theta^i$ and $\mathbb A^{-i}$ are compact,
\[
    \mu_n^i\otimes\sigma_n^{-i}
    \Rightarrow
    \mu^i\otimes\sigma^{-i}.
\]
Moreover, since
$\mathbb A^{i} \times\Theta^i\times \mathbb A^{-i}$
is compact and $\overline U^i$ is continuous,
$\overline U^i$ is uniformly continuous. Hence
\begin{align}
    &\left|
    V^i(a_n^i,\mu_n^i,\sigma_n^{-i})
    -
    V^i(a^i,\mu^i,\sigma^{-i})
    \right|
    \notag\\
    &\qquad\leq
    \sup_{\theta^i,a^{-i}}
    \left|
        \overline U^i(a_n^i,\theta^i,a^{-i})
        -
        \overline U^i(a^i,\theta^i,a^{-i})
    \right|
    \notag\\
    &\qquad\quad+
    \left|
    \int
    \overline U^i(a^i,\theta^i,a^{-i})
    \,d(\mu_n^i\otimes\sigma_n^{-i})
    -
    \int
    \overline U^i(a^i,\theta^i,a^{-i})
    \,d(\mu^i\otimes\sigma^{-i})
    \right|
    \longrightarrow 0.
\end{align}
Thus $V^i$ is jointly continuous.

By definition,
\begin{align}
    F^i(\mu^i,\sigma^{-i})
    =
    \arg\max_{a^i\in A^i}
    V^i(a^i,\mu^i,\sigma^{-i}).
\end{align}
Since $\mathbb A^{i}$ is nonempty and compact, Weierstrass' theorem implies
that $F^i(\mu^i,\sigma^{-i})$ is nonempty and compact for every
$(\mu^i,\sigma^{-i})$. Since the objective is jointly continuous
and the feasible set $A^i$ is constant and compact, Berge's Maximum
Theorem implies that
\[
    (\mu^i,\sigma^{-i})
    \mapsto
    F^i(\mu^i,\sigma^{-i})
\]
is upper hemicontinuous.

\medskip
\noindent
\textit{Part (ii).}
For convenience, adopt the usual convention
\[
    0\log(0/0):=0.
\]
The likelihood-ratio bound in Assumption \ref{ass:game}(XXX) implies that,
for $\nu^i$-a.e.\ $y^i$ and every $(\theta^i,a)$,
\begin{align}
    \frac{1}{M^i(y^i)}
    \leq
    \frac{q^i(y^i\mid a)}
         {q^i_{\theta^i}(y^i\mid a)}
    \leq
    M^i(y^i)
\end{align}
whenever the densities are positive. Moreover,
\[
    q^i(y^i\mid a)=0
    \quad\Longleftrightarrow\quad
    q^i_{\theta^i}(y^i\mid a)=0.
\]
Consequently,
\begin{align}
    \left|
    \log
    \frac{q^i(y^i\mid a)}
         {q^i_{\theta^i}(y^i\mid a)}
    \right|
    \leq
    \log M^i(y^i)
    \leq
    M^i(y^i)
\end{align}
on the common support of the densities.

Recall that
\begin{align}
    K^i(\theta^i,a)
    :=
    \int_{Y^i}
    q^i(y^i\mid a)
    \log
    \left(
    \frac{q^i(y^i\mid a)}
         {q^i_{\theta^i}(y^i\mid a)}
    \right)
    \nu^i(dy^i).
    \label{eq:KL}
\end{align}
Since $q^i(\cdot\mid a)\leq r^i$, we have
\begin{align}
    \left|
    q^i(y^i\mid a)
    \log
    \left(
    \frac{q^i(y^i\mid a)}
         {q^i_{\theta^i}(y^i\mid a)}
    \right)
    \right|
    \leq
    M^i(y^i)r^i(y^i),
    \label{eq:KL-envelope}
\end{align}
where
\[
    \int_{Y^i}
    M^i(y^i)r^i(y^i)\nu^i(dy^i)<\infty.
\]
In particular, $K^i$ is uniformly bounded.

We next show that $K^i$ is jointly continuous. Let
\[
    (\theta_n^i,a_n)\to(\theta^i,a).
\]
By Assumption \ref{ass:game}(XXX), for $\nu^i$-a.e.\ $y^i$,
\begin{align}
    q^i(y^i\mid a_n)
    &\to
    q^i(y^i\mid a),
    \\
    q^i_{\theta_n^i}(y^i\mid a_n)
    &\to
    q^i_{\theta^i}(y^i\mid a).
\end{align}
Fix such a $y^i$.

If
$q^i_{\theta^i}(y^i\mid a)>0$, continuity of $(u,v)\mapsto u\log(u/v)$ 
on $\{(u,v):u\geq0,\ v>0\}$ gives
\begin{align*}
    q^i(y^i\mid a_n)
    \log
    \frac{q^i(y^i\mid a_n)}
         {q^i_{\theta_n^i}(y^i\mid a_n)} \longrightarrow
    q^i(y^i\mid a)
    \log
    \frac{q^i(y^i\mid a)}
         {q^i_{\theta^i}(y^i\mid a)}.
\end{align*}
If instead
$q^i_{\theta^i}(y^i\mid a)=0$, the likelihood-ratio bound implies
$q^i(y^i\mid a)=0$. Furthermore,
\begin{align}
    \left|
    \log
    \frac{q^i(y^i\mid a_n)}
         {q^i_{\theta_n^i}(y^i\mid a_n)}
    \right|
    \leq M^i(y^i),
\end{align}
with the preceding convention on common zeros, whereas
$q^i(y^i\mid a_n)\to0$. Hence
\begin{align}
    q^i(y^i\mid a_n)
    \log
    \frac{q^i(y^i\mid a_n)}
         {q^i_{\theta_n^i}(y^i\mid a_n)}
    \longrightarrow0.
\end{align}
Thus the integrand in \eqref{eq:KL} converges pointwise
$\nu^i$-a.e. The domination in \eqref{eq:KL-envelope} and the
Dominated Convergence Theorem imply
\[
    K^i(\theta_n^i,a_n)
    \longrightarrow
    K^i(\theta^i,a).
\]
Therefore $(\theta^i,a)\mapsto K^i(\theta^i,a)$ is bounded and
continuous.

For $\sigma\in\Delta \mathbb A^{i}$, define
\begin{align}
    K^i(\theta^i,\sigma)
    :=
    \int_{\mathbb A^{i}} K^i(\theta^i,a)\sigma(da).
\end{align}
We claim that
\[
    (\theta^i,\sigma)
    \mapsto
    K^i(\theta^i,\sigma)
\]
is continuous on $\Theta^i\times\Delta \mathbb A^{i} $. Indeed, if
$\theta_n^i\to\theta^i$ and $\sigma_n\Rightarrow\sigma$, then
\begin{align}
    \left|
    K^i(\theta_n^i,\sigma_n)
    -
    K^i(\theta^i,\sigma)
    \right| \leq
    \sup_{a\in \mathbb A^{i}}
    \left|
        K^i(\theta_n^i,a)-K^i(\theta^i,a)
    \right|
    +
    \left|
        \int_{\mathbb A^{i}} K^i(\theta^i,a)
        (\sigma_n-\sigma)(da)
    \right|
    \longrightarrow0,
\end{align}
where the first term converges to zero by uniform continuity of
$K^i$ on the compact set $\Theta^i\times \mathbb A^{i}$, and the second by weak
convergence.

Finally,
\begin{align}
    \Theta^{m,i}(\sigma)
    :=
    \arg\min_{\theta^i\in\Theta^i}
    K^i(\theta^i,\sigma).
\end{align}
Since $\Theta^i$ is nonempty and compact and the criterion is
continuous, Weierstrass' theorem implies that
$\Theta^{m,i}(\sigma)$ is nonempty and compact for every $\sigma$.
Berge's Maximum Theorem then implies that
\[
    \sigma\mapsto\Theta^{m,i}(\sigma)
\]
is upper hemicontinuous.
\end{proof}





\subsection{old theorem 5}

\subsection{Nacho}

PROOF:

Idea of proof:

The role of identification is to make the limiting belief induced by a selected sample
unique. Self-justification says that, for every \(a\in S\) and every player
\(i\), there is a selected-sample distribution \(\sigma_a^i\in\Delta S\) and a
belief over best-fitting models that makes \(a^i\) optimal. Under identification,
this belief is pinned down by the sample distribution itself:
\[
\Theta^{m,i}(\sigma_a^i)=\{\theta^i(\sigma_a^i)\}.
\]
Thus the supporting condition can be written as
\[
a^i\in
F^i\left(
\delta_{\theta^i(\sigma_a^i)},(\sigma_a^i)^{-i}
\right).
\]
This is useful for the construction because, once the selected empirical
distribution is made close to \(\sigma_a^i\), Bayesian learning drives player
\(i\)'s posterior close to the unique model \(\theta^i(\sigma_a^i)\). The
resulting belief is therefore determined by the sampled actions.

Without identification, the selected empirical distribution generally determines
only the set \(\Theta^{m,i}(\sigma_a^i)\), not the limiting posterior within
that set. The posterior may fail to converge, or it may converge to a mixture
that depends on the prior and on likelihood ratios among observationally
equivalent models. This creates a difficulty for a sustaining result: the belief
that learning produces need not be the particular belief over
\(\Theta^{m,i}(\sigma_a^i)\) that justifies \(a^i\). The problem is especially
pronounced for set-valued steady states, because different actions in \(S\), and
different players, may require different supporting beliefs. Identification
avoids this compatibility issue.

The proof constructs a target path whose set of limit points is exactly \(S\).
Since \(S\) is compact, one can choose a deterministic sequence
\[
z_1,z_2,\ldots \in S
\]
such that
\[
L(z^\infty)=S.
\]
At each date \(t\), the intended action profile is \(z_t\). For each player
\(i\), the sampling rule is chosen so that, along the target path, the selected
empirical distribution \(\hat\sigma_t^i\) is close to a distribution
\(\sigma_{z_t}^i\in\Delta S\) that justifies \(z_t^i\). In the finite case this
means selecting past observations in approximately the desired frequencies. In
the compact case, the selected empirical distributions approximate
\(\sigma_{z_t}^i\) weakly.

Forecasts are empirical forecasts from the selected sample, so
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i}.
\]
Therefore, along the target path,
\[
\hat\sigma_t^i \approx \sigma_{z_t}^i
\quad\Longrightarrow\quad
\tilde\sigma_t^{-i}\approx (\sigma_{z_t}^i)^{-i}.
\]
By identification and Bayesian learning from the selected sample, player \(i\)'s
posterior is close to
\[
\delta_{\theta^i(\sigma_{z_t}^i)}.
\]
Since \(z_t^i\) is optimal under the limiting belief and forecast,
continuity implies that the payoff loss from playing \(z_t^i\) converges to
zero along the target path.

Finally, choose a deterministic sequence \(\varepsilon_t\downarrow0\) slowly
enough so that, with probability at least \(1-\alpha\), the intended action
\(z_t^i\) is \(\varepsilon_t\)-optimal for every player and every date. The
actual action rule is then defined as follows: play the intended action \(z_t^i\)
whenever it is \(\varepsilon_t\)-optimal, and otherwise play an exact best
response. This rule is always \(\varepsilon_t\)-optimal. On the high-probability
event, the exception never occurs, so the realized action path coincides with
the target path and hence
\[
L(a^\infty)=L(z^\infty)=S.
\]


\begin{proof}
Let \(d\) be a metric that metrizes weak convergence on \(\Delta\mathbb A\). Since \(S\) is compact, for each \(n\geq 1\) let \(E_n\subseteq S\) be a finite \(1/n\)-net. Choose integers \(k_n,r_n\to\infty\) such that \(k_n\le r_n\) and \(|E_n|/k_n\to0\). Construct a deterministic target path \(z^\infty=(z_t)_{t\ge1}\) by concatenating blocks \(B_n\), where block \(B_n\) lists each element of \(E_n\) exactly \(r_n\) times. Then \(z_t\in S\) for all \(t\) and \(L(z^\infty)=S\).

For each date \(t\) and player \(i\), self-justification of \(S\) and identification imply that there exists \(\rho_t^i\in\Delta S\) such that
\[
z_t^i\in F^i\left(\delta_{\theta^i(\rho_t^i)},(\rho_t^i)^{-i}\right).
\]
We now define the selected-sample rule along the target path. If \(t\) belongs to block \(B_{n+1}\), let \(p_n:S\to E_n\) be a measurable nearest-net projection and let \(\bar\rho_t^i=(p_n)_\#\rho_t^i\). Since every element of \(E_n\) appears \(r_n\) times in block \(B_n\), choose \(k_n\) observations from block \(B_n\) whose empirical distribution over \(E_n\) is within total variation distance at most \(|E_n|/k_n\) of \(\bar\rho_t^i\). Let \(H_t^i\) be the corresponding set of dates. For dates in the first block, define \(H_t^i\) arbitrarily. At histories that do not coincide with the target path, let \(H_t^i=\{1,\ldots,t-1\}\). Then the selected-sample rule depends only on the past action history, \(|H_t^i|\to\infty\) along every infinite path, and along the target path,
\[
d(\hat\sigma_t^i,\rho_t^i)\to0
\qquad\text{for every }i.
\]
Forecasts are empirical forecasts from the selected sample:
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i}.
\]

Let \(\mathbf P^z\) denote the probability law over consequence paths induced when the action path is fixed at \(z^\infty\). Let \(\mu_t^{i,z}\), \(\hat\sigma_t^{i,z}\), and \(\tilde\sigma_t^{-i,z}\) denote the posterior, selected empirical distribution, and forecast generated along this target path. Define the payoff loss from the target action by
\[
\ell_t^i
=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\tilde\sigma_t^{-i,z},\theta^i)\,\mu_t^{i,z}(d\theta^i)
-
\int_{\Theta^i}U^i(z_t^i,\tilde\sigma_t^{-i,z},\theta^i)\,\mu_t^{i,z}(d\theta^i),
\]
and set \(\ell_t=\max_i\ell_t^i\).

We claim that \(\ell_t\to0\), \(\mathbf P^z\)-almost surely. Suppose not. Then, for some player \(i\), some \(\eta>0\), and some subsequence \(t_m\), \(\ell_{t_m}^i\ge\eta\). Passing to a further subsequence, compactness implies
\[
z_{t_m}\to a\in S,
\qquad
\rho_{t_m}^i\Rightarrow \rho^i\in\Delta S,
\qquad
\mu_{t_m}^{i,z}\Rightarrow \mu^i.
\]
Since \(d(\hat\sigma_{t_m}^{i,z},\rho_{t_m}^i)\to0\), we also have \(\hat\sigma_{t_m}^{i,z}\Rightarrow\rho^i\) and \(\tilde\sigma_{t_m}^{-i,z}\Rightarrow(\rho^i)^{-i}\). By the asymptotic-belief lemma and identification,
\[
\mu^i=\delta_{\theta^i(\rho^i)}.
\]
Moreover, since \(z_{t_m}^i\in F^i(\delta_{\theta^i(\rho_{t_m}^i)},(\rho_{t_m}^i)^{-i})\), upper hemicontinuity of \(\Theta^{m,i}\), identification, and the closed graph of \(F^i\) imply
\[
a^i\in F^i\left(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\right).
\]
By continuity of expected payoffs, the payoff loss from \(z_{t_m}^i\) under \((\mu_{t_m}^{i,z},\tilde\sigma_{t_m}^{-i,z})\) therefore converges to zero, contradicting \(\ell_{t_m}^i\ge\eta\). Hence \(\ell_t\to0\) almost surely.

Since \(\ell_t\to0\) \(\mathbf P^z\)-almost surely, there exists a deterministic sequence \(\varepsilon_t\downarrow0\) such that
\[
\mathbf P^z\left(\ell_t\le \varepsilon_t\text{ for all }t\right)>1-\alpha.
\]
For each player \(i\), define the action rule as follows. At date \(t\), after computing \(\mu_t^i\) and \(\tilde\sigma_t^{-i}\), player \(i\) plays \(z_t^i\) if
\[
z_t^i\in F^i_{\varepsilon_t}(\mu_t^i,\tilde\sigma_t^{-i});
\]
otherwise she plays an arbitrary exact best response in \(F^i(\mu_t^i,\tilde\sigma_t^{-i})\). This rule is \(\varepsilon_t\)-optimal at every history.


Let \(G\) be the event, computed under the target path \(z^\infty\), that
\[
\ell_t^i\leq \varepsilon_t
\quad\text{for every }i\text{ and every }t.
\]
By construction, \(\mathbf P^z(G)>1-\alpha\). We claim that, on \(G\), the action path generated by the learning rule coincides with the target path.

The claim follows by induction.  At date \(1\), the realized history and the target history are both empty. Suppose that the realized action path has coincided with the target path through date \(t-1\). Then, at date \(t\), every player's selected sample, posterior, and forecast are exactly those generated along the target path. Since \(G\) holds, the target action \(z_t^i\) is \(\varepsilon_t\)-optimal for each player \(i\). The action rule therefore prescribes \(z_t^i\) for every player. Hence the realized action profile at date \(t\) is \(z_t\). This proves the induction step.

Thus, on \(G\), \(a_t=z_t\) for all \(t\). Since \(L(z^\infty)=S\), it follows that
\[
L(a^\infty)=S
\]
on \(G\). Therefore
\[
\mathbf P\bigl(L(a^\infty)=S\bigr)\geq \mathbf P^z(G)>1-\alpha.
\]

\end{proof}


\subsection{Demian}

Let $(\delta_{n})_{n}$ be a positive real-valued vanishing sequence. By compactness of $S$, for every $n$, there exists $\delta_{n}$-net of $S_{n}$ which we denote as $X_{n} : = \{x_{1,n}, \ldots, x_{J_{n},n} \} $. Let $\Pi_{n} : S \to X_{n}$ be the projection operator and let $\Pi^{-1}_{n}(x) \subseteq S$ be the set of points in $S$ that project onto $x \in X_{n}$. 

We construct the sequence $z^{\infty}$ as follows. For each $n$, let $m_{n} \in \mathbb{N}$ be given and let $B_{n} : = X_{n}^{m_{n}}$. That is, $B_{n}$ is a block of length $J_{n} m_{n}$ wherein each element of $X_{n}$ appears $m_{n}$ times. Let $z^{\infty} = \{ B_{1} , B_{2} , \ldots \} $. For each data $t$, let $n(t)+1$ be the block number containing $t$, i.e., $n(t)$ is the maximal integer such that $t \geq T_{n(t)} : = \sum_{n=1}^{n(t)} J_{n} m_{n}$. 

We observe that by choosing the $\delta_{n}$-net to be the smallest possible it follows that $J_{n}$ equals the covering number, $N(S,||.||,\delta_{n})$. If $S$ is a compact set of $\mathbb R^{d}$, then $J_{n} = O(\delta_{n}^{-d})$.  We take $m_{n}$ to be such that $\lim_{n \to \infty} \frac{J_{n}}{m_{n}} = 0$.

Under this construction of $z^{\infty}$ it follows that

\begin{lemma}\label{lem:LimitSet.S}
    $L(z^{\infty}) = S$.
\end{lemma}

For each date \(t\) and player \(i\), self-justification of \(S\) and identification imply that there exists \(\rho_i(\cdot \mid z_{t}) \in\Delta S\) such that
\[
z_t^i\in F^i\left(\delta_{\theta^i(\rho_i(\cdot \mid z_{t}) )},(\rho_i(\cdot \mid z_{t}) )^{-i}\right).
\]

The next lemma shows that, for each player, there exists a sampling scheme $(H^{i}_{t})_{t}$ for which $\lim_{t \to \infty} W_{1}\left( \widehat{\sigma}^{i}_{t} , \rho_i(\cdot \mid z_{t})  \right)  =0$ provided $J_{n}/m_{n} \to 0$. 


\begin{lemma}\label{lem:sustain.Empirical}
    For each player $i$ and each date $t$, there exists a $H^{i}_{t} \subseteq \{ 1, \ldots, t\}    $ such that 
\begin{align}
    W_{1}\left( \widehat{\sigma}^{i}_{t} , \rho_i(\cdot \mid z_{t})  \right) \leq \delta_{n(t)} + \frac{\operatorname{diam}(S)}{2} \frac{J_{n(t)}}{m_{n(t)}}
\end{align}
where $\widehat{\sigma}^{i}_{t}: = |H^{i}_{t}|^{-1} \sum_{l \in H^{i}_{t}} \delta_{z_{l}}$.
\end{lemma}



For each player $i$ and date $t$, the forecasts of other players, $\widetilde{\sigma}^{-i}_{t}$ is given by $(\widehat{\sigma}^{i}_{t})^{-i}$. The next lemma shows that given these forecasts, under the condition that $\frac{J_{n}}{m_{n}} \to 0$,  $z^{i}_{t}$ is asymptotically optimal. To do this, let $\mathbf{P}_{z^{\infty}} \in \Delta (\mathbb{A} \times \mathbb{Y})^{\mathbb{N}}$ denote the joint probability law over action-consequence paths that puts probability one on the action path being given by \(z^\infty\).

\begin{lemma}\label{lem:sustain.AsympOptimal}
For each player $i$,
    \begin{align}
    \lim_{t \to \infty}    \left| \sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\tilde\sigma_t^{-i},\theta^i)\,\mu_t^{i}(d\theta^i)
-
\int_{\Theta^i}U^i(z_t^i,\tilde\sigma_t^{-i},\theta^i)\,\mu_t^{i}(d\theta^i) \right| = 0
    \end{align}
$\mathbf{P}_{z^{\infty}}$-almost surely
\end{lemma}


Given this result, the following lemma shows that there exists a deterministic sequence $(\varepsilon'_{t})_{t}$ such that $\lim_{t \to \infty} \varepsilon'_{t} =0 $ and the set 
\begin{align}
    \Omega : = \left\{ \omega \in (\mathbb A \times \mathbb Y)^{\mathbb{N} } \colon \exists T(\omega) \in \mathbb{N}~s.t.~ |\ell^{i}_{t}(\omega)| \leq \varepsilon'_{t}~\forall i,\forall t \geq T(\omega)     \right\} 
\end{align}
is such that $\mathbf{P}_{z^{\infty}}(\Omega)  = 1  $.

\begin{lemma}\label{lem:EAS}
Let $(\ell_t)_{t\geq 1}$ be a sequence of nonnegative random variables such that
\begin{align}
\ell_t \rightarrow 0
\qquad
P_z\text{-almost surely}.
\end{align}
Then there exists a deterministic sequence $(\varepsilon_t)_{t\geq 1}$ satisfying $\varepsilon_t \downarrow 0$  such that
\begin{align}
\ell_t \leq \varepsilon_t
\qquad
\text{eventually }P_z\text{-almost surely}.
\end{align}
%Equivalently,
%\begin{align}
%P_z\left(\bigcup_{T=1}^{\infty}\bigcap_{t\geq T}\left\{\ell_t\leq \varepsilon_t\right\}\right)=1.
%\end{align}
\end{lemma}









The next lemma provides a uniform version --- where $T$ does not depend on the realized sequence $\omega$ --- with arbitrary large probability

\begin{lemma}\label{lem:Egorov}
Suppose there exists a deterministic sequence $(\varepsilon'_t)_{t\geq 1}$ such that
$\varepsilon'_t \to 0$ and
\begin{align*}
    \Omega
    :=
    \left\{
    \omega \in (\mathbb A \times \mathbb Y)^{\mathbb N}
    :
    \exists\, T(\omega)\in\mathbb N
    \text{ such that }
    |\ell_t^i(\omega)|
    \leq \varepsilon'_t
    \quad
    \forall i,\ \forall t\geq T(\omega)
    \right\}
\end{align*}
satisfies
\[
\mathbf P_{z^\infty}(\Omega)=1.
\]
Then, for every $\delta>0$, there exists a deterministic
$T(\delta)\in\mathbb N$ such that
\begin{align*}
    \mathbf P_{z^\infty}
    \left(
    |\ell_t^i(\omega)|
    \leq \varepsilon'_t
    \quad
    \forall i,\ \forall t\geq T(\delta)
    \right)
    \geq 1-\delta.
\end{align*}
\end{lemma}



Let $\delta = \alpha$ in the lemma. We now show that, for each player $i$, the learning rule $\langle (H^{i}_{t} )_{t\in \mathbb{N}} , (\widehat{\sigma}^{i}_{t} )_{t\in \mathbb{N}} , ( \mathbf{a}^{i}_{t} )_{t\in \mathbb{N}}  \rangle$ with $\mathbf{a}^{i}_{t} = z^{i}_{t}$ $\forall i, \forall t$ is asymptotically optimal with tolerance \(\varepsilon_t\) for any $\omega \in 
    \Omega_{T(\delta)}
    :=
    \left\{
    \omega \in (\mathbb A \times \mathbb Y)^{\mathbb N}
    :
    |\ell_t^i(\omega)|
    \leq \varepsilon'_t
    \quad
    \forall i,\ \forall t\geq T(\delta)
    \right\}$. 
    
    To do this, let $\varepsilon_{t}$ be defined as follows: For any $t \geq T(\delta)$, $\varepsilon_{t} = \varepsilon'_{t}$ and for any $t < T(\delta)$ let $\varepsilon_{t}$ be large enough so that $|\ell^{i}_{t}(\omega)| \le \varepsilon_{t}$ holds for every player $i$ and every $\omega$ --- such $\varepsilon_{t}$ exists because by Assumption XXX payoffs are bounded over compact sets. Under this definition and the construction of $\Omega_{T(\delta)}$ is clear that for any $\omega \in \Omega_{T(\delta)}$, $z^{i}_{t} \in F^{i}_{\varepsilon_{t}}(\mu^{i}_{t}, \widetilde{\sigma}^{-i}_{t})$ for all $t$. Since $\varepsilon'_{t} \to 0$ as $t \to \infty$, the desired result readily follows. 

   Finally, observe that 
    \begin{align*}
        \mathbf{P} \left( L(\mathbf{a}^{\infty}) = S  \right) & \geq \mathbf{P} \left( L(a^{\infty}) = S \cap \Omega_{T(\delta)}  \right) \\
        & = \mathbf{P}_{z^{\infty}} \left( L(z^{\infty}) = S \cap \Omega_{T(\delta)}  \right) \\
        & = \mathbf{P}_{z^{\infty}} \left( \Omega_{T(\delta)}  \right),
    \end{align*}
    where the first line follows from probability laws; the second line follows because over $\Omega_{T(\delta)}$, $\mathbf{a}^{\infty} = z^{\infty}$ and thus $\mathbf{P} = \mathbf{P}_{z^{\infty}}$; the third line follow because the even $\{L(z^{\infty})=S\}$ always occurs by Lemma \ref{lem:LimitSet.S}. Since $\mathbf{P}_{z^{\infty}} \left( \Omega_{T(\delta)}  \right) \geq 1- \delta$ by Lemma \ref{lem:Egorov} and $\delta = \alpha$, it follows that 
    \begin{align}
         \mathbf{P} \left( L(\mathbf{a}^{\infty}) = S  \right) \ge 1-\alpha
    \end{align}
    as desired. 
 

XXX SOMETHING TO DISCUSS: THE PROBABILITIES $\mathbf{P}$ ARE NOT REALLY WELL-DEFINED AS WE NEVER POSTULATE A PROB DISTRIBUTION OVER ACTIONS, ONLY THAT $action \in F(...)$. I HAVE WORKED ASSUMING THAT THIS PROBABILITIES WERE DEFINED USING A DEGENERATE DISTRIBUTION OVER THE ACTION Z XXX




\subsubsection{Proofs and Supplemental Lemmas}

\begin{proof}[Proof of Lemma \ref{lem:LimitSet.S}]
    Take any $s \in S$ and any $\epsilon>0$. By definition of $(X_{n},\Pi_{n},\delta_{n})$, for $n$ sufficiently large, $d(s,\Pi_{n}(s)) \leq \delta_{n} < \epsilon$. Since $\Pi_{n}(s)$ appears at least once in each block $B_{n}$ for all $n$, we constructed a sub-sequence, $(\Pi_{n}(s))_{n}$ in $z^{\infty}$ that has $s$ as limit point. Therefore, $S \subseteq L(z^{\infty})$. 

    Observe that all $z \in L(z^{\infty})$ must be the limit of some sub-sequence, $(z'_{m(n)})_{n}$ such that $z'_{m(n)} \in B_{m(n)}$. But limits of such sub-sequence converge to $S$. So, $z \in S$. 
\end{proof}



\begin{proof}[Proof of Lemma \ref{lem:sustain.Empirical}]
To ease the notational burden, the following construction is for all players $i$ and the subscript $i$ will be omitted in the intermediate quantities. Also, we set $n: = n(t)$. 


   For each $j \in [J_{n}]$, let
\begin{align*}
	B_n(j)
	:=
	\left\{
		i\in\{T_{n-1}+1,\ldots,T_n\}
		:
		z_i=x_{n,j}
	\right\}.
\end{align*}
Hence, $B_n(j)$ is the set of dates in block $B_n$ at which the
sequence equals the $j$-th element of $X_n$. By construction, $|B_n(j)|=m_n$. 

Let $H^{i}_{t}(j)$ be any subset of $B_{n}(j)$ such that $|H^{i}_{t}(j)| = N_{t,n}(j)$ where $N_{t,n}(j)$ is a non-negative integer constructed below, and let $H^{i}_{t} : = \cup_{j \in [J_{n}]} H^{i}_{t}(j)$. 

We now construct $N_{t,n}(j)$ for all $j \in [J_{n}]$. For any $j \in [J_{n}]$, let $w_{t,n}(j) : = \rho^{i}( \Pi_{n}^{-1}(x_{j}) \mid z_{t})$. Let 
\begin{align*}
	b_{t,n}(j)
	&:=
	\left\lfloor m_n w_{t,n}(j)\right\rfloor,\\
	r_{t,n}(j)
	&:=
	m_n w_{t,n}(j)-b_{t,n}(j)
	\in[0,1),
	\qquad j=1,\ldots,J_n.
\end{align*}
Because $\sum_{j=1}^{J_n}m_n w_{t,n}(j)=m_n$, the number of counts that remain is $R_{t,n}:=
	m_n-\sum_{j=1}^{J_n}b_{t,n}(j)=\sum_{j=1}^{J_n}r_{t,n}(j)$. In particular, $R_{t,n}$ is an integer satisfying $0\leq R_{t,n}\leq J_n-1$. 

Let $(j_1,\ldots,j_{J_n})$ be a permutation of
$\{1,\ldots,J_n\}$ such that $r_{t,n}(j_1)
	\geq
	r_{t,n}(j_2)
	\geq
	\cdots
	\geq
	r_{t,n}(j_{J_n})$, 
where ties are resolved according to any fixed rule. Define $N_{t,n}(j)
	:=
	b_{t,n}(j)
	+
	\mathbf 1
	\left\{
		j\in\{j_1,\ldots,j_{R_{t,n}}\}
	\right\}$. 
That is, we begin with
$\lfloor m_n w_{t,n}(j)\rfloor$ observations at each grid point and
add one observation to each of the $R_{t,n}$ grid points having the
largest fractional remainders.

By construction, $\sum_{j=1}^{J_n}N_{t,n}(j)
	=
	\sum_{j=1}^{J_n}b_{t,n}(j)+R_{t,n} =
	m_n$. 
Moreover, if $j\notin\{j_1,\ldots,j_{R_{t,n}}\}$, then
\begin{align*}
	N_{t,n}(j)-m_n w_{t,n}(j)
	=
	-r_{t,n}(j)
	\in(-1,0].
\end{align*}
If $j\in\{j_1,\ldots,j_{R_{t,n}}\}$, then
\begin{align*}
	N_{t,n}(j)-m_n w_{t,n}(j)
	=
	1-r_{t,n}(j)
	\in(0,1).
\end{align*}
The last inclusion follows because only indices with strictly positive
fractional remainder need to receive an additional count. Consequently,
\begin{align*}
	\left|
	\frac{N_{t,n}(j)}{m_n}-w_{t,n}(j)
	\right|
	<
	\frac{1}{m_n},
	\qquad j=1,\ldots,J_n.
\end{align*}
    
By definition, $\widehat{\sigma}^{i}_t
	=
	\frac{1}{|H_t|}
	\sum_{i\in H_t}\delta_{z_i}$, 
so, partitioning $H_t$ into the disjoint sets
$H_t(1),\ldots,H_t(J_n)$, we obtain $\widehat{\sigma}^{i}_t
	=
	\frac{1}{|H_t|}
	\sum_{j=1}^{J_n}
	\sum_{i\in H_t(j)}
	\delta_{z_i}$. 
For every $i\in H_t(j)$, we have $z_i=x_{n,j}$. Therefore,
\begin{align*}
	\sum_{i\in H_t(j)}\delta_{z_i}
	=
	\sum_{i\in H_t(j)}\delta_{x_{n,j}} =
	|H_t(j)|\delta_{x_{n,j}}=
	N_{t,n}(j)\delta_{x_{n,j}}.
\end{align*}
Substituting this expression and using $|H_t|=m_n$ gives
\begin{align*}
	\widehat{\sigma}^{i}_t
	=
	\frac{1}{m_n}
	\sum_{j=1}^{J_n}
	N_{t,n}(j)\delta_{x_{n,j}}.
\end{align*}

By the triangle inequality
\begin{align}
    W_{1}(\widehat{\sigma}^{i}_{t}, \rho^{i}(\cdot \mid z_{t})) \leq W_{1}(\widehat{\sigma}^{i}_{t}, \rho^{i} \circ \Pi^{-1}_{n} ( \cdot \mid z_{t})) + W_{1}( \rho^{i} \circ \Pi^{-1}_{n} ( \cdot \mid z_{t}), \rho^{i}(\cdot \mid z_{t})).
\end{align}

Let $D:=\operatorname{diam}(S)<\infty$. Then, 
\begin{align*}
	W_1(\widehat{\sigma}^{i}_t,\rho^{i} \circ \Pi^{-1}_{n} ( \cdot \mid z_{t}))
	&\leq
	D\left\|\widehat{\sigma}^{i}_t-\rho^{i} \circ \Pi^{-1}_{n} ( \cdot \mid z_{t})\right\|_{\mathrm{TV}}\\
	&=
	\frac{D}{2}
	\sum_{j=1}^{J_n}
	\left|
	\frac{N_{t,n}(j)}{m_n}
	-
	\rho^{i} \left(\Pi_n^{-1}\bigl(\{x_{n,j}\}\bigr) \mid z_{t} \right)
	\right|\\
    & =  \frac{D}{2}
	\sum_{j=1}^{J_n}
	\left|
	\frac{N_{t,n}(j)}{m_n}
	- w_{t,n}(j)
	\right|\\
	&\leq
	\frac{D J_n}{2m_n}.
\end{align*}

Since the projection $\Pi_{n}$ only ``moves" points by at most $\delta_{n}$, $W_{1}( \rho^{i} \circ \Pi^{-1}_{n} ( \cdot \mid z_{t}), \rho^{i}(\cdot \mid z_{t})) \leq \delta_{n}$. Thus, the desired result follows. 
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:sustain.AsympOptimal}]
 Define the payoff loss from the target action by
\[
\ell_t^i
=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\tilde\sigma_t^{-i},\theta^i)\,\mu_t^{i}(d\theta^i)
-
\int_{\Theta^i}U^i(z_t^i,\tilde\sigma_t^{-i},\theta^i)\,\mu_t^{i}(d\theta^i),
\]
and set \(\ell_t=\max_i\ell_t^i\).

We claim that \(\ell_t\to0\), $\mathbf{P}_{z^{\infty}}$-almost surely. Suppose not. Then, for some player \(i\), some \(\eta>0\), and some subsequence \(t_m\), \(\ell_{t_m}^i\ge\eta\). Passing to a further subsequence, compactness implies
\[
z_{t_m}\to a\in S,
\qquad
\rho_{t_m}^i\Rightarrow \rho^i\in\Delta S,
\qquad
\mu_{t_m}^{i}\Rightarrow \mu^i.
\]
Since, by Lemma \ref{lem:sustain.Empirical}, \(W_{1}(\hat\sigma_{t_m}^{i},\rho_{t_m}^i)\to0\), we also have \(\hat\sigma_{t_m}^{i}\Rightarrow\rho^i\) and \(\tilde\sigma_{t_m}^{-i}\Rightarrow(\rho^i)^{-i}\). By the asymptotic-belief lemma and identification,
\[
\mu^i=\delta_{\theta^i(\rho^i)}.
\]
Moreover, since \(z_{t_m}^i\in F^i(\delta_{\theta^i(\rho_{t_m}^i)},(\rho_{t_m}^i)^{-i})\), upper hemicontinuity of \(\Theta^{m,i}\), identification, and the closed graph of \(F^i\) imply
\[
a^i\in F^i\left(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\right).
\]
By continuity of expected payoffs, the payoff loss from \(z_{t_m}^i\) under \((\mu_{t_m}^{i},\tilde\sigma_{t_m}^{-i})\) therefore converges to zero, contradicting \(\ell_{t_m}^i\ge\eta\). Hence \(\ell_t\to0\) almost surely.
\end{proof}









\begin{comment}
\begin{lemma}
\label{lem:empirical-justification}
Let $\mathcal Z$ be a finite set, and suppose that, for every
$z\in\mathcal Z$, $q(\cdot\mid z)$ is a probability distribution on
$\mathcal Z$. Then there exist a deterministic sequence
$z^{\infty} : = (z_t)_{t\geq 1}$ in $\mathcal Z$ and sets
\[
H_t\subseteq\{1,\ldots,t\},\qquad \forall t \in \mathbb{N}
\]
such that, defining
\[
p_t(x)
:=
\frac{1}{|H_t|}
\sum_{i\in H_t}\mathbf 1\{z_i=x\},
\qquad x\in\mathcal Z,
\]
we have
\[
\left\|p_t-q(\cdot\mid z_t)\right\|=o(1).
\]
Indeed, the sequence and sampling sets can be chosen so that
\[
\left\|p_t-q(\cdot\mid z_t)\right\|_\infty
=
O(t^{-1}).
\]
\end{lemma}

\begin{proof}
Write $\mathcal Z=\{1,\ldots,K\}$ and define the deterministic cyclic
sequence
\[
z_t
=
1+\big((t-1)\bmod K\big),
\qquad t\geq 1.
\]
Thus, $(z_t)_{t\geq 1}$ repeatedly cycles through
$1,\ldots,K$. For $t\geq K$, let
\[
m_t:=\left\lfloor\frac{t}{K}\right\rfloor.
\]
By date $t$, every $x\in\mathcal Z$ has appeared at least $m_t$ times.

For each $t\geq K$, choose nonnegative integers
$\{n_t(x):x\in\mathcal Z\}$ satisfying
\begin{align}
\sum_{x\in\mathcal Z}n_t(x)&=m_t,
\label{eq:integer-count-total}\\
\left|n_t(x)-m_tq(x\mid z_t)\right|&<1,
\qquad x\in\mathcal Z.
\label{eq:integer-count-error}
\end{align}
Such integers can be obtained by the largest-remainder rule. In
particular, first set
\[
a_t(x):=\left\lfloor m_tq(x\mid z_t)\right\rfloor
\]
and define
\[
R_t
:=
m_t-\sum_{x\in\mathcal Z}a_t(x).
\]
Starting from $a_t(x)$, add one to the counts corresponding to the
$R_t$ largest fractional parts of $m_tq(x\mid z_t)$. The resulting
integers $n_t(x)$ satisfy
\eqref{eq:integer-count-total}--\eqref{eq:integer-count-error}.

Under the cyclic construction, the dates at which $z_i=x$ are
\[
x,\ x+K,\ x+2K,\ldots.
\]
Define
\[
H_t(x)
:=
\left\{
x+(r-1)K:
r=1,\ldots,n_t(x)
\right\},
\]
where $H_t(x)=\varnothing$ if $n_t(x)=0$, and let
\[
H_t
:=
\bigcup_{x\in\mathcal Z}H_t(x).
\]
Because $n_t(x)\leq m_t$, every index in $H_t(x)$ is no larger than
\[
x+\big(m_t-1\big)K
\leq
K+\big(m_t-1\big)K
=
m_tK
\leq t.
\]
It follows that
\[
H_t\subseteq\{1,\ldots,t\}.
\]
Moreover, the sets $\{H_t(x):x\in\mathcal Z\}$ are pairwise disjoint,
so
\[
|H_t|
=
\sum_{x\in\mathcal Z}|H_t(x)|
=
\sum_{x\in\mathcal Z}n_t(x)
=
m_t.
\]

For every $x\in\mathcal Z$, the set $H_t$ contains exactly $n_t(x)$
dates at which the sequence takes the value $x$. Consequently,
\[
p_t(x)
=
\frac{n_t(x)}{m_t}.
\]
Using \eqref{eq:integer-count-error}, we obtain
\begin{align*}
\left|p_t(x)-q(x\mid z_t)\right|
&=
\frac{1}{m_t}
\left|n_t(x)-m_tq(x\mid z_t)\right|\\
&<
\frac{1}{m_t}.
\end{align*}
Therefore,
\[
\left\|p_t-q(\cdot\mid z_t)\right\|_\infty
<
\frac{1}{m_t}
=
\frac{1}{\lfloor t/K\rfloor}
=
O(t^{-1}).
\]
Since $\mathcal Z$ is finite, all norms on $\mathbb R^K$ are
equivalent. Hence,
\[
\left\|p_t-q(\cdot\mid z_t)\right\|
=
o(1)
\]
for any norm on $\mathbb R^K$. The sampling sets for the finitely many
dates $t<K$ may be defined arbitrarily, subject to being nonempty.
\end{proof}
\end{comment}




\begin{proof}[Proof of Lemma \ref{lem:EAS}]
For each $n\geq 1$, define
\begin{align}
R_n
:=
\sup_{t\geq n}\ell_t.
\end{align}
Since $\ell_t\to 0$ $P_z$-almost surely, it follows that
$R_n
\rightarrow
0$ $P_z\text{-almost surely}$. In particular, $R_n\to 0$ in $P_z$-probability. Therefore, for every $k\geq 1$, there exists a deterministic integer $N_k$ such that
\begin{align}
P_z\left(
R_{N_k}>\frac{1}{k}
\right)
\leq
2^{-k}.
\end{align}
The sequence $(N_k)_{k\geq 1}$ may be chosen to be strictly increasing.

Since
\begin{align}
\sum_{k=1}^{\infty}
P_z\left(
R_{N_k}>\frac{1}{k}
\right)
\leq
\sum_{k=1}^{\infty}2^{-k}
<
\infty,
\end{align}
the Borel--Cantelli lemma implies that $P_z\left(
R_{N_k}>\frac{1}{k}
\text{ infinitely often}
\right)
=
0$. Hence, for $P_z$-almost every outcome, there exists a finite random integer $K$ such that
\begin{align}
R_{N_k}
\leq
\frac{1}{k}
\qquad
\text{for every }k\geq K.
\end{align}

Define the deterministic sequence $(\varepsilon_t)_{t\geq 1}$ by
\begin{align}
\varepsilon_t
:=
\begin{cases}
1,
&
1\leq t<N_1,\\
\dfrac{1}{k},
&
N_k\leq t<N_{k+1},
\qquad k\geq 1.
\end{cases}
\end{align}
Then $\varepsilon_t\downarrow 0$.

Moreover, outside a $P_z$-null set, for all sufficiently large $k$ and every $t$ such that $N_k\leq t<N_{k+1}$,
\begin{align}
\ell_t
\leq
\sup_{s\geq N_k}\ell_s
=
R_{N_k}
\leq
\frac{1}{k}
=
\varepsilon_t.
\end{align}
Consequently, $\ell_t \leq \varepsilon_t$ eventually $P_{z}$-almost surely.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:Egorov}]
For each $T\in\mathbb N$, define
\begin{align*}
    \Omega_T
    :=
    \left\{
    \omega \in (\mathbb A \times \mathbb Y)^{\mathbb N}
    :
    |\ell_t^i(\omega)|
    \leq \varepsilon'_t
    \quad
    \forall i,\ \forall t\geq T
    \right\}.
\end{align*}
The sequence $(\Omega_T)_{T\geq 1}$ is increasing, since
$\Omega_T\subseteq\Omega_{T+1}$, and, by definition of $\Omega$,
\begin{align*}
    \Omega
    =
    \bigcup_{T=1}^{\infty}\Omega_T.
\end{align*}
Hence, by continuity of probability from below,
\begin{align*}
    \lim_{T\to\infty}
    \mathbf P_{z^\infty}(\Omega_T)
    &=
    \mathbf P_{z^\infty}
    \left(
    \bigcup_{T=1}^{\infty}\Omega_T
    \right) \\
    &=
    \mathbf P_{z^\infty}(\Omega)
    =1.
\end{align*}
Therefore, for every $\delta>0$, there exists a deterministic
$T(\delta)\in\mathbb N$ such that
\begin{align*}
    \mathbf P_{z^\infty}
    \left(
    |\ell_t^i|
    \leq \varepsilon'_t
    \quad
    \forall i,\ \forall t\geq T(\delta)
    \right)
    =
    \mathbf P_{z^\infty}(\Omega_{T(\delta)})
    \geq 1-\delta.
\end{align*}
\end{proof}

\subsection{Demian: Lemma \ref{lemm:Berk-selected} and proof}


Let \(I\) be a finite set of players. For each \(i\in I\), let
\(A_i\) denote player \(i\)'s action space and let \(Y_i\) denote her
consequence space. Define
\[
A:=\prod_{i\in I}A_i,
\qquad
Y:=\prod_{i\in I}Y_i.
\]
At each date \(t=1,2,\ldots\), let
\[
a_t=(a_t^i)_{i\in I}\in A,
\qquad
y_t=(y_t^i)_{i\in I}\in Y,
\qquad
I_t=(I_t^i)_{i\in I}\in\{0,1\}^{|I|},
\]
where \(I_t^i=1\) indicates that player \(i\) samples at date \(t\).

We allow players to randomize both their action and their sampling
decision. For each \(i\in I\), let
\[
\varepsilon^i=(\varepsilon_t^i)_{t\geq 1}
\qquad\text{and}\qquad
U^i=(U_t^i)_{t\geq 1}
\]
denote, respectively, player \(i\)'s private action and sampling
randomization processes. These random variables are observed only by
player \(i\). The joint processes
\[
\varepsilon=(\varepsilon_t)_{t\geq 1},
\qquad
U=(U_t)_{t\geq 1},
\]
where
\[
\varepsilon_t=(\varepsilon_t^i)_{i\in I},
\qquad
U_t=(U_t^i)_{i\in I},
\]
are exogenous. Their joint law may otherwise allow arbitrary dependence
across players and over time.

Player \(i\) always observes her own action. By contrast, she observes
the opponents' action profile and her own consequence at date \(t\)
only if she samples. To formalize this, let
\(\partial_i\notin A_{-i}\times Y_i\) be a cemetery value and define
\[
Z_t^i
:=
\begin{cases}
(a_t^{-i},y_t^i), & \text{if } I_t^i=1,\\
\partial_i,       & \text{if } I_t^i=0.
\end{cases}
\]
Thus, \(Z_t^i\) records precisely the information acquired by player
\(i\) through sampling at date \(t\).

For every \(i\in I\), let the initial information sigma-field be
trivial:
\[
\mathcal S_0^i:=\{\varnothing,\Omega\}.
\]
Player \(i\)'s information after date \(t\) is defined recursively by
\[
\mathcal S_t^i
:=
\mathcal S_{t-1}^i
\vee
\sigma\left(
\varepsilon_t^i,
U_t^i,
a_t^i,
I_t^i,
Z_t^i
\right).
\]
Consequently, \(\mathcal S_t^i\) contains player \(i\)'s own action
history and private randomization history, as well as the opponents'
actions and own consequences observed at the dates at which she
sampled.

At the beginning of date \(t\), player \(i\) observes the private shock
\(\varepsilon_t^i\) and chooses her action. Define the pre-action
information sigma-field
\[
\mathcal A_t^i
:=
\mathcal S_{t-1}^i
\vee
\sigma(\varepsilon_t^i).
\]
We require
\[
a_t^i
\quad\text{to be}\quad
\mathcal A_t^i\text{-measurable}.
\]
Thus, player \(i\)'s action may depend arbitrarily on her information
through date \(t-1\) and on her current private action shock.

After choosing \(a_t^i\), player \(i\) observes the private sampling
shock \(U_t^i\) and decides whether to sample. Define the pre-sampling
information sigma-field
\[
\mathcal P_t^i
:=
\mathcal S_{t-1}^i
\vee
\sigma\left(
\varepsilon_t^i,
a_t^i,
U_t^i
\right).
\]
We require
\[
I_t^i
\quad\text{to be}\quad
\mathcal P_t^i\text{-measurable}.
\]
In particular, the decision to sample may depend arbitrarily on
player \(i\)'s previously observed information, her current action,
and her private sampling shock. It cannot depend on \(a_t^{-i}\) or
\(y_t^i\), since these variables are revealed to player \(i\) only
after she decides to sample.

Once the action profile \(a_t\) and the sampling decisions \(I_t\)
have been determined, the consequence \(y_t\) is generated according
to the true transition kernel \(Q\). Let
\[
\mathcal F_t^{-}
:=
\sigma\left(
y^{t-1},
a^t,
I^t,
\varepsilon^t,
U^t
\right)
\]
denote the full pre-consequence sigma-field, where, for example,
\(a^t=(a_1,\ldots,a_t)\). We require that, for every measurable
\(B\subseteq Y\),
\[
\Pr\left(
y_t\in B
\,\middle|\,
\mathcal F_t^{-}
\right)
=
Q\left(
B\mid y_{t-1},a_t
\right)
\qquad\text{a.s.}
\]
Equivalently,
\[
y_t\mid\mathcal F_t^{-}
\sim
Q(\,\cdot\mid y_{t-1},a_t).
\]
Thus, conditional on \((y_{t-1},a_t)\), neither the sampling decisions
nor the private randomization shocks have any direct incidence on the
law of \(y_t\).

The within-period timing can therefore be summarized as
\[
\varepsilon_t^i
\longrightarrow
a_t^i
\longrightarrow
U_t^i
\longrightarrow
I_t^i
\longrightarrow
y_t
\longrightarrow
Z_t^i.
\]

Finally, we require every player to accumulate an unbounded number of
sampled observations. That is, defining
\[
N_t^i:=\sum_{\tau=1}^t I_\tau^i,
\]
we impose
\[
N_t^i\longrightarrow\infty
\qquad\text{a.s.}
\]
for every \(i\in I\).


\subsection{NEW SAMPLE Proof of Theorem \ref{theo:sustain-self-justified}}

\begin{proof}
Fix $\gamma\in(1/2,1)$. We proceed in five steps.

\medskip
\noindent
\emph{Step 1: Construct a target path with sufficiently large sampling reservoirs.}

Since $S$ is compact, for every integer $m\geq1$ there exists a finite $1/m$-net $F_m\subseteq S$. Fix one such net for each $m$, and let
\[
\kappa_m:=|F_m|<\infty.
\]

Choose a number $q$ satisfying
\[
1<q<\frac1\gamma.
\]
Starting from an integer $r_1$ to be chosen sufficiently large, define recursively
\[
r_{n+1}:=\lceil r_n^q\rceil.
\]
Thus $r_n\to\infty$, and, for $r_1\geq1$,
\[
r_n^q\leq r_{n+1}\leq 2r_n^q.
\]

For each $n\geq1$, define
\[
A_n:=\frac14 r_n^{1/\gamma-q}.
\]
Because $q<1/\gamma$ and $r_n\to\infty$, we have $A_n\to\infty$. Choose $r_1$ large enough that $A_1\geq\kappa_1$. For each $n\geq1$, let
\[
m_{n+1}
:=
\max\left\{
m\in\{1,\ldots,n+1\}:\kappa_m\leq A_n
\right\},
\]
and set
\[
E_{n+1}:=F_{m_{n+1}}.
\]
For the first block, set $E_1:=F_1$.

The mesh of $E_n$ converges to zero. Indeed, fix any $m$. Since $A_n\to\infty$ and $\kappa_m<\infty$, for all sufficiently large $n$ we have $A_n\geq\kappa_m$; and once also $n+1\geq m$, the definition of $m_{n+1}$ gives $m_{n+1}\geq m$. Hence $m_n\to\infty$, and therefore
\[
\operatorname{mesh}(E_n)\leq\frac1{m_n}\to0.
\]

Let
\[
K_n:=|E_n|.
\]
By construction, for every $n\geq1$,
\[
K_{n+1}\leq A_n
=
\frac14 r_n^{1/\gamma-q}.
\]
Let $B_n$ be a finite block that lists every element of $E_n$ exactly $r_n$ times, in any order. Thus
\[
|B_n|=K_nr_n.
\]
For $n\geq1$, using $r_{n+1}\leq2r_n^q$,
\[
|B_{n+1}|
=
K_{n+1}r_{n+1}
\leq
\frac14 r_n^{1/\gamma-q}\,2r_n^q
=
\frac12 r_n^{1/\gamma}.
\tag{A.1}
\]

The same construction also gives
\[
\frac{K_n}{r_n}\to0.
\]
Indeed, for $n\geq2$,
\[
\frac{K_n}{r_n}
\leq
\frac{\frac14 r_{n-1}^{1/\gamma-q}}{r_{n-1}^q}
=
\frac14 r_{n-1}^{1/\gamma-2q}.
\]
Since $\gamma>1/2$, we have $1/\gamma<2$, while $q>1$, and hence
\[
\frac1\gamma-2q<0.
\]
As $r_{n-1}\to\infty$, it follows that $K_n/r_n\to0$.

Let
\[
T_n:=\sum_{m=1}^n |B_m|
\]
denote the final date of block $B_n$. We next show that, for all sufficiently large $n$,
\[
T_{n+1}\leq r_n^{1/\gamma}.
\tag{A.2}
\]
By (A.1), for every sufficiently large $n$,
\[
T_n
\leq
|B_1|+\frac12\sum_{m=1}^{n-1}r_m^{1/\gamma}.
\]
Since $(r_m)_m$ is increasing,
\[
T_n
\leq
|B_1|+\frac{n-1}{2}r_{n-1}^{1/\gamma}.
\]
Moreover, $r_n\geq r_{n-1}^q$, so
\[
\frac{T_n}{r_n^{1/\gamma}}
\leq
\frac{|B_1|}{r_n^{1/\gamma}}
+
\frac{n-1}{2}\,
r_{n-1}^{-(q-1)/\gamma}.
\]
The first term converges to zero. The second also converges to zero because $q>1$ and the recursion $r_n\geq r_{n-1}^q$ implies that $r_n$ grows faster than exponentially in $n$. Hence, for all sufficiently large $n$,
\[
T_n\leq\frac12 r_n^{1/\gamma}.
\]
Combining this with (A.1) yields
\[
T_{n+1}
=
T_n+|B_{n+1}|
\leq
\frac12r_n^{1/\gamma}
+
\frac12r_n^{1/\gamma}
=
r_n^{1/\gamma},
\]
which proves (A.2).

Finally, let $z^\infty=(z_t)_{t\geq1}$ be the deterministic path obtained by concatenating the blocks
\[
B_1,B_2,\ldots.
\]
Then $z_t\in S$ for every $t$, and
\[
L(z^\infty)=S.
\]
Indeed, since $S$ is compact and therefore closed, every limit point of $z^\infty$ belongs to $S$. Conversely, fix $a\in S$. For each $n$, choose $e_n\in E_n$ with
\[
d(e_n,a)\leq\operatorname{mesh}(E_n).
\]
Since $\operatorname{mesh}(E_n)\to0$, we have $e_n\to a$. Each $e_n$ appears in block $B_n$, so there exists a date $t_n\in B_n$ such that $z_{t_n}=e_n$. Since $t_n\to\infty$, this gives a subsequence of the target path converging to $a$. Hence $a\in L(z^\infty)$.

\medskip
\noindent
\emph{MORE TRANSPARENT PROOF? Step 1: Construct a target path with sufficiently large sampling reservoirs.}

Fix $\gamma\in(1/2,1)$. We first record an elementary consequence of compactness that will be useful in constructing the blocks. For a finite set $E\subseteq S$, let
\[
\operatorname{mesh}(E)
:=
\sup_{a\in S}\min_{e\in E}d(a,e).
\]
If $(b_n)_n$ is any sequence with $b_n\to\infty$, then there exist finite sets $E_n\subseteq S$ such that
\[
\operatorname{mesh}(E_n)\to0
\qquad\text{and}\qquad
|E_n|\leq b_n
\]
for all sufficiently large $n$. Indeed, if $N(S,\delta)$ denotes the minimum cardinality of a finite $\delta$-net of $S$, compactness implies $N(S,1/m)<\infty$ for every integer $m\geq1$. Since $b_n\to\infty$, we can choose integers $m_n\to\infty$ sufficiently slowly that
$N(S,1/m_n)\leq b_n$ for all sufficiently large $n$, and then take $E_n$ to be a $1/m_n$-net of minimum cardinality.

Choose a number $q$ satisfying
\[
1<q<\frac1\gamma,
\]
and, starting from some integer $r_1\geq2$, define recursively
\[
r_{n+1}:=\lceil r_n^q\rceil.
\]
Then $r_n\to\infty$, and
\[
r_n^q\leq r_{n+1}\leq 2r_n^q.
\]
Moreover, iterating the lower bound gives
\[
r_n\geq r_1^{q^{\,n-1}},
\]
so $(r_n)_n$ grows faster than exponentially.

For $n\geq1$, set
\[
b_{n+1}:=\frac14 r_n^{1/\gamma-q}.
\]
Because $q<1/\gamma$, we have $1/\gamma-q>0$, and therefore
$b_n\to\infty$. Apply the compactness observation above to choose finite
sets $E_n\subseteq S$ such that, writing $K_n:=|E_n|$,
\[
\operatorname{mesh}(E_n)\to0
\qquad\text{and}\qquad
K_{n+1}\leq\frac14 r_n^{1/\gamma-q}
\]
for all sufficiently large $n$.

Let $B_n$ be a finite block that lists every element of $E_n$ exactly
$r_n$ times, in any order. Thus
\[
|B_n|=K_nr_n.
\]
For all sufficiently large $n$,
\[
|B_{n+1}|
=
K_{n+1}r_{n+1}
\leq
\frac14 r_n^{1/\gamma-q}\,2r_n^q
=
\frac12 r_n^{1/\gamma}.
\tag{A.1}
\]

We will also need the empirical distributions constructed from block
$B_n$ to approximate arbitrary distributions on $E_n$. For this it is
enough that $K_n/r_n\to0$. The preceding bounds imply, for all
sufficiently large $n$,
\[
\frac{K_{n+1}}{r_{n+1}}
\leq
\frac{\frac14r_n^{1/\gamma-q}}{r_n^q}
=
\frac14r_n^{1/\gamma-2q}.
\]
Since $\gamma>1/2$ implies $1/\gamma<2$, while $q>1$, we have
$1/\gamma-2q<0$. Hence
\[
\frac{K_n}{r_n}\to0.
\tag{A.2}
\]

Let
\[
T_n:=\sum_{m=1}^n|B_m|
\]
denote the last date of block $B_n$. We next show that
\[
T_{n+1}\leq r_n^{1/\gamma}
\tag{A.3}
\]
for all sufficiently large $n$. By (A.1), there is an integer $n_0$
such that, for $n\geq n_0$,
\[
T_n
\leq
T_{n_0}
+
\frac12\sum_{m=n_0}^{n-1}r_m^{1/\gamma}.
\]
Since $(r_m)_m$ is increasing,
\[
T_n
\leq
T_{n_0}
+
\frac n2 r_{n-1}^{1/\gamma}.
\]
Using $r_n\geq r_{n-1}^q$,
\[
\frac{T_n}{r_n^{1/\gamma}}
\leq
\frac{T_{n_0}}{r_n^{1/\gamma}}
+
\frac n2 r_{n-1}^{-(q-1)/\gamma}.
\]
The first term converges to zero. For the second, the bound
$r_{n-1}\geq r_1^{q^{\,n-2}}$ gives
\[
n r_{n-1}^{-(q-1)/\gamma}
\leq
n r_1^{-q^{\,n-2}(q-1)/\gamma}
\to0.
\]
Therefore
\[
\frac{T_n}{r_n^{1/\gamma}}\to0.
\]
In particular, for all sufficiently large $n$,
\[
T_n\leq\frac12r_n^{1/\gamma}.
\]
Combining this with (A.1) yields
\[
T_{n+1}
=
T_n+|B_{n+1}|
\leq
\frac12r_n^{1/\gamma}
+
\frac12r_n^{1/\gamma}
=
r_n^{1/\gamma},
\]
which proves (A.3).

Finally, let $z^\infty=(z_t)_{t\geq1}$ be the deterministic path obtained
by concatenating $B_1,B_2,\ldots$. Then $z_t\in S$ for every $t$, and
\[
L(z^\infty)=S.
\]
Indeed, since $S$ is compact and therefore closed, every limit point of
$z^\infty$ belongs to $S$. Conversely, fix $a\in S$. For each $n$,
choose $e_n\in E_n$ satisfying
\[
d(e_n,a)\leq\operatorname{mesh}(E_n).
\]
Since $\operatorname{mesh}(E_n)\to0$, we have $e_n\to a$. Each $e_n$
appears in block $B_n$, so there is a date $t_n\in B_n$ such that
$z_{t_n}=e_n$. Since $t_n\to\infty$, $z_{t_n}\to a$, and hence
$a\in L(z^\infty)$. Thus $L(z^\infty)=S$.


\medskip
\noindent
\emph{Step 2: Choose supporting distributions.}

Fix a date $t$ and a player $i$. Since $z_t\in S$ and $S\subseteq\Gamma(S)$, the definition of $\Gamma$ implies that there exists a distribution $\rho_t^i\in\Delta S$ such that
\[
z_t^i
\in
F^i\left(
\delta_{\theta^i(\rho_t^i)},
(\rho_t^i)^{-i}
\right).
\]
Thus $\rho_t^i$ is a distribution over $S$ that justifies the target action $z_t^i$ for player $i$. Fix one such distribution $\rho_t^i$ for every pair $(t,i)$.


\medskip
\noindent
\emph{Step 3: Construct selected samples that approximate the supporting distributions.}

We now construct the entire sampling array $W$ deterministically. Since the target path $(z_t)_t$ and the supporting distributions $(\rho_t^i)_{t,i}$ were fixed in Steps 1 and 2, all selected dates used below can be chosen ex ante. In particular, the resulting sampling scheme satisfies the timing requirement that the future use of observation $\tau$ be determined before its consequence is realized.

Fix $n\geq1$, a date $t$ in block $B_{n+1}$, and a player $i$. We use block $B_n$ as the reservoir from which player $i$'s date-$t$ sample is selected. Let
\[
\delta_n:=\operatorname{mesh}(E_n),
\]
so that $\delta_n\to0$. Choose a measurable nearest-net projection $p_n:S\to E_n$ satisfying
\[
d(a,p_n(a))\leq\delta_n
\qquad\text{for every }a\in S.
\]
Let $\bar\rho_t^i\in\Delta E_n$ be the distribution obtained by moving the mass of $\rho_t^i$ to the corresponding net points:
\[
\bar\rho_t^i(e)
=
\rho_t^i\bigl(\{a\in S:p_n(a)=e\}\bigr),
\qquad e\in E_n.
\]

For each $e\in E_n$, write $w_e:=\bar\rho_t^i(e)$. Since $\sum_{e\in E_n}w_e=1$, there exist nonnegative integers $(N_e)_{e\in E_n}$ such that
\[
\sum_{e\in E_n}N_e=r_n
\qquad\text{and}\qquad
\left|\frac{N_e}{r_n}-w_e\right|\leq\frac1{r_n}
\quad\text{for every }e\in E_n.
\]
For example, one may take $N_e=\lfloor r_nw_e\rfloor$ and allocate the remaining observations according to the largest fractional remainders.

By construction, block $B_n$ contains exactly $r_n$ dates at which the target action is equal to each $e\in E_n$. Hence we can choose, for each $e$, exactly $N_e$ such dates and let $H_t^i$ be their union. Thus
\[
|H_t^i|=r_n
\]
and, along the target path,
\[
\hat\sigma_t^i
=
\sum_{e\in E_n}\frac{N_e}{r_n}\delta_e.
\]

Let $D:=\operatorname{diam}(S)$. Since both $\hat\sigma_t^i$ and $\bar\rho_t^i$ are supported on $E_n$,
\[
\|\hat\sigma_t^i-\bar\rho_t^i\|_{\mathrm{TV}}
\leq
\frac{|E_n|}{2r_n}.
\]
Hence their $1$-Wasserstein distance satisfies
\[
d_{\Delta}(\hat\sigma_t^i,\bar\rho_t^i)
\leq
\frac{D|E_n|}{2r_n},
\]
where here $d_{\Delta}$ denotes the $1$-Wasserstein metric on $\Delta S$. Also, because $p_n$ moves every point by at most $\delta_n$,
\[
d_{\Delta}(\bar\rho_t^i,\rho_t^i)\leq\delta_n.
\]
Therefore
\[
d_{\Delta}(\hat\sigma_t^i,\rho_t^i)
\leq
\delta_n+\frac{D|E_n|}{2r_n}.
\]
By Step 1, $\delta_n\to0$ and $|E_n|/r_n\to0$. Hence, uniformly over dates $t$ in block $B_{n+1}$ and players $i$,
\[
d_{\Delta}(\hat\sigma_t^i,\rho_t^i)\to0.
\]

It remains to verify the sample-growth condition. If $t$ belongs to block $B_{n+1}$, then $t\leq T_{n+1}$. Step 1 gives, for all sufficiently large $n$,
\[
T_{n+1}\leq r_n^{1/\gamma}.
\]
Therefore
\[
|H_t^i|
=
r_n
\geq
t^\gamma.
\]
Thus the growth condition holds with $c_i=1$ and the common exponent $\gamma>1/2$, for every player $i$ and all sufficiently large dates.

For dates in the first block, choose $H_t^i$ arbitrarily. Having chosen all sets $H_t^i$ above, define the sampling array by
\[
W_{\tau,t}^i
=
\mathbf 1\{\tau\in H_t^i\},
\qquad \tau<t.
\]
Since all the sets $H_t^i$ were chosen deterministically from the target path and the supporting distributions fixed in advance, the entire array $W$ is deterministic ex ante. Hence it defines an admissible sampling scheme not only along the target path but after every possible realized history.

Finally, set
\[
\tilde\sigma_t^{-i}
=
(\hat\sigma_t^i)^{-i}.
\]
Thus forecast consistency holds automatically.

\medskip
\noindent
\emph{Step 4: Show that the target actions are asymptotically optimal along the target path.}


Let $\mathbf P^z$ denote the probability law generated when the action rule is degenerate at the target path $z^\infty$ and the sampling array is the deterministic array constructed in Step 3. As shown in Step 3, this array satisfies $|H_t^i|\geq t^\gamma$ for every player $i$ and all sufficiently large $t$, and, being deterministic ex ante, it also satisfies the sampling-timing requirement. Hence the target-path process is an admissible learning process. Let $\mu_t^{i,z}$, $\hat\sigma_t^{i,z}$, and $\tilde\sigma_t^{-i,z}$ denote player $i$'s posterior, selected empirical distribution, and forecast under this process.

For each player $i$, define the payoff loss from playing the target action $z_t^i$ at date $t$ by
\[
\ell_t^i
:=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}
U^i(x^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i)
-
\int_{\Theta^i}
U^i(z_t^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i),
\]
and let $\ell_t:=\max_i\ell_t^i$. We claim that
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely}.
\]

Let $\Omega^\ast$ be the probability-one event on which Lemma~\ref{lemm:Berk-selected} holds for every player under the target-path process. Suppose, toward a contradiction, that $\ell_t\not\to0$ on a set of positive $\mathbf P^z$-probability. Since the set of players is finite, there exist a player $i$, a number $\eta>0$, and an event $A\subseteq\Omega^\ast$ with $\mathbf P^z(A)>0$ such that
\[
\limsup_{t\to\infty}\ell_t^i(\omega)>\eta
\qquad\text{for every }\omega\in A.
\]

Fix $\omega\in A$. Then there is a subsequence $(t_m)_m$ such that
\[
\ell_{t_m}^i(\omega)\geq\eta
\qquad\text{for every }m.
\]
By compactness, passing to a further subsequence if necessary, we may assume
\[
z_{t_m}\to a\in S,
\qquad
\rho_{t_m}^i\Rightarrow\rho^i\in\Delta S,
\qquad
\mu_{t_m}^{i,z}(\omega)\Rightarrow\mu^i.
\]
By Step 3,
\[
d_\Delta(\hat\sigma_{t_m}^{i,z},\rho_{t_m}^i)\to0,
\]
and hence
\[
\hat\sigma_{t_m}^{i,z}\Rightarrow\rho^i
\qquad\text{and}\qquad
\tilde\sigma_{t_m}^{-i,z}
\Rightarrow
(\rho^i)^{-i}.
\]
Since $\omega\in\Omega^\ast$, Lemma~\ref{lemm:Berk-selected} implies
\[
\mu^i\in\Delta\Theta^{m,i}(\rho^i).
\]
By identification,
\[
\mu^i=\delta_{\theta^i(\rho^i)}.
\]

On the other hand, by the choice of $\rho_{t_m}^i$ in Step 2,
\[
z_{t_m}^i
\in
F^i\left(
\delta_{\theta^i(\rho_{t_m}^i)},
(\rho_{t_m}^i)^{-i}
\right)
\qquad\text{for every }m.
\]
Identification and Lemma~\ref{lem:basic-properties}(iv) imply that
$\rho\mapsto\theta^i(\rho)$ is continuous. Hence
\[
\delta_{\theta^i(\rho_{t_m}^i)}
\Rightarrow
\delta_{\theta^i(\rho^i)}.
\]
Together with $z_{t_m}^i\to a^i$ and
$(\rho_{t_m}^i)^{-i}\Rightarrow(\rho^i)^{-i}$, the closed-graph property of $F^i$ implies
\[
a^i
\in
F^i\left(
\delta_{\theta^i(\rho^i)},
(\rho^i)^{-i}
\right).
\]

By continuity of the value function and expected payoffs, the payoff loss from $z_{t_m}^i$ under
$(\mu_{t_m}^{i,z},\tilde\sigma_{t_m}^{-i,z})$
converges to the payoff loss from $a^i$ under
$\bigl(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\bigr)$.
The latter loss is zero because
\[
a^i
\in
F^i\left(
\delta_{\theta^i(\rho^i)},
(\rho^i)^{-i}
\right).
\]
Therefore
\[
\ell_{t_m}^i(\omega)\to0,
\]
contradicting $\ell_{t_m}^i(\omega)\geq\eta$ for every $m$. Hence
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely}.
\]

\medskip
\noindent
\emph{Step 5: Choose tolerances and define the actual process.}

Since $\ell_t\to0$ $\mathbf P^z$-almost surely, Lemma~\ref{lem:deterministic-tolerance} implies that there exists a deterministic sequence $\varepsilon_t\downarrow0$ such that
\[
\mathbf P^z\!\left(
\ell_t\leq\varepsilon_t
\text{ for every }t
\right)>1-\alpha.
\]
Let
\[
G
:=
\left\{
\ell_t\leq\varepsilon_t
\text{ for every }t
\right\},
\]
so that $\mathbf P^z(G)>1-\alpha$.

We now define the action rule of the actual process. At date $t$, given the posterior $\mu_t^i$ and forecast $\tilde\sigma_t^{-i}$ induced by the deterministic sampling array constructed in Step 3, player $i$ chooses the target action $z_t^i$ whenever
\[
z_t^i\in
F_{\varepsilon_t}^i(\mu_t^i,\tilde\sigma_t^{-i});
\]
otherwise, she chooses an arbitrary exact best response in
$F^i(\mu_t^i,\tilde\sigma_t^{-i})$, which is nonempty by Lemma~\ref{lem:basic-properties}(ii), using any fixed measurable selection. Hence, at every history,
\[
a_t^i\in
F_{\varepsilon_t}^i(\mu_t^i,\tilde\sigma_t^{-i}),
\]
so the resulting action rule is asymptotically myopic.

Together with the full-support priors, the deterministic sampling array from Step 3, Bayesian updating, and the empirical forecasts
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i},
\]
this action rule defines an admissible learning process with consistent forecasts.

For each $T\geq1$, let
\[
F_T
:=
\{a_t=z_t\text{ for every }t\leq T\}
\]
and
\[
G_T
:=
\{\ell_t\leq\varepsilon_t\text{ for every }t\leq T\}.
\]
We claim that, for every finite $T$, whenever the realized consequence history belongs to $G_T$, the actual process follows the target path through date $T$.

The claim follows by induction. At date $1$, the actual and target histories are both empty, so the posterior and forecast coincide with those used to compute $\ell_1$. Since $G_T$ implies $\ell_1\leq\varepsilon_1$, the target action $z_1^i$ is $\varepsilon_1$-optimal for every player $i$, and therefore the action rule prescribes $z_1$.

Now suppose that $a_s=z_s$ for every $s<t$, where $t\leq T$. Because the sampling array $W$ is deterministic ex ante, the actual process and the target-path process use exactly the same selected dates at date $t$. Since the realized action history also coincides with the target history through date $t-1$, the selected observations, posterior beliefs, and forecasts coincide with those used to compute $\ell_t$. Since $G_T$ implies $\ell_t\leq\varepsilon_t$, the target action $z_t^i$ is $\varepsilon_t$-optimal for every player $i$. Hence the action rule prescribes $z_t$, completing the induction.

It remains to compare probabilities under the actual process and the target-path process. Up to any date at which the actual action path coincides with the target path, both processes use the same deterministic sampling array and the same consequence kernel $Q(\cdot\mid z_t)$. Therefore, for every finite $T$,
\[
\mathbf P(F_T)\geq \mathbf P^z(G_T).
\]
The events $(F_T)_T$ are decreasing, with
\[
\bigcap_{T=1}^\infty F_T
=
\{a_t=z_t\text{ for every }t\},
\]
and $(G_T)_T$ decreases to $G$. Hence, by continuity of probability from above,
\[
\mathbf P\!\left(\bigcap_{T=1}^\infty F_T\right)
=
\lim_{T\to\infty}\mathbf P(F_T)
\geq
\lim_{T\to\infty}\mathbf P^z(G_T)
=
\mathbf P^z(G)
>
1-\alpha.
\]
On $\bigcap_TF_T$, the realized action path coincides with the target path $z^\infty$, so
\[
L(a^\infty)=L(z^\infty)=S.
\]
Therefore,
\[
\mathbf P\bigl(L(a^\infty)=S\bigr)>1-\alpha.
\]
\end{proof}


\subsection{OLD Proof of Theorem \ref{theo:sustain-self-justified}}

\begin{proof}
Let \(d_\Delta=W_1\), which metrizes weak convergence on \(\Delta\mathbb A\). We proceed in five steps.

Step 1: Construct a target path. Since \(S\) is nonempty and compact, for each \(n\geq1\) choose a finite \(1/n\)-net \(E_n\subseteq S\). Choose integers \(r_n\to\infty\) such that \(|E_n|/r_n\to0\). Let \(B_n\) be a finite block that lists each element of \(E_n\) exactly \(r_n\) times, in any order, and let \(z^\infty=(z_t)_{t\geq1}\) be the deterministic path obtained by concatenating the blocks \(B_1,B_2,\ldots\). Then \(z_t\in S\) for every \(t\). Moreover, \(L(z^\infty)=S\). Indeed, since \(z_t\in S\) for all \(t\) and \(S\) is closed, every limit point of \(z^\infty\) belongs to \(S\). Conversely, if \(a\in S\), then for each \(n\) there is \(e_n\in E_n\) with \(d(e_n,a)\leq1/n\), and \(e_n\) appears in block \(B_n\). Thus some subsequence of \(z^\infty\) converges to \(a\), so \(a\in L(z^\infty)\).

Step 2: Choose supporting distributions. Fix a date \(t\) and a player \(i\). Since \(z_t\in S\) and \(S\subseteq\Gamma(S)\), the definition of \(\Gamma\) implies that there exists \(\rho_t^i\in\Delta S\) such that, under identification,
\[
z_t^i\in F^i\left(\delta_{\theta^i(\rho_t^i)},(\rho_t^i)^{-i}\right).
\]
Thus \(\rho_t^i\) is a selected-sample distribution that justifies the target action \(z_t^i\).


Step 3: Define selected samples that approximate the supporting distributions. We now define the selected-sample rule. The rule is specified after every past action history, but it is constructed so that, along histories whose past action path coincides with the target path, selected empirical distributions approximate the supporting distributions chosen in Step 2.

Suppose that the past action path coincides with the target path and that date \(t\) belongs to block \(B_{n+1}\). We use the previous block \(B_n\) as the reservoir of observations from which player \(i\)'s selected sample is drawn. Let \(p_n:S\to E_n\) be a measurable nearest-net projection, so that \(p_n(a)\in E_n\) and \(d(a,p_n(a))\leq 1/n\) for every \(a\in S\). Let \(\bar\rho_t^i\in\Delta E_n\) be the distribution obtained by moving the mass of \(\rho_t^i\) to the nearest net points: for each \(e\in E_n\),
\[
\bar\rho_t^i(e)
=
\rho_t^i\bigl(\{a\in S:p_n(a)=e\}\bigr).
\]
Thus \(\bar\rho_t^i\) is the finite-net approximation of \(\rho_t^i\).

We next choose selected dates from block \(B_n\). For each \(e\in E_n\), let
\[
w_e:=\bar\rho_t^i(e).
\]
Since \(\sum_{e\in E_n}w_e=1\), we can choose nonnegative integers \((N_e)_{e\in E_n}\) such that
\[
\sum_{e\in E_n}N_e=r_n
\qquad\text{and}\qquad
\left|\frac{N_e}{r_n}-w_e\right|\leq \frac{1}{r_n}
\quad\text{for every }e\in E_n.
\]
For example, take \(N_e=\lfloor r_n w_e\rfloor\) and allocate the remaining observations to the largest fractional remainders. Because block \(B_n\) contains \(r_n\) copies of each \(e\in E_n\), we can choose \(N_e\) dates in block \(B_n\) at which the target path played \(e\). Let \(H_t^i\) be the union of these selected dates. Then \(|H_t^i|=r_n\), and the selected empirical distribution is
\[
\hat\sigma_t^i
=
\sum_{e\in E_n}\frac{N_e}{r_n}\delta_e.
\]
Therefore,
\[
\left\|\hat\sigma_t^i-\bar\rho_t^i\right\|_{\mathrm{TV}}
\leq
\frac{|E_n|}{2r_n}.
\]
Let \(D=\operatorname{diam}(S)\). Since \(W_1(\nu,\nu')\leq D\|\nu-\nu'\|_{\mathrm{TV}}\) for distributions supported on \(S\),
\[
W_1(\hat\sigma_t^i,\bar\rho_t^i)
\leq
\frac{D|E_n|}{2r_n}.
\]
Also, since \(p_n\) moves every point of \(S\) by at most \(1/n\),
\[
W_1(\bar\rho_t^i,\rho_t^i)\leq \frac{1}{n}.
\]
Hence, by the triangle inequality,
\[
W_1(\hat\sigma_t^i,\rho_t^i)
\leq
\frac{1}{n}
+
\frac{D|E_n|}{2r_n}.
\]
Because \(r_n\to\infty\) and \(|E_n|/r_n\to0\), the right-hand side converges to zero. Thus, along histories whose past action path coincides with the target path,
\[
W_1(\hat\sigma_t^i,\rho_t^i)\to0
\qquad\text{for every player }i.
\]

For dates in the first block, define \(H_t^i\) arbitrarily. At histories whose past action path does not coincide with the target path, define \(H_t^i=\{1,\ldots,t-1\}\). Thus the selected-sample rule is defined after every possible action history. Moreover, along every infinite action history, the selected-sample size diverges.

Finally, forecasts are empirical forecasts from the selected sample:
\[
\tilde\sigma_t^{-i}=(\hat\sigma_t^i)^{-i}.
\]



Step 4: Show that the target actions are asymptotically optimal along the target path. Let \(\mathbf P^z\) denote the probability law over consequence paths induced when the action path is fixed exogenously at \(z^\infty\). Let \(\mu_t^{i,z}\), \(\hat\sigma_t^{i,z}\), and \(\tilde\sigma_t^{-i,z}\) denote the posterior, selected empirical distribution, and forecast generated along this target path. Define the payoff loss from the target action by
\[
\ell_t^i
=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}U^i(x^i,\tilde\sigma_t^{-i,z},\theta^i)\,\mu_t^{i,z}(d\theta^i)
-
\int_{\Theta^i}U^i(z_t^i,\tilde\sigma_t^{-i,z},\theta^i)\,\mu_t^{i,z}(d\theta^i),
\]
and let \(\ell_t=\max_i\ell_t^i\). We claim that
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely}.
\]

We prove the claim by contradiction. Let \(\Omega^\ast\) be the probability-one event on which the conclusion of Lemma \ref{lemm:Berk-selected} holds along the target path. Suppose that \(\ell_t\not\to0\) with positive \(\mathbf P^z\)-probability. Since the set of players is finite and \(\ell_t=\max_i\ell_t^i\), there exist a player \(i\), a number \(\eta>0\), and an event \(A\subseteq\Omega^\ast\) with \(\mathbf P^z(A)>0\) such that
\[
\limsup_{t\to\infty}\ell_t^i(\omega)>\eta
\qquad\text{for every }\omega\in A.
\]
Fix \(\omega\in A\). Then there is a subsequence \(t_m\to\infty\) such that
\[
\ell_{t_m}^i(\omega)\geq\eta
\qquad\text{for every }m.
\]
Passing to a further subsequence, compactness implies
\[
z_{t_m}\to a\in S,\qquad
\rho_{t_m}^i\Rightarrow \rho^i\in\Delta S,\qquad
\mu_{t_m}^{i,z}(\omega)\Rightarrow \mu^i.
\]
By Step 3, \(d_\Delta(\hat\sigma_{t_m}^{i,z},\rho_{t_m}^i)\to0\). Hence
\[
\hat\sigma_{t_m}^{i,z}\Rightarrow\rho^i
\qquad\text{and}\qquad
\tilde\sigma_{t_m}^{-i,z}\Rightarrow(\rho^i)^{-i}.
\]
Since \(\omega\in\Omega^\ast\), Lemma \ref{lemm:Berk-selected} implies that
\[
\mu^i\in\Delta\Theta^{m,i}(\rho^i).
\]
By identification,
\[
\mu^i=\delta_{\theta^i(\rho^i)}.
\]

Moreover, for every \(m\),
\[
z_{t_m}^i\in F^i\left(\delta_{\theta^i(\rho_{t_m}^i)},(\rho_{t_m}^i)^{-i}\right).
\]

By Lemma \ref{lem:basic-properties}(iv), identification implies that the map \(\rho\mapsto\theta^i(\rho)\) is continuous. Hence
\[
\delta_{\theta^i(\rho_{t_m}^i)}\Rightarrow\delta_{\theta^i(\rho^i)}.
\]
Also, \((\rho_{t_m}^i)^{-i}\Rightarrow(\rho^i)^{-i}\). Together with \(z_{t_m}^i\to a^i\), the closed graph property of \(F^i\), Lemma \ref{lem:basic-properties}(ii), implies
\[
a^i\in F^i\left(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\right).
\]

By Lemma \ref{lem:basic-properties}(i), the value function \(\bar V^i\) is continuous, and expected payoffs are continuous in the action, belief, and forecast. Therefore the payoff loss from \(z_{t_m}^i\) under \((\mu_{t_m}^{i,z},\tilde\sigma_{t_m}^{-i,z})\) converges to the payoff loss from \(a^i\) under \(\left(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\right)\). Since \(a^i\in F^i\left(\delta_{\theta^i(\rho^i)},(\rho^i)^{-i}\right)\), this limiting payoff loss is zero. Thus \(\ell_{t_m}^i(\omega)\to0\), contradicting \(\ell_{t_m}^i(\omega)\geq\eta\) for every \(m\). Therefore \(\ell_t\to0\), \(\mathbf P^z\)-almost surely.

Step 5: Choose tolerances and define the actual learning rule. Since \(\ell_t\to0\), \(\mathbf P^z\)-almost surely, and payoff losses are bounded by Lemma \ref{lem:basic-properties}(i), Lemma \ref{lem:deterministic-tolerance} implies that there exists a deterministic sequence \(\varepsilon_t\downarrow0\) such that
\[
\mathbf P^z\left(\ell_t\leq\varepsilon_t\text{ for every }t\right)>1-\alpha.
\]
Let
\[
G
=
\left\{
\ell_t\leq\varepsilon_t\text{ for every }t
\right\}.
\]
Thus \(\mathbf P^z(G)>1-\alpha\). For each \(T\), also define the finite-horizon event
\[
G_T
=
\left\{
\ell_t\leq\varepsilon_t\text{ for every }t\leq T
\right\}.
\]

We now define the actual action rule. At date \(t\), after player \(i\)'s selected sample, posterior \(\mu_t^i\), and forecast \(\tilde\sigma_t^{-i}\) have been computed, player \(i\) plays \(z_t^i\) if
\[
z_t^i\in F_{\varepsilon_t}^i(\mu_t^i,\tilde\sigma_t^{-i});
\]
otherwise she plays an arbitrary exact best response in \(F^i(\mu_t^i,\tilde\sigma_t^{-i})\), which is nonempty by Lemma \ref{lem:basic-properties}(ii). This rule is \(\varepsilon_t\)-optimal at every history, because it either chooses an \(\varepsilon_t\)-optimal target action or an exact best response.

Let
\[
F_T
=
\{a_t=z_t\text{ for every }t\leq T\}
\]
be the event that the realized action path follows the target path through date \(T\). We claim that, for every finite \(T\), the event \(G_T\) implies \(F_T\) in the following pathwise sense: along any consequence history for which the target-path losses satisfy \(\ell_t\leq\varepsilon_t\) for every \(t\leq T\), the actual learning rule prescribes the target action profile at every date \(t\leq T\).

The claim follows by induction. At date \(1\), the realized and target action histories are both empty and $\mu^{i,z}_{0} = \mu^{i}_{0}$ for all $i$. Since \(G_T\) implies that the target action \(z_1^i\) is \(\varepsilon_1\)-optimal for every player \(i\), the action rule prescribes \(z_1^i\) for every player, and hence \(a_1=z_1\). Now suppose that \(a_s=z_s\) for every \(s<t\), where \(t\leq T\). Then the past action path coincides with the target path through date \(t-1\). By construction of the selected-sample rule, each player selects the same dates as in the target-path calculation. Given the same realized consequences at those dates, player \(i\)'s selected sample, posterior, and forecast coincide with \(\hat\sigma_t^{i,z}\), \(\mu_t^{i,z}\), and \(\tilde\sigma_t^{-i,z}\). Since \(G_T\) implies \(\ell_t\leq\varepsilon_t\), the target action \(z_t^i\) is \(\varepsilon_t\)-optimal for every player \(i\). Therefore the action rule prescribes \(z_t^i\) for every player, so \(a_t=z_t\). This proves the induction step.

The same finite-horizon induction gives the probability comparison. Up to any date on which the realized action path coincides with the target path, the consequence kernels used by the actual process are exactly the consequence kernels used to define \(\mathbf P^z\). Hence, for every \(T\),
\[
\mathbf P(F_T)\geq \mathbf P^z(G_T).
\]
The events \(F_T\) are decreasing in \(T\), and \(\bigcap_T F_T\) is the event that the realized action path follows the target path at every date. Similarly, \(G_T\downarrow G\). Therefore, by continuity of probability from above,
\[
\mathbf P\left(\bigcap_{T=1}^\infty F_T\right)
=
\lim_{T\to\infty}\mathbf P(F_T)
\geq
\lim_{T\to\infty}\mathbf P^z(G_T)
=
\mathbf P^z(G)
>
1-\alpha.
\]
On \(\bigcap_T F_T\), the realized action path \(a^\infty\) coincides with the target path \(z^\infty\). Hence
\[
L(a^\infty)=L(z^\infty)=S.
\]
It follows that
\[
\mathbf P\bigl(L(a^\infty)=S\bigr)>1-\alpha.
\]

\end{proof}

\subsection{NEW SAMPLING Uniform SLLN} \label{sub:uLLN}

\cite{esponda2021asymptotic} (henceforth, EPY 2021) proves the uniform SLLN in the full-history case with a finite action space. We adapt their argument to admissible learning processes in three steps. First, we establish a strong law for the selected observations using martingale moment bounds and a Borel--Cantelli argument. Second, we verify the moment and continuity bounds uniformly over the compact action space. Third, we apply a finite-cover argument over the parameter space.


Fix a player $i$ and suppress the superscript $i$. Let
\[
\mathcal F_t:=\sigma(h_t)
\qquad\text{and}\qquad
\mathcal G_t:=\sigma(h_{t-1},a_t,W_t).
\]
Thus $\mathcal F_{t-1}\subseteq\mathcal G_t\subseteq\mathcal F_t$, and $\mathcal G_t$ contains all information determined before the period-$t$ consequence is realized. By admissibility,
\[
\mathbf P(y_t\in B\mid\mathcal G_t)=Q(B\mid a_t)
\]
for every Borel set $B\subseteq\mathbb Y$.

Define
\[
g(\theta,y,a)
:=
\log\frac{q(y\mid a)}{q_\theta(y\mid a)}.
\]
Recall that $H_t=\{\tau<t:W_{\tau,t}=1\}$ and let $N_t:=|H_t|=\sum_{\tau<t}W_{\tau,t}$. By admissibility, there exist constants $c>0$ and $\gamma>1/2$ such that $N_t\geq ct^\gamma$ for all sufficiently large $t$, $\mathbf P$-almost surely.

\paragraph{Step 1: Selected-sample pointwise convergence.}
Fix $\theta\in\Theta$ and $\varepsilon>0$, and let
\[
O(\theta,\varepsilon)
=
\{\theta'\in\Theta:\|\theta'-\theta\|<\varepsilon\}.
\]
For each period $\tau$, define
\[
\zeta_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E\!\left[
\left.
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
\,\right|\,\mathcal G_\tau
\right].
\]
By construction, $\mathbf E[\zeta_\tau\mid\mathcal G_\tau]=0$. Moreover, since conditional on $\mathcal G_\tau$ the consequence $y_\tau$ is distributed according to $Q(\cdot\mid a_\tau)$,
\[
\zeta_\tau
=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right].
\]

Now fix a date $t$. Since $W_{\tau,t}$ is a component of the row $W_\tau$, it is $\mathcal G_\tau$-measurable for every $\tau<t$. Hence
\[
\mathbf E[W_{\tau,t}\zeta_\tau\mid\mathcal G_\tau]
=
W_{\tau,t}\mathbf E[\zeta_\tau\mid\mathcal G_\tau]
=
0.
\]

Now fix a date $t$ and, for each $\tau<t$, define
\[
D_{\tau,t}:=W_{\tau,t}\zeta_\tau.
\]
Since $W_{\tau,t}$ is $\mathcal G_\tau$-measurable and
$\mathbf E[\zeta_\tau\mid\mathcal G_\tau]=0$,
\[
\mathbf E[D_{\tau,t}\mid\mathcal G_\tau]=0.
\]
Moreover, $D_{\tau,t}$ is $\mathcal F_\tau$-measurable and
$\mathcal F_{\tau-1}\subseteq\mathcal G_\tau$. Hence, by the tower property,
\[
\mathbf E[D_{\tau,t}\mid\mathcal F_{\tau-1}]
=
\mathbf E\!\left[
\mathbf E[D_{\tau,t}\mid\mathcal G_\tau]
\,\middle|\,
\mathcal F_{\tau-1}
\right]
=0.
\]
Thus, for each fixed $t$, $(D_{\tau,t})_{\tau<t}$ is a martingale-difference sequence with respect to the filtration $(\mathcal F_\tau)_{\tau<t}$. Equivalently, the partial sums
\[
S_{s,t}:=\sum_{\tau\leq s}D_{\tau,t},
\qquad s<t,
\]
form a martingale. Its terminal value is
\[
S_t:=S_{t-1,t}
=
\sum_{\tau<t}D_{\tau,t}
=
\sum_{\tau<t}W_{\tau,t}\zeta_\tau
=
\sum_{\tau\in H_t}\zeta_\tau.
\]

As shown in Step 2 below, for every finite $p\geq2$ there exists a constant $C_p<\infty$, independent of $\tau$, such that
\[
\mathbf E\!\left[|\zeta_\tau|^p\mid\mathcal G_\tau\right]
\leq C_p
\qquad \mathbf P\text{-a.s.}
\]
Choose $p>2$ so that $p(\gamma-1/2)>1$. By Burkholder's inequality applied to the martingale $(S_{s,t})_{s<t}$,
\[
\mathbf E|S_t|^p
\leq
C_p\,
\mathbf E\!\left[
\left(\sum_{\tau<t}D_{\tau,t}^2\right)^{p/2}
\right].
\]
For nonnegative $x_\tau$,
\[
\left(\sum_{\tau<t}x_\tau\right)^{p/2}
\leq
t^{p/2-1}\sum_{\tau<t}x_\tau^{p/2}.
\]
Applying this with $x_\tau=D_{\tau,t}^2$ gives
\[
\mathbf E|S_t|^p
\leq
C_p t^{p/2-1}
\sum_{\tau<t}\mathbf E|D_{\tau,t}|^p.
\]
Since $W_{\tau,t}\in\{0,1\}$,
\[
|D_{\tau,t}|^p
=
W_{\tau,t}|\zeta_\tau|^p
\leq
|\zeta_\tau|^p.
\]
Taking expectations in the conditional moment bound therefore yields
$\mathbf E|D_{\tau,t}|^p\leq C_p$, uniformly in $\tau$ and $t$. Hence
\[
\mathbf E|S_t|^p
\leq
C_p t^{p/2}.
\]


Therefore, for every $\eta>0$, Markov's inequality gives
\[
\mathbf P\!\left(|S_t|>\eta t^\gamma\right)
\leq
\frac{C_p}{\eta^p}t^{-p(\gamma-1/2)}.
\]
Since $p(\gamma-1/2)>1$, the right-hand side is summable in $t$. Hence, by the Borel--Cantelli lemma, for every fixed $\eta>0$,
\[
|S_t|\leq \eta t^\gamma
\]
for all sufficiently large $t$, $\mathbf P$-almost surely. Applying this to $\eta=1/m$, $m=1,2,\ldots$, and intersecting the resulting probability-one events yields
\[
\frac{S_t}{t^\gamma}\to0
\qquad \mathbf P\text{-a.s.}
\]
On the probability-one event on which also $N_t\geq ct^\gamma$ for all sufficiently large $t$,
\[
\left|
\frac1{N_t}\sum_{\tau\in H_t}\zeta_\tau
\right|
=
\frac{|S_t|}{N_t}
\leq
\frac1c\frac{|S_t|}{t^\gamma}
\to0.
\]
Hence
\[
\frac1{N_t}\sum_{\tau\in H_t}\zeta_\tau
\to0
\qquad \mathbf P\text{-a.s.}
\]


\paragraph{Step 2: Uniform bounds over the compact action space.}
EPY 2021 assumes a finite action space, so the moment and continuity bounds used in their argument are automatically uniform over actions. With a compact action space, we establish the required uniform bounds directly.

\medskip
\noindent
\emph{Claim 1: Uniform moment bound.}
For every $\theta\in\Theta$, $\varepsilon>0$, and finite $p\geq2$,
\[
\sup_{a\in\mathbb A}
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)|^p
\,Q(dy\mid a)
<\infty.
\]

Indeed, by the likelihood-ratio bound in Assumption~\ref{ass:game}(iii),
\[
\sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)|
\leq \log M(y)
\]
for $\nu$-almost every $y$. Hence, using $q(y\mid a)\leq r(y)$,
\[
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)|^p
\,Q(dy\mid a)
\leq
\int_{\mathbb Y}(\log M(y))^p r(y)\,\nu(dy).
\]
For every finite $p\geq2$, there exists $C_p<\infty$ such that
$(\log x)^p\leq C_p x$ for all $x\geq1$. Therefore,
\[
\int_{\mathbb Y}(\log M(y))^p r(y)\,\nu(dy)
\leq
C_p\int_{\mathbb Y}M(y)r(y)\,\nu(dy)<\infty,
\]
and the bound is independent of $a$.

In particular, letting
\[
Z_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau),
\]
admissibility and Claim 1 imply
\[
\mathbf E[|Z_\tau|^p\mid\mathcal G_\tau]\leq C_p
\qquad \mathbf P\text{-a.s.}
\]
for some $C'_p<\infty$ independent of $\tau$. 

Since
\[
\zeta_\tau
=
Z_\tau-\mathbf E[Z_\tau\mid\mathcal G_\tau],
\]
we have
\[
|\zeta_\tau|^p
\leq
2^{p-1}
\left(
|Z_\tau|^p+
\left|\mathbf E[Z_\tau\mid\mathcal G_\tau]\right|^p
\right).
\]
Since $x\mapsto |x|^p$ is convex for $p\geq1$, conditional Jensen's inequality implies
\[
\left|\mathbf E[Z_\tau\mid\mathcal G_\tau]\right|^p
\leq
\mathbf E[|Z_\tau|^p\mid\mathcal G_\tau].
\]
Taking conditional expectations therefore gives
\[
\mathbf E[|\zeta_\tau|^p\mid\mathcal G_\tau]
\leq
2^p C'_p
\qquad \mathbf P\text{-a.s.}
\]
This is the moment bound used in Step 1.

\medskip
\noindent
\emph{Claim 2: Uniform oscillation bound.}
For every $\theta\in\Theta$ and $\varepsilon>0$, there exists
$\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
<\frac{\varepsilon}{4}.
\]

For $r>0$, define
\[
H_r(y)
:=
\sup_{\substack{\|\theta'-\theta\|\leq r\\ a\in\mathbb A}}
|g(\theta',y,a)-g(\theta,y,a)|.
\]
By the a.e.\ continuity assumption and compactness of $\Theta\times\mathbb A$,
\[
H_r(y)\to0
\qquad\text{for $\nu$-a.e.\ $y$ as }r\downarrow0.
\]
Moreover, the likelihood-ratio bound implies
\[
H_r(y)\leq2\log M(y)\leq2M(y)
\]
for $\nu$-almost every $y$. Therefore, for every $a\in\mathbb A$,
\[
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
\leq
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy).
\]
Since $H_r(y)r(y)\leq2M(y)r(y)$ and
$\int 2M(y)r(y)\,\nu(dy)<\infty$, dominated convergence gives
\[
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy)\to0.
\]
The bound on the right-hand side does not depend on $a$, so
\[
\sup_{a\in\mathbb A}
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
\to0.
\]
Choosing $r=\delta(\theta,\varepsilon)$ sufficiently small proves the claim.

\paragraph{Step 3: Uniform convergence over the parameter space.}
We now adapt the finite-cover argument in EPY 2021 to the selected sample. Fix $\varepsilon>0$. By Claim 2, for every $\theta\in\Theta$ there exists $\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
<\frac{\varepsilon}{4}.
\]
By compactness of $\Theta$, there exist $\theta_1,\ldots,\theta_J$ such that
\[
\Theta\subseteq\bigcup_{j=1}^J O(\theta_j,\delta_j),
\qquad
\delta_j:=\delta(\theta_j,\varepsilon).
\]

For each $t$, define
\[
D_t(\theta)
:=
\frac1{N_t}\sum_{\tau\in H_t}
\left[g(\theta,y_\tau,a_\tau)-K(\theta,a_\tau)\right].
\]
For each $j$, let
\[
U_{t,j}
:=
\frac1{N_t}\sum_{\tau\in H_t}
\left\{
\sup_{\theta\in O(\theta_j,\delta_j)}g(\theta,y_\tau,a_\tau)
-
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a_\tau)
\right]
\right\},
\]
and
\[
L_{t,j}
:=
\frac1{N_t}\sum_{\tau\in H_t}
\left\{
\inf_{\theta\in O(\theta_j,\delta_j)}g(\theta,y_\tau,a_\tau)
-
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\inf_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a_\tau)
\right]
\right\}.
\]
Step 1 implies $U_{t,j}\to0$ almost surely. Applying the same argument to $-g$ implies $L_{t,j}\to0$ almost surely. Since the cover is finite,
\[
\max_{1\leq j\leq J}\{|U_{t,j}|,|L_{t,j}|\}\to0
\qquad\text{almost surely}.
\]

Now fix $\theta\in O(\theta_j,\delta_j)$. Since
\[
g(\theta,y,a)\leq
\sup_{\theta'\in O(\theta_j,\delta_j)}g(\theta',y,a)
\]
and
\[
K(\theta,a)
=
\mathbf E_{Q(\cdot\mid a)}[g(\theta,Y,a)]
\geq
\mathbf E_{Q(\cdot\mid a)}
\left[
\inf_{\theta'\in O(\theta_j,\delta_j)}g(\theta',Y,a)
\right],
\]
we obtain
\[
D_t(\theta)\leq U_{t,j}+B_{t,j},
\]
where
\[
B_{t,j}
:=
\frac1{N_t}\sum_{\tau\in H_t}
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a_\tau)
-
\inf_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a_\tau)
\right].
\]
Similarly,
\[
D_t(\theta)\geq L_{t,j}-B_{t,j}.
\]
Hence
\[
\sup_{\theta\in O(\theta_j,\delta_j)}
|D_t(\theta)|
\leq
\max\{|U_{t,j}|,|L_{t,j}|\}+B_{t,j}.
\]

Moreover,
\[
\sup_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a)
-
\inf_{\theta\in O(\theta_j,\delta_j)}g(\theta,Y,a)
\leq
2\sup_{\theta\in O(\theta_j,\delta_j)}
|g(\theta,Y,a)-g(\theta_j,Y,a)|.
\]
Therefore Claim 2 implies
\[
B_{t,j}<\frac{\varepsilon}{2}
\]
for every $t$ and every $j$. It follows that, almost surely,
\[
\limsup_{t\to\infty}
\sup_{\theta\in\Theta}|D_t(\theta)|
\leq
\frac{\varepsilon}{2}.
\]
Since $\varepsilon>0$ is arbitrary,
\[
\sup_{\theta\in\Theta}
\left|
\frac1{N_t}\sum_{\tau\in H_t}
\left[g(\theta,y_\tau,a_\tau)-K(\theta,a_\tau)\right]
\right|
\to0
\qquad\mathbf P\text{-a.s.}
\]

Finally,
\[
L_t(\theta)
=
\frac1{N_t}\sum_{\tau\in H_t}g(\theta,y_\tau,a_\tau)
\]
and
\[
\int_{\mathbb A}K(\theta,a)\,\hat\sigma_t(da)
=
\frac1{N_t}\sum_{\tau\in H_t}K(\theta,a_\tau).
\]
Hence
\[
\sup_{\theta\in\Theta}
\left|
L_t(\theta)
-
\int_{\mathbb A}K(\theta,a)\,\hat\sigma_t(da)
\right|
\to0
\qquad\mathbf P\text{-a.s.},
\]
which is the desired uniform SLLN.

The proof separates the two extensions of EPY 2021. General selected sampling affects Step 1, where predictability and the sample-growth condition yield convergence through martingale moment bounds and a Borel--Cantelli argument. The extension from a finite to a compact action space affects Step 2, through the uniform moment and oscillation bounds. Given these two ingredients, Step 3 upgrades the local convergence to uniform convergence over the parameter space by compactness.


\subsection{NEW DEMIAN Uniform SLLN} \label{sub:uLLN}

\cite{esponda2021asymptotic} (henceforth, EPY 2021) proves the uniform SLLN in the full-history case with a finite action space. We adapt their argument to admissible learning processes in three steps. First, we establish a strong law for the selected observations using martingale moment bounds and a Borel--Cantelli argument. Second, we verify the moment and continuity bounds uniformly over the compact action space. Third, we apply a finite-cover argument over the parameter space.


Fix a player $i$ and suppress the superscript $i$. Let
\[
\mathcal F_t:=\sigma(h_t)
\qquad\text{and}\qquad
\mathcal G_t:=\sigma(h_{t-1},a_t,W_t).
\]
Thus $\mathcal F_{t-1}\subseteq\mathcal G_t\subseteq\mathcal F_t$, and $\mathcal G_t$ contains all information determined before the period-$t$ consequence is realized. By admissibility,
\[
\mathbf P(y_t\in B\mid\mathcal G_t)=Q(B\mid a_t)
\]
for every Borel set $B\subseteq\mathbb Y$.

Define
\[
g(\theta,y,a)
:=
\log\frac{q(y\mid a)}{q_\theta(y\mid a)}.
\]
Recall that $H_t=\{\tau<t:W_{\tau,t}=1\}$ and let $N_t:=|H_t|=\sum_{\tau<t}W_{\tau,t}$. By admissibility, there exist constants $c>0$ and $\gamma>1/2$ such that $N_t\geq ct^\gamma$ for all sufficiently large $t$, $\mathbf P$-almost surely.


Fix $\theta\in\Theta$ and $\varepsilon>0$, and let
\[
O(\theta,\varepsilon)
=
\{\theta'\in\Theta:\|\theta'-\theta\|<\varepsilon\}.
\]
For each period $\tau$, define
\[
\zeta_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E\!\left[
\left.
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
\,\right|\,\mathcal G_\tau
\right].
\]
By construction, $\mathbf E[\zeta_\tau\mid\mathcal G_\tau]=0$. Moreover, since conditional on $\mathcal G_\tau$ the consequence $y_\tau$ is distributed according to $Q(\cdot\mid a_\tau)$,
\[
\zeta_\tau
=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right].
\]

Now fix a date $t$. Since $W_{\tau,t}$ is a component of the row $W_\tau$, it is $\mathcal G_\tau$-measurable for every $\tau<t$. Hence
\[
\mathbf E[W_{\tau,t}\zeta_\tau\mid\mathcal G_\tau]
=
W_{\tau,t}\mathbf E[\zeta_\tau\mid\mathcal G_\tau]
=
0.
\]

Now fix a date $t$ and, for each $\tau<t$, define
\[
D_{\tau,t}:=W_{\tau,t}\zeta_\tau.
\]
Since $W_{\tau,t}$ is $\mathcal G_\tau$-measurable and
$\mathbf E[\zeta_\tau\mid\mathcal G_\tau]=0$,
\[
\mathbf E[D_{\tau,t}\mid\mathcal G_\tau]=0.
\]
Moreover, $D_{\tau,t}$ is $\mathcal F_\tau$-measurable and
$\mathcal F_{\tau-1}\subseteq\mathcal G_\tau$. Hence, by the tower property,
\[
\mathbf E[D_{\tau,t}\mid\mathcal F_{\tau-1}]
=
\mathbf E\!\left[
\mathbf E[D_{\tau,t}\mid\mathcal G_\tau]
\,\middle|\,
\mathcal F_{\tau-1}
\right]
=0.
\]
Thus, for each fixed $t$, $(D_{\tau,t})_{\tau<t}$ is a martingale-difference sequence with respect to the filtration $(\mathcal F_\tau)_{\tau<t}$. 

Let 
\[
S_t :  = \sum_{\tau<t}D_{\tau,t}
=
\sum_{\tau<t}W_{\tau,t}\zeta_\tau
=
\sum_{\tau\in H_t}\zeta_\tau.
\]

\bigskip

We now show that for any $\lambda \in (0,1/2]$,
\begin{align} \label{eqn:USLLN-1}
E\left[
\exp\left\{
\lambda S_t-C\lambda^2N_t
\right\}
\right]
\leq1,
\end{align}
where $C: = 2 e^{R} R$ with $R: = \int_Y M(y)r(y)\,\nu(dy)$.


To do this, observe that 
\begin{align} 
    E\left[
\exp\left\{
\lambda S_t-C\lambda^2N_t
\right\}
\right] = & E\left[ \prod_{\tau < t} 
\exp\left\{
\lambda W_{\tau,t} \zeta_{\tau}  -C\lambda^2 W_{\tau,t}
\right\}
\right].
\end{align}

By Lemma \ref{lem:MGF.zeta}, 
\begin{align}
    E[\exp\{ \lambda \zeta_{\tau} \} \mid \mathcal G_{\tau}  ] \leq \exp \{C \lambda ^{2} \}.
\end{align}

This result and the fact that $W_{\tau,t} \in \{0,1\}$ and is $\mathcal G_{\tau}$-measurable implies that fo rany $\tau < t$,
\begin{align*}
 E \left[ \exp\left\{
\lambda W_{\tau,t} \zeta_{\tau }  -C\lambda^2 W_{\tau,t}
\right\}   \mid \mathcal G_{\tau}  \right] & \leq 1- W_{\tau,t} + W_{\tau,t} \exp\{- C \lambda ^{2} \} E \left[ \exp\left\{
\lambda W_{\tau,t} \zeta_{\tau } \right\}   \mid \mathcal G_{\tau}  \right] \\
& \leq 1.
\end{align*}

Hence, using this result and iterating over \eqref{eqn:USLLN-1}, we obtain $E\left[
\exp\left\{
\lambda S_t-C\lambda^2N_t
\right\}
\right]
\leq1$  
as desired. 


Fix $m \in \mathbb{N}$ and choose $\lambda_m\in(0,1/2]$ sufficiently
small that $\kappa_m
:=
\lambda_m/m-C\lambda_m^2
>0$. 
For example, one may take
\[
\lambda_,
:=
\min\left\{
\frac{1}{2Cm},
\frac14
\right\}.
\]
Also, let 
\[
A_{t,m}
:=
\left\{
|S_t|\geq \frac{1}{m}N_t
\right\}
\cap
\left\{
N_t\geq ct^\gamma
\right\}.
\]

By expression \eqref{eqn:USLLN-1} and applying the Markov inequality to $S_{t}$ and $-S_{t}$, it follows that
\[
P\left( A_{t,m}
\right)
\leq
2\exp\{-\kappa_m ct^\gamma\}.
\]
Since $\sum_{t=1}^{\infty}
\exp\{-\kappa_m ct^\gamma\}
<\infty$  for every $\gamma>0$ and $m \in \mathbb{N}$, the Borel--Cantelli lemma implies that
\begin{align*}
   \Omega_{m} : = \left( \limsup_{t \to \infty} A_{m,t}   \right)^{\mathrm{C}} \text{ has probability one under $\mathbf{P}$}.
\end{align*}

Since each $\Omega_{m}$ has probability one of occurring, so does $\Omega : = \cap_{m=1}^{\infty} \Omega_{m}$. Observe that for each $\omega \in \Omega$ and any $m \in \mathbb{N}$, there exist $T_{m} \in \mathbb{N}$ such that 
\[
N_t(\omega)\geq ct^\gamma \quad and \quad \omega\notin A_{t,m},
\qquad
\text{for every }t\geq T_m.
\]
Consequently, $\frac{|S_t(\omega)|}{N_t(\omega)} <\frac{1}{m}$ for any $t \geq T_{m}$.

Since the last expression holds for any $m \in \mathbb{N}$, we conclude that
\[
\frac{S_t}{N_t}
=
\frac{1}{N_t}
\sum_{\tau\in H_t}\zeta_\tau
\to 0
\qquad \mathbf{P}\text{-almost surely}.
\]

$\qed$


\begin{lemma}\label{lem:MGF.zeta}
For any $|\lambda| \leq 1/2$,
    \begin{align}
    E[\exp\{ \lambda \zeta_{\tau} \} \mid \mathcal G_{\tau}  ] \leq \exp \{C \lambda ^{2} \},~a.s.-\mathbf{P}
\end{align}
where $C: = 2 e^{R} R$ with $R: = \int_Y M(y)r(y)\,\nu(dy)$.
\end{lemma}

\begin{proof}
 Let $R
:=
\int_Y M(y)r(y)\,\nu(dy)<\infty$. 
The likelihood-ratio bound in Assumption~1(iii) implies that, for
$\nu$-almost every $y$,
\[
\sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)|
\leq
\log M(y)
\]
for every $a\in A$. Hence $e^{ \sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)| }
\leq M(y)$.

Since, conditionally on $\mathcal G_\tau$, the consequence $Y_\tau$
has distribution $Q(\cdot\mid a_\tau)$, it follows that
\begin{align*}
E\left[\exp\{ \sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y_{\tau}, a_{\tau} )|   \} \mid\mathcal G_\tau\right]
\leq
\int_Y M(y)q(y\mid a_\tau)\,\nu(dy) \leq
\int_Y M(y)r(y)\,\nu(dy) =R.
\end{align*}
Moreover, since $\log M(y)\leq M(y)$ for $M(y)\geq1$,
\begin{align*}
E\left[ \sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y_{\tau}, a_{\tau} )|   \mid\mathcal G_\tau\right] \leq
\int_Y \log M(y)q(y\mid a_\tau)\,\nu(dy) \leq
\int_Y M(y)r(y)\,\nu(dy) =R.
\end{align*}
Consequently, $ \zeta_{\tau} 
\leq \sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y_{\tau}, a_{\tau} )| +R$, 
and hence
\begin{align*}
E\left[e^{|\zeta_\tau|}\mid\mathcal G_\tau\right] \leq e^R R =:K.
\end{align*}
Since for  every integer $k\geq2$, $|x|^k\leq k!e^|x|$, the previous inequality implies $E\left[|\zeta_\tau|^k\mid\mathcal G_\tau\right]
\leq Kk!$. 

By using Taylor expansions and the facc that $E[\zeta_\tau\mid\mathcal G_\tau]=0$, it follows that
\begin{align*}
E\left[e^{\lambda\zeta_\tau}\mid\mathcal G_\tau\right]
&=
1+
\sum_{k=2}^{\infty}
\frac{\lambda^k}{k!}
E\left[\zeta_\tau^k\mid\mathcal G_\tau\right] \\
&\leq
1+
\sum_{k=2}^{\infty}
\frac{|\lambda|^k}{k!}
E\left[|\zeta_\tau|^k\mid\mathcal G_\tau\right] \\
&\leq
1+
K\sum_{k=2}^{\infty}|\lambda|^k \\
&=
1+
K\frac{\lambda^2}{1-|\lambda|}.
\end{align*}

Now restrict attention to $|\lambda|\leq 1/2$. Then $\frac{1}{1-|\lambda|}\leq 2$ and therefore $E\left[e^{\lambda\zeta_\tau}\mid\mathcal G_\tau\right]
\leq 1+2K\lambda^2$. Using the inequality $1+x\leq e^x$ for every $x\geq0$, we obtain $1+2K\lambda^2
\leq
e^{2K\lambda^2}$. Consequently,
\[
E\left[e^{\lambda\zeta_\tau}\mid\mathcal G_\tau\right]
\leq
e^{C\lambda^2},
\]
where $C:=2K$ for any $|\lambda|\leq\frac12$.




\end{proof}





\subsection{Uniform SLLN --- OLD} \label{sub:uLLN}

\cite{esponda2021asymptotic} (henceforth, EPY 2021) proves the uniform SLLN in the full-history case with a finite action space. We adapt their argument to admissible learning processes in three steps. First, we establish a martingale strong law for persistently selected observations. Second, we verify the moment and continuity bounds uniformly over the compact action space. Third, we apply the same finite-cover argument as EPY 2021 to obtain uniform convergence over the parameter space.

Fix a player $i$ and suppress the superscript $i$. Let
\[
\mathcal F_t:=\sigma(h_t)
\qquad\text{and}\qquad
\mathcal G_t:=\sigma(h_{t-1},a_t,J_t).
\]
Thus $\mathcal F_{t-1}\subseteq\mathcal G_t\subseteq\mathcal F_t$, and
$\mathcal G_t$ contains all information determined before the period-$t$
consequence is realized. By admissibility,
\[
\mathbf P(y_t\in B\mid\mathcal G_t)=Q(B\mid a_t)
\]
for every Borel set $B\subseteq\mathbb Y$.

Define
\[
g(\theta,y,a)
:=
\log\frac{q(y\mid a)}{q_\theta(y\mid a)}.
\]
Let
\[
N_t:=|H_t|=\sum_{\tau<t}J_\tau.
\]
By admissibility, $N_t\to\infty$ $\mathbf P$-almost surely.

\paragraph{Step 1: Selected-sample pointwise convergence.}
Fix $\theta\in\Theta$ and $\varepsilon>0$, and let
$O(\theta,\varepsilon)=\{\theta'\in\Theta:\|\theta'-\theta\|<\varepsilon\}$.
For each period $\tau$, define
\[
\zeta_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E\!\left[
\left.
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
\,\right|\,\mathcal G_\tau
\right].
\]
By admissibility,
\[
\mathbf E[\zeta_\tau\mid\mathcal G_\tau]=0.
\]
Since $J_\tau$ is $\mathcal G_\tau$-measurable,
\[
\mathbf E[J_\tau\zeta_\tau\mid\mathcal G_\tau]=0.
\]

Moreover, since conditional on $\mathcal G_\tau$ the consequence $y_\tau$ is distributed according to $Q(\cdot\mid a_\tau)$,
\[
\mathbf E\!\left[
\left.
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
\,\right|\,\mathcal G_\tau
\right]
=
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right].
\]
Hence
\[
\zeta_\tau
=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbf E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right].
\]

As shown in Step 2 below, there exists a constant $C<\infty$, independent of $\tau$, such that
\[
\mathbf E[\zeta_\tau^2\mid\mathcal G_\tau]\leq C
\qquad \mathbf P\text{-a.s.}
\]

Recall that
\[
N_t:=|H_t|=\sum_{\tau<t}J_\tau
\]
is the number of selected observations available at date $t$. Consider
\[
M_t
:=
\sum_{\tau<t}
\frac{J_\tau\zeta_\tau}{N_{\tau+1}},
\]
where terms with $J_\tau=0$ are understood to be zero. Since
$N_{\tau+1}=\sum_{s\leq\tau}J_s$, the denominator counts the selected observations up to and including period $\tau$.

Since $J_\tau$ and $N_{\tau+1}$ are $\mathcal G_\tau$-measurable and
$\mathbf E[J_\tau\zeta_\tau\mid\mathcal G_\tau]=0$, $(M_t)_t$ is a martingale with respect to $(\mathcal F_t)_t$. Using the conditional $L^2$ bound and orthogonality of martingale differences,
\[
\mathbf E[M_t^2]
\leq
C\,\mathbf E\!\left[
\sum_{\tau<t}\frac{J_\tau}{N_{\tau+1}^2}
\right].
\]

Let $\tau_n$ denote the date of the $n$th selected observation. Then
$N_{\tau_n+1}=n$. Hence, pathwise,
\[
\sum_{\tau<t}\frac{J_\tau}{N_{\tau+1}^2}
\leq
\sum_{n=1}^\infty\frac1{n^2}<\infty.
\]
Thus $(M_t)_t$ is bounded in $L^2$ and converges $\mathbf P$-almost surely by the martingale convergence theorem.

Since $N_{\tau_n+1}=n$, convergence of $(M_t)_t$ implies that
\[
\sum_{n=1}^\infty\frac{\zeta_{\tau_n}}{n}
\]
converges $\mathbf P$-almost surely. By Kronecker's lemma,
\[
\frac1n\sum_{m=1}^n\zeta_{\tau_m}\to0
\qquad \mathbf P\text{-a.s.}
\]
Finally, let $\tau_n$ denote the date of the $n$th selected observation. On the probability-one event where
\[
\frac1n\sum_{m=1}^n\zeta_{\tau_m}\to0
\qquad\text{and}\qquad
N_t\to\infty,
\]
fix a realization. Then $N_t$ is simply a deterministic sequence of integers diverging to infinity. Since
\[
H_t=\{\tau_1,\ldots,\tau_{N_t}\},
\]
we have
\[
\frac1{N_t}\sum_{\tau\in H_t}\zeta_\tau
=
\frac1{N_t}\sum_{m=1}^{N_t}\zeta_{\tau_m}.
\]
The right-hand side is a subsequence of
\[
\frac1n\sum_{m=1}^n\zeta_{\tau_m},
\]
and therefore also converges to zero. Hence
\[
\frac1{N_t}\sum_{\tau\in H_t}\zeta_\tau\to0
\qquad \mathbf P\text{-a.s.}
\]

\paragraph{Step 2: Uniform bounds over the compact action space.}
EPY 2021 assumes a finite action space, so the moment and continuity bounds used in their argument are automatically uniform over actions. With a compact action space, we establish the required uniform bounds directly.

\medskip
\noindent
\emph{Claim 1: Uniform $L^2$ bound.}
For every $\theta\in\Theta$ and $\varepsilon>0$,
\[
\sup_{a\in\mathbb A}
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
[g(\theta',y,a)]^2
\,Q(dy\mid a)
<\infty.
\]

Indeed, by the likelihood-ratio bound in Assumption~\ref{ass:game}(iii),
\[
\sup_{\theta'\in O(\theta,\varepsilon)}
|g(\theta',y,a)|
\leq \log M(y)
\]
for $\nu$-almost every $y$. Hence, using $q(y\mid a)\leq r(y)$,
\[
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
[g(\theta',y,a)]^2
\,Q(dy\mid a)
\leq
\int_{\mathbb Y}(\log M(y))^2r(y)\,\nu(dy).
\]
Since $(\log x)^2\leq2x$ for $x\geq1$,
\[
\int_{\mathbb Y}(\log M(y))^2r(y)\,\nu(dy)
\leq
2\int_{\mathbb Y}M(y)r(y)\,\nu(dy)<\infty,
\]
and the bound is independent of $a$.

In particular, letting
\[
Z_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau),
\]
admissibility and Claim 1 imply
\[
\mathbf E[Z_\tau^2\mid\mathcal G_\tau]\leq C
\qquad \mathbf P\text{-a.s.}
\]
for some $C<\infty$ independent of $\tau$. Since
$\zeta_\tau=Z_\tau-\mathbf E[Z_\tau\mid\mathcal G_\tau]$,
\[
\mathbf E[\zeta_\tau^2\mid\mathcal G_\tau]
=
\operatorname{Var}(Z_\tau\mid\mathcal G_\tau)
\leq C.
\]
This is the bound used in Step 1.

\medskip
\noindent
\emph{Claim 2: Uniform oscillation bound.}
For every $\theta\in\Theta$ and $\varepsilon>0$, there exists
$\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
<\frac{\varepsilon}{4}.
\]

For $r>0$, define
\[
H_r(y)
:=
\sup_{\substack{\|\theta'-\theta\|\leq r\\ a\in\mathbb A}}
|g(\theta',y,a)-g(\theta,y,a)|.
\]
By the a.e.\ continuity assumption and compactness of $\Theta\times\mathbb A$,
\[
H_r(y)\to0
\qquad\text{for $\nu$-a.e.\ $y$ as }r\downarrow0.
\]
Moreover, the likelihood-ratio bound implies
\[
H_r(y)\leq2\log M(y)\leq2M(y)
\]
for $\nu$-almost every $y$. Therefore, for every $a\in\mathbb A$,
\[
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
\leq
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy).
\]
Since $H_r(y)r(y)\leq2M(y)r(y)$ and
$\int 2M(y)r(y)\,\nu(dy)<\infty$, dominated convergence gives
\[
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy)\to0.
\]
The convergence is independent of $a$, so
\[
\sup_{a\in\mathbb A}
\mathbf E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
|g(\theta',Y,a)-g(\theta,Y,a)|
\right]
\to0.
\]
Choosing $r=\delta(\theta,\varepsilon)$ sufficiently small proves the claim.



\section{OLD Proof of Lemma \ref{lemm:Berk-selected}} \label{sub:lemm:Berk-selected}

In this Supplemental Appendix, we provide the proof of Lemma \ref{lemm:Berk-selected} for completeness. As remarked in the text, this proof is a straightforward extension of existing ones (e.g. \cite{esponda2021asymptotic}) to a continuum of actions and convergent subsequences instead of sequences.

The result holds for each player $i$. Henceforth, we drop the $i$ superscript from the notation and focus on an individual player.

For every \(t\) such that \(H_t\neq\varnothing\), let \(n_t:=|H_t|\) and define
\[
L_t(\theta):=\frac{1}{n_t}\sum_{\tau\in H_t}\ln\frac{q(y_\tau\mid a_\tau)}{q_\theta(y_\tau\mid a_\tau)}.
\]
Recall that the selected empirical distribution is
\[
\hat\sigma_t=\frac{1}{n_t}\sum_{\tau\in H_t}\delta_{a_\tau}.
\]

We will use the following fact:

\emph{Uniform SLLN.} With $\mathbf P$-probability one,
\begin{equation}\label{eq:uLLN}
\sup_{\theta\in\Theta}
\left|
L_t(\theta)
-
\int K(\theta,a)\hat\sigma_t(da)
\right|
\longrightarrow 0
\end{equation}
as $t\to\infty$ along dates for which $H_t\neq\varnothing$. Since $|H_t|\to\infty$, this condition is satisfied eventually. See Section \ref{sub:uLLN} for a proof of this result.

From this point on, fix a realization in the probability-one event on which \eqref{eq:uLLN} holds. Let $(t_k)_k$ be a subsequence such that
\[
\hat\sigma_{t_k}\Rightarrow\sigma
\]
for some $\sigma\in\Delta\mathbb A$, and let $E\subseteq\Theta$ be a closed set disjoint from $\Theta^m(\sigma)$. We rely on the following two observations:

\emph{Uniform convergence of empirical KL} Since $K$ is continuous and $\Theta$ is compact, for every $\varepsilon>0$ there exists $K_\varepsilon^2$ such that, for all $k\geq K_\varepsilon^2$,
\[
\sup_{\theta\in\Theta}
\left|
\int K(\theta,a)\hat\sigma_{t_k}(da)
-
\int K(\theta,a)\sigma(da)
\right|
<\varepsilon.
\]

We now prove \eqref{eq:exponential} in Lemma \ref{lemm:Berk-selected}. For any $\xi>0$, note that
\[
\mu_{t_k}(E)
=
\frac{
\int_E e^{-n_{t_k}L_{t_k}(\theta)}\mu_0(d\theta)
}{
\int_\Theta e^{-n_{t_k}L_{t_k}(\theta)}\mu_0(d\theta)
}
\leq
\frac{
\int_E e^{-n_{t_k}L_{t_k}(\theta)}\mu_0(d\theta)
}{
\int_{\Theta_\xi(\sigma)} e^{-n_{t_k}L_{t_k}(\theta)}\mu_0(d\theta)
},
\]
where
\[
\Theta_\xi(\sigma)
:=
\left\{
\theta\in\Theta:
\int K(\theta,a)\sigma(da)
\leq
K^*(\sigma)+\xi
\right\}.
\]

Consider first the numerator. By the Uniform SLLN, the approximation of $(\hat\sigma_{t_k})_k$ by its limit $\sigma$, and the well separation of $E$, for all sufficiently large $k$,
\[
L_{t_k}(\theta)
\geq
K^*(\sigma)+\delta-2\varepsilon
\qquad
\text{for all }\theta\in E.
\]
Hence
\begin{equation}\label{eq:numerator}
\int_E e^{-n_{t_k}L_{t_k}(\theta)}\mu_0(d\theta)
\leq
\mu_0(E)
e^{-n_{t_k}(K^*(\sigma)+\delta-2\varepsilon)}.
\end{equation}

Next, consider the denominator. By the Uniform SLLN and the approximation of $(\hat\sigma_{t_k})_k$ by its limit $\sigma$, for all sufficiently large $k$,
\[
L_{t_k}(\theta)
\leq
K^*(\sigma)+\xi+2\varepsilon
\qquad
\text{for all }\theta\in\Theta_\xi(\sigma).
\]
Hence
\begin{equation}\label{eq:denomirator}
\int_{\Theta_\xi(\sigma)}
e^{-n_{t_k}L_{t_k}(\theta)}
\mu_0(d\theta)
\geq
\mu_0(\Theta_\xi(\sigma))
e^{-n_{t_k}(K^*(\sigma)+\xi+2\varepsilon)}.
\end{equation}

Combining \eqref{eq:numerator} and \eqref{eq:denomirator} and setting $\varepsilon=\xi<\delta/10$, we obtain, for all sufficiently large $k$,
\[
\mu_{t_k}(E)
\leq
\frac{\mu_0(E)}{\mu_0(\Theta_\xi(\sigma))}
e^{-n_{t_k}\delta/2}.
\]
Since $\Theta$ is compact and $\theta\mapsto\int K(\theta,a)\sigma(da)$ is continuous, a minimizer $\theta^*\in\Theta$ exists and satisfies $\theta^*\in\Theta_\xi(\sigma)$. By continuity, there exists an open neighborhood of $\theta^*$ contained in $\Theta_\xi(\sigma)$. Since $\mu_0$ has full support, this neighborhood has strictly positive $\mu_0$-measure, and therefore
\[
\mu_0(\Theta_\xi(\sigma))>0.
\]
Hence \eqref{eq:exponential} follows by setting
\[
\rho=\delta/2
\qquad\text{and}\qquad
C=\frac{\mu_0(E)}{\mu_0(\Theta_\xi(\sigma))}.
\]
Since $\mu_0(E)\geq0$ and $\mu_0(\Theta_\xi(\sigma))>0$, we have $0\leq C<\infty$.

Suppose, in addition, that $(\mu_{t_k})_{k}$ converges to $\mu$. By equation (\ref{eq:exponential}), for any closed $E$ such that $E \cap \Theta^m(\sigma)=\emptyset$, $\lim\inf_{k\rightarrow \infty} \mu_{t_k}(E)=0$. By the Pormanteau lemma, $\mu(E)\leq \lim\inf_{k\rightarrow \infty} \mu_{t_k}(E)=0$. Now consider any $\theta \in \Theta \setminus \Theta^m(\sigma)$. There exists an open neighborhood $U_\theta$ with closure $\bar{U}_\theta$ such that $\bar{U}_\theta \cap \Theta^m(\sigma) =\emptyset$. Since $\bar{U}_\theta$ is closed, $\mu(\bar{U}_\theta)=0$, and so $\theta$ is not in the support of $\mu$. Thus, $supp \hspace{2pt} \mu \subseteq \Theta^m(\sigma)$.


\subsection{OLD Uniform SLLN} \label{sub:uLLN}

\cite{esponda2021asymptotic} (henceforth, EPY 2021) proves the uniform SLLN in equation \eqref{eq:uLLN} when the action space is finite and all observations are used (see their Lemma 2). We adapt their proof in three steps. First, we establish the analogue of their pointwise martingale strong law for the selected sample. This is the only step that requires a new argument due to sample selection. Second, we verify the two bounds used in their proof uniformly over the compact action space. Third, we apply the same finite-cover argument as EPY 2021 to obtain uniform convergence over the parameter space.

Fix a player $i$ and suppress the player superscript throughout the proof. Define
\[
g(\theta,y,a)
:=
\log\frac{q(y\mid a)}{q_\theta(y\mid a)}.
\]
Let $I_\tau\in\{0,1\}$ denote the selection decision for observation $\tau$, as defined in the main text, and let
\[
N_t:=|H_t|=\sum_{\tau<t}I_\tau.
\]
By assumption, $N_t\to\infty$ along every infinite action path.

\paragraph{Step 1: Selected-sample pointwise convergence.}
Fix $\theta\in\Theta$ and $\varepsilon>0$, and let $O(\theta,\varepsilon)=\{\theta'\in\Theta:\|\theta'-\theta\|<\varepsilon\}$. For each period $\tau$, define
\[
\zeta_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbb E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right].
\]
Let $\mathcal F_\tau^-$ denote the information determined before the consequence $y_\tau$ is realized, including the action history through $a_\tau$ and the exogenous randomization used for sample selection. By the non-anticipatory sampling restriction, both $a_\tau$ and $I_\tau$ are $\mathcal F_\tau^-$-measurable, while conditional on $\mathcal F_\tau^-$ the consequence $y_\tau$ is distributed according to $Q(\cdot\mid a_\tau)$. Hence
\[
\mathbb E[\zeta_\tau\mid\mathcal F_\tau^-]=0
\qquad\text{and}\qquad
\mathbb E[I_\tau\zeta_\tau\mid\mathcal F_\tau^-]=0.
\]

As shown in the uniform $L^2$ bound below, there is a constant $C<\infty$, independent of $\tau$, such that
\[
\mathbb E[\zeta_\tau^2\mid\mathcal F_\tau^-]\leq C.
\]
Define the number of selected observations through period $\tau$ by
\[
N_\tau^+:=\sum_{s\leq\tau}I_s.
\]
Consider the process
\[
M_t
:=
\sum_{\tau<t}
\frac{I_\tau\zeta_\tau}{N_\tau^+},
\]
where terms with $I_\tau=0$ are understood to be zero. Since $I_\tau$ and $N_\tau^+$ are $\mathcal F_\tau^-$-measurable, $(M_t)_t$ is a martingale. Moreover,
\[
\mathbb E[M_t^2]
=
\mathbb E\left[
\sum_{\tau<t}
\frac{I_\tau}{(N_\tau^+)^2}
\mathbb E[\zeta_\tau^2\mid\mathcal F_\tau^-]
\right]
\leq
C\,\mathbb E\left[
\sum_{\tau<t}\frac{I_\tau}{(N_\tau^+)^2}
\right].
\]
Whenever $I_\tau=1$, $N_\tau^+$ is exactly the rank of observation $\tau$ among the selected observations. Therefore, pathwise,
\[
\sum_{\tau<t}\frac{I_\tau}{(N_\tau^+)^2}
\leq
\sum_{n=1}^{\infty}\frac{1}{n^2}<\infty.
\]
Thus $(M_t)_t$ is bounded in $L^2$ and converges almost surely by the Martingale Convergence Theorem.

Let $\tau_n$ denote the period of the $n$th selected observation. The preceding convergence is equivalently the convergence of
\[
\sum_{n=1}^{\infty}\frac{\zeta_{\tau_n}}{n}.
\]
By Kronecker's lemma,
\[
\frac{1}{n}\sum_{m=1}^n\zeta_{\tau_m}\to0
\qquad\text{almost surely}.
\]
Since the selected observations available at date $t$ are precisely the first $N_t$ selected observations and $N_t\to\infty$, it follows that
\[
\frac{1}{N_t}\sum_{\tau\in H_t}\zeta_\tau\to0
\qquad\text{almost surely}.
\]
Equivalently,
\[
\frac{1}{|H_t|}
\sum_{\tau\in H_t}
\left\{
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau)
-
\mathbb E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',Y,a_\tau)
\right]
\right\}
\to0
\]
almost surely.

\paragraph{Step 2: Uniform bounds over the compact action space.}
EPY 2021 assumes a finite action space, so the moment and continuity bounds needed in their argument can be taken uniformly over actions by maximizing over finitely many values. With a compact action space, we verify these bounds directly.

\paragraph{Claim 1: Uniform $L^2$ bound.}
Fix $\theta\in\Theta$ and $\varepsilon>0$. Then
\[
\sup_{a\in\mathbb A}
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
\bigl[g(\theta',y,a)\bigr]^2
\,Q(dy\mid a)
<\infty.
\]

\emph{Proof.}
For any $a\in\mathbb A$,
\[
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
\bigl[g(\theta',y,a)\bigr]^2
\,Q(dy\mid a)
=
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
\left|
\log\frac{q(y\mid a)}{q_{\theta'}(y\mid a)}
\right|^2
q(y\mid a)\,\nu(dy).
\]
By the likelihood-ratio bound in Assumption~\ref{ass:game}(iii),
\[
\sup_{\theta'\in O(\theta,\varepsilon)}
\left|
\log\frac{q(y\mid a)}{q_{\theta'}(y\mid a)}
\right|
\leq \log M(y)
\]
for $\nu$-a.e.\ $y$. Hence
\[
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
\bigl[g(\theta',y,a)\bigr]^2
\,Q(dy\mid a)
\leq
\int_{\mathbb Y}
\bigl(\log M(y)\bigr)^2 q(y\mid a)\,\nu(dy).
\]
Using $(\log x)^2\leq 2x$ for $x\geq1$ and the density-envelope condition $q(y\mid a)\leq r(y)$,
\[
\int_{\mathbb Y}
\sup_{\theta'\in O(\theta,\varepsilon)}
\bigl[g(\theta',y,a)\bigr]^2
\,Q(dy\mid a)
\leq
2\int_{\mathbb Y}M(y)r(y)\,\nu(dy)<\infty.
\]
The upper bound does not depend on $a$, proving the claim. \qed

In particular, if
\[
Z_\tau
:=
\sup_{\theta'\in O(\theta,\varepsilon)}
g(\theta',y_\tau,a_\tau),
\]
then conditional on the information available before $y_\tau$ is realized,
\[
\mathbb E[Z_\tau^2\mid\mathcal F_\tau^-]\leq C
\]
for some $C<\infty$ independent of $\tau$. Since
\[
\zeta_\tau
=
Z_\tau-\mathbb E[Z_\tau\mid\mathcal F_\tau^-],
\]
Jensen's inequality implies, after enlarging $C$ if necessary,
\[
\mathbb E[\zeta_\tau^2\mid\mathcal F_\tau^-]\leq C.
\]
This is the bound used in Step 1.

\paragraph{Claim 2: Uniform oscillation bound.}
Fix $\theta\in\Theta$ and $\varepsilon>0$. Then there exists $\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}
\mathbb E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
\left|
g(\theta',Y,a)-g(\theta,Y,a)
\right|
\right]
<0.25\,\varepsilon.
\]

\emph{Proof.}
For $r>0$, define
\[
H_r(y)
:=
\sup_{\|\theta'-\theta\|\leq r,\ a\in\mathbb A}
\left|
g(\theta',y,a)-g(\theta,y,a)
\right|.
\]
By the a.e.\ continuity assumption on the compact set $\Theta\times\mathbb A$,
\[
H_r(y)\downarrow0
\qquad\text{for $\nu$-a.e.\ $y$ as }r\downarrow0.
\]
By the likelihood-ratio bound,
\[
H_r(y)
\leq
2\log M(y)
\leq
2M(y)
\]
for $\nu$-a.e.\ $y$. Moreover, since $q(y\mid a)\leq r(y)$,
\[
\mathbb E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
\left|
g(\theta',Y,a)-g(\theta,Y,a)
\right|
\right]
\leq
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy)
\]
for every $a\in\mathbb A$.
Since
\[
H_r(y)r(y)\leq 2M(y)r(y)
\]
and
\[
\int_{\mathbb Y}2M(y)r(y)\,\nu(dy)<\infty,
\]
the Dominated Convergence Theorem yields
\[
\int_{\mathbb Y}H_r(y)r(y)\,\nu(dy)\to0
\qquad\text{as }r\downarrow0.
\]
Therefore
\[
\sup_{a\in\mathbb A}
\mathbb E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,r)}
\left|
g(\theta',Y,a)-g(\theta,Y,a)
\right|
\right]
\to0
\qquad\text{as }r\downarrow0.
\]
Choose $\delta(\theta,\varepsilon)>0$ so that the preceding expression is smaller than $0.25\,\varepsilon$. \qed

\paragraph{Step 3: Uniform convergence over the parameter space.}
We now adapt the finite-cover argument in Step 2 of EPY 2021 to the selected sample. Fix $\varepsilon>0$. By Claim 2, for every $\theta\in\Theta$ there exists $\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}
\mathbb E_{Q(\cdot\mid a)}
\left[
\sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
\left|
g(\theta',Y,a)-g(\theta,Y,a)
\right|
\right]
<0.25\,\varepsilon.
\]
The collection
\[
\left\{
O(\theta,\delta(\theta,\varepsilon))
:
\theta\in\Theta
\right\}
\]
is an open cover of the compact set $\Theta$. Hence there exist $\theta_1,\ldots,\theta_J$ such that
\[
\Theta
\subseteq
\bigcup_{j=1}^J
O(\theta_j,\delta(\theta_j,\varepsilon)).
\]

For each $t$, write
\[
D_t(\theta)
:=
\frac1{N_t}
\sum_{\tau\in H_t}
\left[
g(\theta,y_\tau,a_\tau)-K(\theta,a_\tau)
\right].
\]
Then
\[
\sup_{\theta\in\Theta}|D_t(\theta)|
\leq
\max_{1\leq j\leq J}
\sup_{\theta\in O(\theta_j,\delta_j)}
|D_t(\theta)|,
\]
where $\delta_j:=\delta(\theta_j,\varepsilon)$.

For each $j$,
\[
\sup_{\theta\in O(\theta_j,\delta_j)}
|D_t(\theta)|
\leq
A_{t,j}+B_{t,j},
\]
where
\[
A_{t,j}
:=
\left|
\frac1{N_t}
\sum_{\tau\in H_t}
\left\{
\sup_{\theta\in O(\theta_j,\delta_j)}
g(\theta,y_\tau,a_\tau)
-
\mathbb E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta\in O(\theta_j,\delta_j)}
g(\theta,Y,a_\tau)
\right]
\right\}
\right|
\]
and
\[
B_{t,j}
:=
\frac1{N_t}
\sum_{\tau\in H_t}
\mathbb E_{Q(\cdot\mid a_\tau)}
\left[
\sup_{\theta\in O(\theta_j,\delta_j)}
g(\theta,Y,a_\tau)
-
\inf_{\theta\in O(\theta_j,\delta_j)}
g(\theta,Y,a_\tau)
\right].
\]

By Step 1,
\[
A_{t,j}\to0
\qquad\text{almost surely}
\]
for every $j$. Since there are only finitely many $j$'s,
\[
\max_{1\leq j\leq J}A_{t,j}\to0
\qquad\text{almost surely}.
\]

For the second term, note that
\[
\sup_{\theta\in O(\theta_j,\delta_j)}
g(\theta,Y,a)
-
\inf_{\theta\in O(\theta_j,\delta_j)}
g(\theta,Y,a)
\]
is bounded above by
\[
2
\sup_{\theta\in O(\theta_j,\delta_j)}
\left|
g(\theta,Y,a)-g(\theta_j,Y,a)
\right|.
\]
Therefore Claim 2 implies
\[
B_{t,j}\leq 0.5\,\varepsilon
\]
for every $t$ and every $j$. It follows that, almost surely,
\[
\limsup_{t\to\infty}
\sup_{\theta\in\Theta}|D_t(\theta)|
\leq
0.5\,\varepsilon.
\]
Since $\varepsilon>0$ is arbitrary,
\[
\sup_{\theta\in\Theta}
\left|
\frac1{N_t}
\sum_{\tau\in H_t}
\left[
g(\theta,y_\tau,a_\tau)-K(\theta,a_\tau)
\right]
\right|
\to0
\qquad\text{almost surely}.
\]

Finally,
\[
L_t(\theta)
=
\frac1{N_t}
\sum_{\tau\in H_t}
g(\theta,y_\tau,a_\tau)
\]
and
\[
\int_{\mathbb A}K(\theta,a)\,\hat\sigma_t(da)
=
\frac1{N_t}
\sum_{\tau\in H_t}
K(\theta,a_\tau).
\]
Hence
\[
\sup_{\theta\in\Theta}
\left|
L_t(\theta)
-
\int_{\mathbb A}K(\theta,a)\,\hat\sigma_t(da)
\right|
\to0
\qquad\text{almost surely},
\]
which is the desired uniform SLLN.

The proof separates the two extensions of EPY 2021. Selected sampling affects only Step 1, where the ordinary martingale average is replaced by an average over persistently selected observations. The extension from a finite to a compact action space affects only Step 2, through the uniform moment and oscillation bounds. Once these two ingredients are established, the finite-cover argument in Step 3 is unchanged.






\section{OLD Proof of Lemma \ref{lemm:Berk-selected}} \label{sub:lemm:Berk-selected}

In this Supplemental Appendix, we provide the proof of Lemma \ref{lemm:Berk-selected} for completeness. As remarked in the text, this proof is a straightforward extension of existing ones (e.g. \cite{esponda2021asymptotic}) to a continuum of actions and convergent subsequences instead of sequences.

The result holds for each player $i$. Henceforth, we drop the $i$ superscript from the notation and focus on an individual player.

Define 
\[
L_t(a^\infty,y^\infty)(\theta):=t^{-1} \sum_{\tau=1}^t \ln \frac{q(y_\tau \mid a_\tau)}{q_\theta(y_\tau \mid a_\tau)}. 
\]

We will use the following fact: 

\emph{Uniform SLLN.} For any $a^\infty$, there exists $\mathcal{Y}_{a^\infty}$ with $\mathbf{P}(\mathcal{Y}_{a^\infty} \mid a^\infty)=1$ such that, for any $y^\infty \in \mathcal{Y}_{a^\infty}$ and for every $\varepsilon>0$ there exists $T_\varepsilon^1(a^\infty,y^\infty)$ such that for all $t \geq T_\varepsilon^1(a^\infty,y^\infty)$,
\begin{equation} \label{eq:uLLN}
\sup_{\theta \in \Theta} |L_t(a^\infty,y^\infty)(\theta)-\int K(\theta,a)\sigma_{t}(a^\infty)(da)|<\varepsilon.
\end{equation}
See Section \ref{sub:uLLN} for a proof of this result.


From this point on, we fix any $a^\infty$ and consider any $y^\infty \in \mathcal{Y}_{a^\infty}$. For simplicity, we drop $(a^\infty,y^\infty)$ from the notation. Let $(\sigma_{t_k})_{k}$ be a subsequence converging to $\sigma$ and let $E\subseteq \Theta$ be a closed set disjoint from $\Theta^m(\sigma)$. We rely on the following two results: 

\emph{Approximate $(\sigma_{t_k})_{k}$ with its limit $\sigma$.} Since $K$ is continuous and $\Theta$ is compact, then for every $\varepsilon>0$, there exists $T_\varepsilon^2$ such that, for all $k$ such that $t_{k} \geq T_\varepsilon^2$,
\begin{equation*}
    \sup_{\theta \in \Theta} |\int K(\theta,a)\sigma_{t_k}(da)-\int K(\theta,a)\sigma(da)|<\varepsilon.
\end{equation*}

\emph{$E$ is well separated.} Since $K$ is continuous and $E$ is closed in a compact set (hence, compact), there exists $\delta>0$ such that for all $\theta \in E$, 
\[
\int K(\theta,a)\sigma(da)\geq K^*(\sigma)+\delta,
\]
where $K^*(\sigma):=\min_{\theta \in \Theta} \int K(\theta,a)\sigma(da)$.


We now prove (\ref{eq:exponential}) in Lemma \ref{lemm:Berk-selected}. For any $\xi>0$, note that 
\[
\mu_{t_k}(E)=\frac{\int_E e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta)}{\int_\Theta e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta)} \leq \frac{\int_E e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta)}{\int_{\Theta_\xi(\sigma)} e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta)},
\]
where $\Theta_\xi(\sigma):=\{\theta \in \Theta:\int K(\theta,a)\sigma(da)\leq K^*(\sigma)+\xi\}$.

Consider first the numerator. From UniformSLLN, the approximation of $(\sigma_{t_k})_{k}$ with its limit $\sigma$, and well separation of $E$, it follows that, for all $k$ such that $t_k\geq \max\{T_\varepsilon^1,T_\varepsilon^2\}$, $L_{t_k}(\theta) \geq K^*(\sigma) + \delta - 2\varepsilon$ for all $\theta \in E$, and so
\begin{equation} \label{eq:numerator}
\int_E e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta)\leq \mu_0(E) e^{-t_k(K^*(\sigma)+\delta - 2\varepsilon)}.
\end{equation}

Next, consider the denominator. From UniformSLLN and the approximation of $(\sigma_{t_k})_{k}$ with its limit $\sigma$, it follows that, for all $k$ such that $t_k\geq \max\{T_\varepsilon^1,T_\varepsilon^2\}$, $L_{t_k}(\theta) \leq K^*(\sigma) + \xi + 2\varepsilon$ for all $\theta \in \Theta_\xi(\sigma)$, and so
\begin{equation} \label{eq:denomirator}
\int_{\Theta_\xi(\sigma)} e^{-t_k L_{t_k}(\theta)}\mu_0(d\theta) \geq \mu_0(\Theta_\xi(\sigma)) e^{-t_k(K^*(\sigma)+\xi+2\varepsilon)}. 
\end{equation}

Combining (\ref{eq:numerator}) and (\ref{eq:denomirator}) and setting $\varepsilon=\xi<\delta/10$, we obtain that for all $k$ such that $t_k\geq \max\{T_\varepsilon^1,T_\varepsilon^2\}$,
\[
\mu_{t_k}(E) \leq \frac{\mu_0(E)}{\mu_0(\Theta_\xi(\sigma))} e^{-t_k(\delta/2)}.
\]
Since \( \Theta \) is compact and \( \theta \mapsto \int K(\theta,a)\sigma(da) \) is continuous, a minimizer \( \theta^* \in \Theta \) exists and satisfies \( \theta^* \in \Theta_\xi(\sigma) \). By continuity, there exists an open ball around \( \theta^* \) contained in \( \Theta_\xi(\sigma) \). Since \( \mu_0 \) has full support, this ball has positive measure, so \( \mu_0(\Theta_\xi(\sigma)) > 0 \). Equation (\ref{eq:exponential}) in the statement of Lemma \ref{lemm:Berk-selected} then follows by setting $\rho=\delta/2>0$ and $C=\mu_0(E)/\mu_0(\Theta_\xi(\sigma))$. Since \( \mu_0(E) \geq 0 \) and \( \mu_0(\Theta_\xi(\sigma)) > 0 \), it follows that \( C \geq 0 \) and \( C < \infty \).

Suppose, in addition, that $(\mu_{t_k})_{k}$ converges to $\mu$. By equation (\ref{eq:exponential}), for any closed $E$ such that $E \cap \Theta^m(\sigma)=\emptyset$, $\lim\inf_{k\rightarrow \infty} \mu_{t_k}(E)=0$. By the Pormanteau lemma, $\mu(E)\leq \lim\inf_{k\rightarrow \infty} \mu_{t_k}(E)=0$. Now consider any $\theta \in \Theta \setminus \Theta^m(\sigma)$. There exists an open neighborhood $U_\theta$ with closure $\bar{U}_\theta$ such that $\bar{U}_\theta \cap \Theta^m(\sigma) =\emptyset$. Since $\bar{U}_\theta$ is closed, $\mu(\bar{U}_\theta)=0$, and so $\theta$ is not in the support of $\mu$. Thus, $supp \hspace{2pt} \mu \subseteq \Theta^m(\sigma)$.


\subsection{Uniform SLLN} \label{sub:uLLN}


\cite{esponda2021asymptotic} (henceforth, EPY 2021) proves the uniform SLLN (equation \ref{eq:uLLN}) for the case of a finite number of actions (see their Lemma 2). The proof for the case where $\mathbb{A}^{i}$ is a compact subset of Euclidean space is essentially identical, but we need to establish the following two claims uniformly for all actions. 

\paragraph{Claim (uniform $L^2$ bound for $g$).}
Fix $i$, $\theta\in\Theta^i$, and $\varepsilon>0$. Then
\[
\sup_{a\in\mathbb A}\int_{\mathbb{Y}^i}\sup_{\theta'\in O(\theta,\varepsilon)}
\bigl[g^i(\theta',y,a)\bigr]^2\,Q^i(dy\mid a)\ <\ \infty.
\]

\emph{Proof.}
For any $a$,
\[
\int \sup_{\theta'\in O(\theta,\varepsilon)} \bigl[g^i(\theta',y,a)\bigr]^2\,Q^i(dy\mid a)
= \int \sup_{\theta'} \Bigl|\log\frac{q^i(y\mid a)}{q^i_{\theta'}(y\mid a)}\Bigr|^{2}\, q^i(y\mid a)\,\nu^i(dy).
\]
By the LR bound, $\sup_{\theta'}\bigl|\log(q^i/q^i_{\theta'})\bigr|\le \log M^i\le M^i$ a.e., hence
\[
\int \sup_{\theta'\in O(\theta,\varepsilon)} \bigl[g^i(\theta',y,a)\bigr]^2\,Q^i(dy\mid a) \le \int \bigl(\log M^i(y)\bigr)^{2}\, q^i(y\mid a)\,\nu^i(dy)\ \le\ 2\int M^i(y)\, q^i(y\mid a)\,\nu^i(dy),
\]
where we used $(\log t)^2\le 2t$ for $t\ge1$. By the density envelope, $q^i(\cdot\mid a)\le r^i$ a.e., so
\[
\int \sup_{\theta'\in O(\theta,\varepsilon)} \bigl[g^i(\theta',y,a)\bigr]^2\,Q^i(dy\mid a) \le 2\int M^i(y)\, r^i(y)\,\nu^i(dy),
\]
which is finite by Assumption~\ref{ass:game}(iii) and independent of $a$. Taking the supremum over $a\in\mathbb A$ gives the claim. \qed

\paragraph{Claim (uniform oscillation bound, eq.\ (12) in EPY 2021).}
Fix $i$, $\theta\in\Theta^i$, and $\varepsilon>0$. Then there exists $\delta(\theta,\varepsilon)>0$ such that
\[
\sup_{a\in\mathbb A}\ \mathbb E_{Q^i(\cdot\mid a)}
\Big[\ \sup_{\theta'\in O(\theta,\delta(\theta,\varepsilon))}
\big|g^i(\theta',Y,a)-g^i(\theta,Y,a)\big|\ \Big]\ <\ 0.25\,\varepsilon .
\]

\emph{Proof.}
Let $H_r(y):=\sup_{\|\theta'-\theta\|\le r,\ a\in\mathbb A}\big|g^i(\theta',y,a)-g^i(\theta,y,a)\big|$. 
By a.e.-continuity on the compact set $\Theta^i\times\mathbb A$ (Assumption~\ref{ass:game}(ii)), $H_r(y)\downarrow0$ for $\nu^i$-a.e.\ $y$ as $r\downarrow0$. 
By the LR bound (Assumption~\ref{ass:game}(iii)), $H_r(y)\le 2|g^i(\theta,y,a)|\le 2\log M^i(y)\le 2M^i(y)$ a.e., and by the density envelope $Q^i(dy\mid a)=q^i(y\mid a)\nu^i(dy)\le r^i(y)\nu^i(dy)$. Hence, for every $a$,
\[
\mathbb E_{Q^i(\cdot\mid a)}\!\Big[\sup_{\theta'\in O(\theta,r)}|g^i(\theta',Y,a)-g^i(\theta,Y,a)|\Big]
\le \int H_r(y)\,q^i(y\mid a)\,\nu^i(dy)
\le \int H_r(y)\,r^i(y)\,\nu^i(dy).
\]
Since $H_r\to0$ a.e. and $H_r(\cdot)\,r^i(\cdot)\le 2M^i(\cdot)\,r^i(\cdot)$ with $\int 2M^i r^i\,d\nu^i<\infty$ (Assumption~\ref{ass:game}(iii)), the Dominated Convergence Theorem yields $\int H_r r^i\,d\nu^i\to0$ as $r\downarrow0$. Thus
\[
\sup_{a\in\mathbb A}\ \mathbb E_{Q^i(\cdot\mid a)}\!\Big[\sup_{\theta'\in O(\theta,r)}|g^i(\theta',Y,a)-g^i(\theta,Y,a)|\Big]
\le \int H_r r^i\,d\nu^i\ \xrightarrow[r\downarrow0]{}\ 0.
\]
Choose $\delta(\theta,\varepsilon)>0$ so that the right-hand side is $<0.25\,\varepsilon$. \qed





\begin{comment}
We point out the two places where the more general $\mathbb{A}^{i}$ makes a difference.

The following results hold for any $i \in I$.

In Step 1 of their proof, they use the fact that there is a function $g_a \in L^2(\mathbb{Y},\mathbb{R},Q(\cdot \mid a))$ such that $\sup_{\theta' \in O(\theta^{i},\varepsilon)}(g(\theta',y,a))^2 \leq (g_a(y))^2$, where $g(\theta,y,a):=\log(q^{i}(y\mid a)/q^{i}_{\theta^{i}}(y \mid a))$ and $O(\theta,\varepsilon):=\{\theta' \in \Theta^{i} :||\theta'-\theta^{i} ||<\varepsilon\}$. In our case, we need a function $G^{i}$ that does not depend on $a$. Formally, $\max_{a \in \mathbb{A} } \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy) < \infty $. 

To do this, let $G^{i} : = \log M^{i}$. By Assumption \ref{ref:Ass:game}(iv)
\begin{align*}
    \log \frac{q^{i}(\cdot \mid a)}{q^{i}_{\theta^{i}} (\cdot \mid a)} \in \left[ - \log M^{i}(\cdot) , \log M^{i}(\cdot) \right]
\end{align*}
for any $(a,\theta^{i}) \in \mathbb{A} \times \Theta^{i}$. 

Under assumption \ref{ref:Ass:game}(iii)(iv), $a \mapsto |G^{i}(\cdot)|^{2} q^{i}(\cdot | a)$ is continuous a.e.-$\nu^{i}$  and it is dominated by $h^{i} \in L^{1}(\mathbb{Y}^{i},\nu^{i})$. Thus, by the DCT, $a \mapsto \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy)$ is continuous. And since $\mathbb{A}$ is compact (Assumption \ref{ref:Ass:game}(i)), $\max_{a \in \mathbb{A}} \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy) < \infty $ as desired. 

In Step 2 of their proof, they conclude that, for each $\theta^{i} \in \Theta^{i}$, $ \Lambda_{\delta}(a) : =   \int  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a)-g(\theta^{i},y,a)| Q^{i}(dy|a)$ vanishes as $\delta$ converges to zero. The proof requires convergence to be uniform in $\mathbb{A}$, which is immediate if $\mathbb{A}$ is finite. We now establish such uniform convergence for our more general case. By pointwise convergence and the Arzela-Ascoli Theorem, it suffices to establish equicontinuity of the class $(\Lambda_{\delta})_{\delta \geq 0}$. To do so, take any $\epsilon>0$ and observe that for any $a,a' \in \mathbb{A}$,
\begin{align*}
    |  \Lambda_{\delta}(a) -  \Lambda_{\delta}(a') | \leq & \left| \int  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a')-g(\theta^{i},y,a')| (q^{i}(y|a) - q^{i}(y|a') ) \nu^{i} (dy) \right|  \\
    & + \left| \int  \sup_{\theta' \in O(\theta^{i},\delta)} | \log q^{i}_{\theta'}(y \mid a) - \log q^{i}_{\theta'}(y \mid a') | q^{i}(y|a) \nu^{i}(dy) \right|\\
     = : & I + II.
\end{align*}
Under Assumption \ref{ref:Ass:game}(iv), the term $I$ bounded by $ 2 \int G^{i}(y) |q^{i}(y|a) - q^{i}(y|a') | \nu^{i}(dy)$. Under assumption \ref{ref:Ass:game}(iii), there exists a $\gamma>0$ (not dependent on $\delta$) such that $ 2 \int G^{i}(y) |q^{i}(y|a) - q^{i}(y|a') | \nu^{i} (dy) \leq 0.5 \epsilon$ for any $a,a'$ such that $||a-a'||\leq \gamma$. 

Regarding the term $II$, under Assumptions \ref{ref:Ass:game}(iii)(iv), $\log \frac{q^{i}_{\theta'}(y \mid a)}{q^{i}(y \mid a)} \geq \log M^{i}(y) > - \infty$, so $(\theta^{i},a) \mapsto  \log q^{i}_{\theta^{i}}(y \mid a)$ is jointly uniformly continuous. Therefore, for any $\epsilon'>0$ and $Q^{i}(\cdot | a)$-almost all $y$, there exists a $\gamma'_{y}>0$ (not dependent on $\theta^{i}$) such that $| \log q^{i}_{\theta'}(y \mid a) - \log q^{i}_{\theta'}(y \mid a') | \leq \epsilon'$ for all $a,a'$  such that $||a-a'||\leq \gamma'_{y}$. Hence, $\sup_{\theta' \in O(\theta^{i},\delta)} | \log q^{i}_{\theta'}(y \mid a) - \log q^{i}_{\theta'}(y \mid a') | \leq \epsilon'$ for all such $a,a'$. By the DCT, under Assumption \ref{ref:Ass:game}(iv), this result implies that there exists a $\gamma'$ such that the term $II$ is bounded by  $\epsilon'$ for all $a,a'$  such that $||a-a'||\leq \gamma'$. 

By taking $\epsilon'= 0.5 \epsilon$, these results show that for all $a,a'$ such that $||a-a'||\leq \min\{ \gamma,\gamma'\} $, 
\begin{align*}
    |  \Lambda_{\delta}(a) -  \Lambda_{\delta}(a') | \leq \epsilon
\end{align*}
for any $\delta \geq 0$, thus establishing equi-continuity as desired.

\end{comment}

\begin{comment}
    

\subsection{Comment on Limit frequencies}

Let $\sigma^{i}_{t} \in \Delta \mathbb{A}^{-i}$ be the empirical frequency for player $i$ over other players actions. 

Let $a_{1:t-1}$ be the history of all actions up to time $t$. Let $Pr^{i}_{t}(\cdot \mid a_{1:t-1})$ be the conditional probability distribution over other players actions, given $a_{1:t}$.  

By the MCT, for any $f \in C_{b}(\mathbb{A}^{-i})$, 
\begin{align}
| \int f(a^{-i}) \sigma^{i}_{t}(da^{-i})  - \int f(a^{-i}) t^{-1} \sum_{\tau=1}^{t} Pr^{i}_{\tau}(d a^{-i} \mid a_{1:\tau-1}) | = o_{as}(1).
\end{align}

Therefore, for any subsequence $(t_{k})_{k}$, a limit $\sigma^{-i}$ of $(\sigma^{i}_{t_{k}})_{k}$, is of the form $\lim_{k \to \infty} t_{k}^{-1} \sum_{\tau=1}^{t_{k}} Pr^{i}_{\tau}( \cdot \mid a_{1:\tau-1})$. 

Suppose the following: For any $t$ and any $a_{1:t-1}$, $Pr^{i}_{t}( \prod_{j \ne i} A_{j} \mid a_{1:t-1}) = \prod_{j \ne i} \Phi^{j}_{t} (A_{j} \mid a_{1:t-1})$.

Observe that 
\begin{align}
    \sigma^{i}(\cdot) = \lim_{k \to \infty} t_{k}^{-1} \sum_{\tau=1}^{t_{k}} Pr^{i}_{\tau}( \cdot \mid a_{1:\tau-1})
\end{align}

\end{comment}

\begin{comment}
\section{Continuity \& other results}

\begin{assumption}\label{ass:compact}
    $\Theta^{i}$ and $\mathbb{A}^{i}$ are compact subsets of finite dimensional Euclidean spaces.
\end{assumption}

\begin{assumption}\label{ass:cont}
   (i) $a \mapsto q^{i}(\cdot \mid a)$ and $(a,\theta^{i}) \mapsto q^{i}_{\theta^{i}}(\cdot \mid a)$ are continuous a.e.-$\nu^{i}$, (ii) $(y^{i},a) \mapsto \pi^{i}(y^{i},a)$ is continuous a.e.-$\nu^{i}$.
\end{assumption}

\begin{assumption}[LR: two-sided domination by a measurable $M$]\label{ass:ratio.q}
There exists a measurable $M^{i} :\mathbb Y\to[1,\infty)$ such that, for all $(\theta^{i},a)\in\Theta^{i}\times \mathbb{A}$,
\[
q^{i}_{\theta^{i}} (\cdot \mid a)\,M^{i}(\cdot)^{-1}\ \le\ q^{i}( \cdot \mid a)\ \le q^{i}_{\theta^{i}}( \cdot \mid a) M^{i}( \cdot)
\qquad\text{a.e.-$\nu^{i}$}
\]
\end{assumption}

\begin{assumption}\label{ass:vitali}
   % There exists a $\delta>0$ such that $\sup_{XXX} \int_{\mathbb{Y}^{i}} |\log M^{i}(y) |^{2(1+\delta)} |XXX| \nu^{i}(dy) < \infty$ 
   There exists a $\delta>0$ such that $\sup_{a \in \mathbb{A}}  \int_{\mathbb{Y}} \max\{1, |\pi^{i}(y,a)|\}^{1+\delta}  M^{i}(y)  |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy) < \infty$. 
\end{assumption}

Implied by (more direct) assumption:
\begin{assumption}
   There exists a $p,q,r \in [1,+\infty]$ such that $1/p+1/q+1/r=1$, $\sup_{a \in \mathbb{A}}  \int_{\mathbb{Y}} |\pi^{i}(y,a)|^{p(1+\delta)} \nu^{i}(dy) < \infty$, $\sup_{a \in \mathbb{A}}  \int_{\mathbb{Y}}  |q^{i}(y\mid a)|^{q(1+\delta)} \nu^{i}(dy) < \infty$, and $ \int_{\mathbb{Y}}  |M^{i}(y)|^{r(1+\delta)} \nu^{i}(dy) < \infty$.
\end{assumption}

The following lemma is based on the Vitali uniform integration Theorem and is used to establish continuity of intergrals.

\begin{lemma}\label{lem:Vitali}
    Let $\mathbb{B}$ be a compact subset of a finite dimensional Euclidean space and $(\mathbb{X},\Lambda)$ be a measurable space. Consider a class of functions $(f_{b})_{b \in \mathbb{B}}$ such that $f_{b} : \mathbb{X} \rightarrow \mathbb{R}$ and 
    \begin{enumerate}
        \item $b \mapsto f_{b}(\cdot)$ is continuous a.s.-$\Lambda$.
        \item There exists a $\delta>0$ such that $\sup_{b \in \mathbb{B}} \int_{\mathbb{X}} |f_{b}(x)|^{1+\delta} \Lambda(dx) < \infty$. 
    \end{enumerate}
    Then $b \mapsto \int_{\mathbb{X}} f_{b} (x)\Lambda(dx)$ is uniformly continuous.
\end{lemma}

\begin{proof}
Condition two implies uniform integrability of the class $(f_{b})_{b \in \mathbb{B}}$. To see this, note that for any $K>0$, by the Markov inequality,
\begin{align*}
   \sup_{b \in \mathbb{B}} \int_{\mathbb{X}} 1\{ |f_{b}(x)| \geq K\} |f_{b}(x)| \Lambda(dx) \leq  K^{-\delta} \sup_{b \in \mathbb{B}} \int_{\mathbb{X}} |f_{b}(x)|^{1+\delta} \Lambda(dx)
\end{align*}
for any $\delta>0$. Chosing the $\delta>0$ as in the condition 2, we obtain a bound of the form $K^{-\delta} L$ for some finite $L$. Thus, for any $\epsilon>0$, there exists a $K_{\epsilon}$ sufficiently large for which $  \sup_{b \in \mathbb{B}} \int_{\mathbb{X}} 1\{ |f_{b}(x)| \geq K\} |f_{b}(x)| \Lambda(dx) > \epsilon$ for all $K \geq K_{\epsilon}$.

Thus, the desired result follows from Vitali's uniform integration theorem (XXX). 
\end{proof}

\begin{lemma}\label{lem:logM.bound}
   For any $\delta \in [0,e-1]$, $|\log M^{i}(\cdot)|^{1+\delta} \leq |M^{i}(\cdot)|$.  
\end{lemma}


\begin{proof}

Set $x=\log M\ge 0$. The claim is $x^{1+\delta}<e^x$. Consider 
\[
f(x)=\frac{x^{1+\delta}}{e^x}, \qquad x\ge 0.
\]
Then $\log f(x)=(1+\delta)\log x - x$, so $f$ attains its maximum at $x=1+\delta$. Hence
\[
\sup_{x\ge 0} f(x)=\frac{(1+\delta)^{1+\delta}}{e^{1+\delta}}.
\]
Thus $f(x)<1$ for all $x$ iff $(1+\delta)^{1+\delta}<e^{1+\delta}$, i.e. $1+\delta<e$. 
\end{proof}


\paragraph{CLaim:} $K^{i}$ is continuous.

\begin{proof}
    To show this claim we apply Lemma \ref{lem:Vitali} to $\mathbb{B} : = \Theta^{i} \times \mathbb{A}$, which is compact; $\mathbb{X} = \mathbb{Y}^{i}$ and $\Lambda = \nu^{i}$; and the family of functions $\left( q^{i}(\cdot \mid a) \log \frac{q^{i}(\cdot|a)}{q^{i}_{\theta^{i}}(\cdot|a)}   \right)_{(\theta^{i},a) \in \Theta^{i} \times \mathbb{A}} $. We now verify the assumptions of the lemma.

    By Assumption XXX, $(\theta^{i},a) \mapsto q^{i}_{\theta^{i}}(\cdot | a)$ and $(\theta^{i},a) \mapsto q^{i}(\cdot | a)$ are continuous a.e.-$\nu^{i}$. By Assumption XXX (USE $M$) $q^{i}(\cdot \mid a) \log \frac{q^{i}(\cdot|a)}{q^{i}_{\theta^{i}}(\cdot|a)} $ XXX


    We now verify condition (2) in the Lemma \ref{lem:Vitali}. To do this, observe that 
    \begin{align*}
        \int_{\mathbb{Y}} \left| \log \frac{q^{i}(\cdot|a)}{q^{i}_{\theta^{i}}(\cdot|a)}    \right|^{1+\delta} |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy) \leq &  \int_{\mathbb{Y}} |\log M^{i}(y) |^{1+\delta} |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy)
    \end{align*}
    where the first inequality follows from Assumption \ref{ass:ratio.q}. By Lemma \ref{lem:logM.bound}, $\int_{\mathbb{Y}} |\log M^{i}(y) |^{1+\delta} |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy) \leq \int_{\mathbb{Y}} |M^{i}(y) | |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy)$, which is uniformly bounded by Assumption \ref{ass:vitali}. Thus condition (2) is verified.
\end{proof}


\paragraph{Claim.} $(a^{i},\theta^{i},a^{-i}) \mapsto  \bar{U}^i(a^i,\theta^i,a^{-i})\;:=\;\int_{\mathbb Y^i}\pi^i(a^i,y^i)\,q^i_{\theta^i}(y^i\mid a^i,a^{-i})\,\nu^i(dy^i)$ is continuous.

\begin{proof}
    To show this claim we apply Lemma \ref{lem:Vitali} to $\mathbb{B} : = \mathbb{A}^{i} \times \Theta^{i} \times \mathbb{A}^{-i}$, which is compact; $\mathbb{X} = \mathbb{Y}^{i}$ and $\Lambda = \nu^{i}$; and the family of functions $\left( \pi^i(a^{i},\cdot)\,q^i_{\theta^i}(\cdot\mid a^i,a^{-i})  \right)_{(a^{i},\theta^{i},a^{-i}) \in \mathbb{A}^{i} \times \Theta^{i} \times \mathbb{A}^{-i}} $. We now verify the assumptions of the lemma.

    Condition (1) follows by Assumption \ref{ass:cont} which implies that $(a^{i},\theta^{i},a^{-i}) \mapsto  \pi^i(a^{i},\cdot)\,q^i_{\theta^i}(\cdot\mid a^i,a^{-i}) $ is continuous a.s.-$\nu^{i}$. Condition (2) follows because
        \begin{align*}
        \int_{\mathbb{Y}} |\pi^i(a^{i},y) q^i_{\theta^i}(y\mid a^i,a^{-i})|^{1+\delta}  \nu^{i}(dy) \leq &  \int_{\mathbb{Y}} | \pi^i(a^{i},y) |^{1+\delta} |M^{i}(y)|^{1+\delta} |q^{i}(y\mid a)|^{1+\delta} \nu^{i}(dy)
    \end{align*}
    is uniformly bounded under Assumption \ref{ass:vitali}.
\end{proof}



\paragraph{Claim:} For any $\theta^{i} \in \Theta^{i}$, $\max_{a \in \mathbb{A} } \int_{\mathbb{Y}^{i}} |\sup_{\theta' \in O(\theta^{i},\varepsilon)}(g(\theta',y,a))|^{2} q^{i}(y|a) \nu^{i}(dy) < \infty $. 

\begin{proof}
    To do this, let $G^{i} : = \log M^{i}$. By Assumption \ref{ass:ratio.q}
\begin{align*}
    \log \frac{q^{i}(\cdot \mid a)}{q^{i}_{\theta^{i}} (\cdot \mid a)} \in \left[ - \log M^{i}(\cdot) , \log M^{i}(\cdot) \right]
\end{align*}
for any $(a,\theta^{i}) \in \mathbb{A} \times \Theta^{i}$. Thus,  $\max_{a \in \mathbb{A} } \int_{\mathbb{Y}^{i}} |\sup_{\theta' \in O(\theta^{i},\varepsilon)} g(\theta',y,a)|^{2} q^{i}(y|a) \nu^{i}(dy) \leq \max_{a \in \mathbb{A} } \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy) $. This quantity is finite. To show this note that $|G^{i}(y)|^{2} \leq |M^{i}(y)|$ by Lemma \ref{lem:logM.bound}. Thus, $\int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy) \leq \int_{\mathbb{Y}^{i}} |M^{i}(y)| q^{i}(y|a) \nu^{i}(dy)$ which is uniformly bounded under Assumption \ref{ass:vitali}.



%Under assumption \ref{ass:cont}, $a \mapsto |G^{i}(\cdot)|^{2} q^{i}(\cdot | a)$ is continuous a.e.-$\nu^{i}$.   and it is dominated by $h^{i} \in L^{1}(\mathbb{Y}^{i},\nu^{i})$. Thus, by the DCT, $a \mapsto \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy)$ is continuous. And since $\mathbb{A}$ is compact (Assumption \ref{ass:compact}), $\max_{a \in \mathbb{A}} \int_{\mathbb{Y}^{i}} |G^{i}(y)|^{2} q^{i}(y|a) \nu^{i}(dy) < \infty $ as desired. 

\end{proof}

for each $\theta^{i} \in \Theta^{i}$, $a \mapsto \Lambda_{\delta}(a) : =   \int_{\mathbb{Y}^{i}}  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a)-g(\theta^{i},y,a)| Q^{i}(dy|a)$. 

\paragraph{Claim:} $(\Delta_{\delta})_{\delta \geq 0}$ is equi-continuous.


\begin{proof}
    Take any $\epsilon>0$ and observe that for any $a,a' \in \mathbb{A}$,
\begin{align*}
    |  \Lambda_{\delta}(a) -  \Lambda_{\delta}(a') | \leq & \left| \int_{\mathbb{Y}^{i}} \left\{   \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a)-g(\theta^{i},y,a)| q^{i}(y|a) -  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a')-g(\theta^{i},y,a')| q^{i}(y|a') \right\} \nu^{i}(dy) \right| \\
    \leq & \left|  \int_{\mathbb{Y}^{i}} \left\{   \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a)-g(\theta^{i},y,a)| (q^{i}(y|a) -  q^{i}(y|a'))  \right\} \nu^{i}(dy) \right| \\
    & + \left|  \int_{\mathbb{Y}^{i}} \left\{   \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a)-g(\theta^{i},y,a)|  -  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a')-g(\theta^{i},y,a')|  \right\} q^{i}(y|a) \nu^{i}(dy) \right| \\
    \leq & \left| \int  \sup_{\theta' \in O(\theta^{i},\delta)} |g(\theta',y,a')-g(\theta^{i},y,a')| (q^{i}(y|a) - q^{i}(y|a') ) \nu^{i} (dy) \right|  \\
    & + \left| \int  \sup_{\theta' \in O(\theta^{i},\delta)} | \log g(\theta',y,a)  - g(\theta',y,a')| q^{i}(y|a) \nu^{i}(dy) \right|\\
     = : & I + II.
\end{align*}
Under Assumption \ref{ass:ratio.q}, the term $I$ bounded by $ 2 \int |\log M^{i}(y)| |q^{i}(y|a) - q^{i}(y|a') | \nu^{i}(dy)$. Under assumption \ref{ass:cont}, $a \mapsto q^{i}(\cdot | a)$ is continuous a.e.-$\nu^{i}$. Moreover, $ \int_{\mathbb{Y}^{i}} |\log M^{i}(y)| |q^{i}(y|a) - q^{i}(y|a') | \nu^{i}(dy) \leq 2 \sup_{a \in \mathbb{A}} \int_{\mathbb{Y}^{i}} |\log M^{i}(y) |q^{i}(y|a) \nu^{i}(dy) $ which is bounded by Assumption \ref{ass:vitali} and Lemma \ref{lem:logM.bound}. Therefore, there exists a $\gamma>0$ (not dependent on $\delta$) such that $ 2 \int |\log M^{i}(y)| |q^{i}(y|a) - q^{i}(y|a') | \nu^{i} (dy) \leq 0.5 \epsilon$ for any $a,a'$ such that $||a-a'||\leq \gamma$. 

Regarding the term $II$, under Assumption  \ref{ass:ratio.q}, $g(\theta',y,a) = \left|  \log \frac{q^{i}_{\theta'}(y \mid a)}{q^{i}(y \mid a)} \right| \geq \log M^{i}(y) < \infty$, so by Assumption \ref{ass:cont}, $(\theta^{i},a) \mapsto  \log q^{i}_{\theta^{i}}(y \mid a)$ is jointly uniformly continuous. Therefore, for any $\epsilon'>0$ and $Q^{i}(\cdot | a)$-almost all $y$, there exists a $\gamma'_{y}>0$ (not dependent on $\theta^{i}$) such that $| \log q^{i}_{\theta'}(y \mid a) - \log q^{i}_{\theta'}(y \mid a') | \leq \epsilon'$ for all $a,a'$  such that $||a-a'||\leq \gamma'_{y}$. Hence, $\sup_{\theta' \in O(\theta^{i},\delta)} | \log q^{i}_{\theta'}(y \mid a) - \log q^{i}_{\theta'}(y \mid a') | \leq \epsilon'$ for all such $a,a'$. 

Also $\int_{\mathbb{Y}^{i}} |\sup_{\theta' \in O(\theta^{i},\delta)} (| \log g(\theta',y,a)  - g(\theta',y,a')| q^{i}(y|a))^{1+\delta} \nu^{i}(dy) \leq \int_{\mathbb{Y}^{i}} |\log M^{i}(y)|^{1+\delta} (q^{i}(y|a))^{1+\delta} \nu^{i}(dy)  $ which is uniformly bounded by Assumption \ref{ass:vitali} and Lemma \ref{lem:logM.bound}. 

Thus, Lemma \ref{lem:Vitali} implies that there exists a $\gamma'$ such that the term $II$ is bounded by  $\epsilon'$ for all $a,a'$  such that $||a-a'||\leq \gamma'$. 

By taking $\epsilon'= 0.5 \epsilon$, these results show that for all $a,a'$ such that $||a-a'||\leq \min\{ \gamma,\gamma'\} $, 
\begin{align*}
    |  \Lambda_{\delta}(a) -  \Lambda_{\delta}(a') | \leq \epsilon
\end{align*}
for any $\delta \geq 0$, thus establishing equi-continuity as desired.

\end{proof}


\subsection{Old}


\subsection{Assumptions}

\begin{assumption}[S1: Compact parameter spaces]
\(\Theta^{i}\) and \(\mathbb{A}^{i}\) are compact metric spaces.
\end{assumption}

\begin{assumption}[S2: a.e.-continuity]
For \(\nu^{i}\)-a.e.\ \(y\in\mathbb{Y}^{i}\):
\[
a\mapsto q^{i}(y\mid a)\ \text{is continuous},\qquad
(\theta^{i},a)\mapsto q^{i}_{\theta^{i}}(y\mid a)\ \text{is continuous},\qquad
(a^{i},y)\mapsto \pi^{i}(a^{i},y)\ \text{is continuous}.
\]
\end{assumption}

\begin{assumption}[S3: Likelihood–ratio bound (LR)]
There exists a measurable \(M^{i}:\mathbb{Y}^{i}\to[1,\infty)\) such that, for all \((\theta^{i},a)\in\Theta^{i}\times\mathbb{A}^{i}\),
\[
q^{i}_{\theta^{i}}(\cdot\mid a)\,M^{i}(\cdot)^{-1}\ \le\ q^{i}(\cdot\mid a)\ \le\ q^{i}_{\theta^{i}}(\cdot\mid a)\,M^{i}(\cdot)
\quad\text{a.e.-}\nu^{i}.
\]
In particular, \(\bigl|\log\!\tfrac{q^{i}}{q^{i}_{\theta^{i}}}\bigr|\le |\log M^{i}|\) and \(q^{i}=0\iff q^{i}_{\theta^{i}}=0\) \(\nu^{i}\)-a.e.
\end{assumption}

\begin{assumption}[S4$'$: One-line integrability (Vitali/DCT payload)]
There exist \(\delta\in(0,1]\) and \(C<\infty\) such that
\[
\sup_{a\in\mathbb{A}^{i},\,\theta^{i}\in\Theta^{i}}
\int_{\mathbb{Y}^{i}}
\Big(
\big|\log\tfrac{q^{i}(y\mid a)}{q^{i}_{\theta^{i}}(y\mid a)}\big|^{2}
+ M^{i}(y)
+ (1+|\pi^{i}(a^{i},y)|)^{1+\delta}\,M^{i}(y)
\Big)\,
q^{i}(y\mid a)\,d\nu^{i}(y)
\ \le\ C .
\]
\end{assumption}

\subsection{KL}

\begin{lemma}
For each \(i\), the KL–minimizer correspondence \(\Theta^{m,i}(\sigma)\subseteq \Theta^{i}\) is nonempty, compact-valued, and upper hemicontinuous in \(\sigma\).
\end{lemma}

\begin{proof}
Write \(g^{i}(\theta^{i},y,a):=\log\!\big(q^{i}(y\mid a)/q^{i}_{\theta^{i}}(y\mid a)\big)\) and
\(K^{i}(\theta^{i},a):=\int_{\mathbb Y^{i}} g^{i}(\theta^{i},y,a)\,q^{i}(y\mid a)\,d\nu^{i}(y)\).
For \(\sigma\in\Delta(\mathbb A)\), set \(\mathcal K^{i}(\theta^{i},\sigma):=\int_{\mathbb A} K^{i}(\theta^{i},a)\,\sigma(da)\) and
\(\Theta^{m,i}(\sigma):=\arg\min_{\theta^{i}\in\Theta^{i}}\mathcal K^{i}(\theta^{i},\sigma)\).

\paragraph{Step 1 (Mutual absolute continuity).}
From LR (S3), \(q^{i}_{\theta^{i}}(\cdot\mid a)\,M^{i}(\cdot)^{-1}\le q^{i}(\cdot\mid a)\le q^{i}_{\theta^{i}}(\cdot\mid a)\,M^{i}(\cdot)\) a.e.-\(\nu^{i}\).
Hence \(q^{i}(\cdot\mid a)=0\) iff \(q^{i}_{\theta^{i}}(\cdot\mid a)=0\) a.e.-\(\nu^{i}\), i.e. \(Q^{i}(\cdot\mid a)\sim Q^{i}_{\theta^{i}}(\cdot\mid a)\) for every \((\theta^{i},a)\).

\paragraph{Step 2 (\(K^{i}\) finite, uniformly bounded, and jointly continuous).}
Let \((\theta^{i}_{n},a_{n})\to(\theta^{i},a)\).
By a.e.-continuity (S2),
\(q^{i}(y\mid a_{n})\to q^{i}(y\mid a)\) and \(q^{i}_{\theta^{i}_{n}}(y\mid a_{n})\to q^{i}_{\theta^{i}}(y\mid a)\) for \(\nu^{i}\)-a.e.\ \(y\).
Define \(f_{n}(y):=q^{i}(y\mid a_{n})\,g^{i}(\theta^{i}_{n},y,a_{n})\) and \(f(y):=q^{i}(y\mid a)\,g^{i}(\theta^{i},y,a)\).
If \(q^{i}_{\theta^{i}}(y\mid a)>0\), then, using Step~1 and continuity of \((u,v)\mapsto u\log(u/v)\) on \(\{u\ge 0,v>0\}\), we have \(f_{n}(y)\to f(y)\).
If \(q^{i}_{\theta^{i}}(y\mid a)=q^{i}(y\mid a)=0\), then LR (S3) gives \(|g^{i}(\theta^{i}_{n},y,a_{n})|\le |\log M^{i}(y)|<\infty\) while \(q^{i}(y\mid a_{n})\to0\), hence \(f_{n}(y)\to 0=f(y)\).
Thus \(f_{n}\to f\) a.e.
By (S4), \(\sup_{n}\int |f_{n}|^{2}\,d\nu^{i}=\sup_{n}\int |g^{i}(\theta^{i}_{n},\cdot,a_{n})|^{2} q^{i}(\cdot\mid a_{n})\,d\nu^{i}<\infty\), so \(\{f_{n}\}\) is uniformly integrable.
Vitali’s theorem yields \(K^{i}(\theta^{i}_{n},a_{n})=\int f_{n}\,d\nu^{i}\to \int f\,d\nu^{i}=K^{i}(\theta^{i},a)\).
Finiteness and a uniform bound follow from Cauchy–Schwarz and the \(L^{2}\) term in (S4).

\paragraph{Step 3 (Continuity of \(\mathcal K^{i}\)).}
By Step~2, \(K^{i}\) is bounded and continuous on the compact \(\Theta^{i}\times\mathbb A\) (S1).
If \((\theta^{i}_{n},\sigma_{n})\to(\theta^{i},\sigma)\) (weak topology on \(\Delta(\mathbb A)\)), then
\(\mathcal K^{i}(\theta^{i}_{n},\sigma_{n})=\int K^{i}(\theta^{i}_{n},a)\,\sigma_{n}(da)\to \int K^{i}(\theta^{i},a)\,\sigma(da)=\mathcal K^{i}(\theta^{i},\sigma)\),
since weak convergence preserves integration of bounded continuous functions.

\paragraph{Step 4 (Nonemptiness and compactness of \(\Theta^{m,i}(\sigma)\)).}
Fix \(\sigma\).
By Step~3, \(\theta^{i}\mapsto \mathcal K^{i}(\theta^{i},\sigma)\) is continuous; by (S1), \(\Theta^{i}\) is compact.
Hence the minimum is attained (Weierstrass), so \(\Theta^{m,i}(\sigma)\) is nonempty and compact.

\paragraph{Step 5 (Upper hemicontinuity).}
Berge’s Maximum Theorem applies: the feasible correspondence is the constant compact set \(\Theta^{i}\) (S1), and the objective \(\mathcal K^{i}\) is continuous in \((\theta^{i},\sigma)\) (Step~3).
Therefore, \(\Theta^{m,i}:\Delta(\mathbb A)\rightrightarrows \Theta^{i}\) is upper hemicontinuous and compact-valued.
\end{proof}


\subsection{$\pi$}


NEW: \paragraph{Step 1 (Uniform integrability for payoff integrands via de la Vallée–Poussin).}
Let $\delta>0$ be as in (S4$'$), and define the Young function
\[
\Phi(t):=
\begin{cases}
t, & 0\le t\le 1,\\[1mm]
t^{\,1+\delta}, & t>1.
\end{cases}
\]
By LR, $q^i_{\theta^i}\le M^i q^i$ a.e., hence for all $(a^i,a^{-i},\theta^i)$ and a.e.\ $y$,
\[
|\pi^i(a^i,y)|\,q^i_{\theta^i}(y\mid a^i,a^{-i})
\ \le\ (1+|\pi^i(a^i,y)|)^{1+\delta} M^i(y)\,q^i(y\mid a^i,a^{-i}).
\]
Split $\mathbb Y^i$ into $\{|\pi^i(a^i,y)|\le 1\}\cup\{|\pi^i(a^i,y)|>1\}$:

\smallskip
\emph{Small payoff region $\{|\pi|\le 1\}$.} Using $q^i_{\theta^i}\le M^i q^i$ and $\Phi(t)\le t$ for $t\le 1$,
\[
\Phi\!\big(|\pi^i|\,q^i_{\theta^i}\big)\ \le\ |\pi^i|\,q^i_{\theta^i}\ \le\ M^i q^i .
\]

\emph{Large payoff region $\{|\pi|>1\}$.} Since $\Phi(t)=t^{1+\delta}$ for $t>1$ and $|\pi|\le (1+|\pi|)^{1+\delta}$,
\[
\Phi\!\big(|\pi^i|\,q^i_{\theta^i}\big)
=\big(|\pi^i|\,q^i_{\theta^i}\big)^{1+\delta}
\ \le\ \big((1+|\pi^i|)^{1+\delta} M^i q^i\big)^{1}
\cdot \big(|\pi^i|\,q^i_{\theta^i}\big)^{\delta}
\ \le\ C_{\delta}\,(1+|\pi^i|)^{1+\delta} M^i q^i,
\]
where the last inequality uses $q^i_{\theta^i}\le M^i q^i$ and absorbs the extra $(|\pi^i|\,q^i_{\theta^i})^{\delta}$ into a constant multiple of $(1+|\pi^i|)^{1+\delta}M^i q^i$ (since $(1+|\pi|)^{1+\delta}\ge 1$ and $M^i\ge 1$ a.e.).

\smallskip
Combining both regions and integrating,
\[
\sup_{(a^i,a^{-i},\theta^i)}
\int_{\mathbb Y^i} \Phi\!\big(|\pi^i(a^i,y)|\,q^i_{\theta^i}(y\mid a^i,a^{-i})\big)\, \nu^i(dy)
\ \le\
C\left[
\sup_{a}\int_{\mathbb Y^i} M^i(y)\,q^i(y\mid a)\,d\nu^i(y)
+\sup_{a}\int_{\mathbb Y^i} (1+|\pi^i(a^i,y)|)^{1+\delta} M^i(y)\,q^i(y\mid a)\,d\nu^i(y)
\right]
<\infty,
\]
by (S4$'$). By de la Vallée–Poussin’s criterion, the family
\[
\Big\{\,|\pi^i(\cdot,a^i)|\,q^i_{\theta^i}(\cdot\mid a^i,a^{-i})\ :\ (a^i,a^{-i},\theta^i)\in \mathbb A^i\times\mathbb A^{-i}\times\Theta^i\,\Big\}
\]
is uniformly integrable in $L^1(\nu^i)$. In particular,
\(\bar U^i(a^i,\theta^i,a^{-i})=\int \pi^i(a^i,y)\,q^i_{\theta^i}(y\mid a^i,a^{-i})\,\nu^i(dy)\)
is well-defined and the collection $\{\bar U^i(a^i,\theta^i,a^{-i})\}$ is uniformly bounded over parameters.




\begin{lemma}
For each \(i\in I\), the best–response correspondence \(F^i(\mu^i,\sigma^{-i})\subseteq \mathbb A^i\) is nonempty, compact-valued, and upper hemicontinuous in \((\mu^i,\sigma^{-i})\).
\end{lemma}

\begin{proof}
Let
\[
\bar U^i(a^i,\theta^i,a^{-i})
:=\int_{\mathbb Y^i}\pi^i(a^i,y^i)\,q^i_{\theta^i}(y^i\mid a^i,a^{-i})\,\nu^i(dy^i),
\qquad
U^i(a^i,\mu^i,\sigma^{-i})
:=\iint \bar U^i(a^i,\theta^i,a^{-i})\,\mu^i(d\theta^i)\,\sigma^{-i}(da^{-i}).
\]
The best–response correspondence is \(F^i(\mu^i,\sigma^{-i})\in\arg\max_{a^i\in\mathbb A^i}U^i(a^i,\mu^i,\sigma^{-i})\).


\paragraph{Step 1 (Uniform $L^1$ envelope for payoff integrands; fix the $\delta$ from (S4$'$)).}
Let $\delta>0$ be as in (S4$'$). By LR, $q^i_{\theta^i}\le M^i\,q^i$ a.e., hence for all $(a^i,a^{-i},\theta^i)$ and $\nu^i$-a.e.\ $y$,
\[
|\pi^i(a^i,y)|\,q^i_{\theta^i}(y\mid a^i,a^{-i})
\;\le\;
|\pi^i(a^i,y)|\,M^i(y)\,q^i(y\mid a^i,a^{-i})
\;\le\;
(1+|\pi^i(a^i,y)|)^{1+\delta}\,M^i(y)\,q^i(y\mid a^i,a^{-i}),
\]
since $|\pi|\le (1+|\pi|)^{1+\delta}$ for every $\delta>0$. Integrating and taking the supremum,
\[
\sup_{(a^i,a^{-i},\theta^i)}
\int_{\mathbb Y^i} |\pi^i(a^i,y)|\,q^i_{\theta^i}(y\mid a^i,a^{-i})\,\nu^i(dy)
\;\le\;
\sup_{a\in\mathbb A}
\int_{\mathbb Y^i} (1+|\pi^i(a^i,y)|)^{1+\delta} M^i(y)\,q^i(y\mid a)\,\nu^i(dy)
\;<\;\infty,
\]
by (S4$'$) with this fixed $\delta$. Thus the family
$\{\,|\pi^i(\cdot,a^i)|\,q^i_{\theta^i}(\cdot\mid a^i,a^{-i})\,\}_{(a^i,a^{-i},\theta^i)}$
admits a parameter–uniform $L^1(\nu^i)$ envelope, hence is uniformly integrable (e.g., by de la Vallée–Poussin with $\Phi(t)=t^{1+\delta}$).
In particular, $\bar U^i(a^i,\theta^i,a^{-i})=\int \pi^i(a^i,y)\,q^i_{\theta^i}(y\mid a^i,a^{-i})\,\nu^i(dy)$
is well-defined and uniformly bounded over $(a^i,\theta^i,a^{-i})$.



\paragraph{Step 2 (Joint continuity of \(\bar U^i\)).}
Let \((a^i_n,\theta^i_n,a^{-i}_n)\to(a^i,\theta^i,a^{-i})\).
By a.e.-continuity (S2), for \(\nu^i\)-a.e.\ \(y\),
\[
\pi^i(a^i_n,y)\to \pi^i(a^i,y),
\qquad
q^i_{\theta^i_n}(y\mid a^i_n,a^{-i}_n)\to q^i_{\theta^i}(y\mid a^i,a^{-i}).
\]
Hence the integrands \(\pi^i(a^i_n,y)\,q^i_{\theta^i_n}(y\mid a^i_n,a^{-i}_n)\) converge a.e. to
\(\pi^i(a^i,y)\,q^i_{\theta^i}(y\mid a^i,a^{-i})\).
By Step~1 the family is uniformly integrable; thus Vitali’s theorem yields
\(\bar U^i(a^i_n,\theta^i_n,a^{-i}_n)\to \bar U^i(a^i,\theta^i,a^{-i})\).
Therefore \(\bar U^i\) is jointly continuous and (by Step~1) uniformly bounded.

\paragraph{Step 3 (Continuity of \(U^i\)).}
Equip \(\Delta(\Theta^i)\) and \(\Delta(\mathbb A^{-i})\) with the weak topologies.
Because \(\bar U^i\) is bounded and continuous on the compact
\(\mathbb A^i\times\Theta^i\times\mathbb A^{-i}\) (S1), the map
\[
(a^i,\mu^i,\sigma^{-i})\ \longmapsto\ U^i(a^i,\mu^i,\sigma^{-i})
=\iint \bar U^i(a^i,\theta^i,a^{-i})\,\mu^i(d\theta^i)\,\sigma^{-i}(da^{-i})
\]
is continuous (integration against weakly convergent measures preserves limits for bounded continuous integrands).

\paragraph{Step 4 (Nonemptiness, compactness, and upper hemicontinuity).}
By (S1), \(\mathbb A^i\) is compact and nonempty. For fixed \((\mu^i,\sigma^{-i})\), the function \(a^i\mapsto U^i(a^i,\mu^i,\sigma^{-i})\) is continuous (Step~3); hence by Weierstrass, the argmax is nonempty and compact.
Moreover, by Berge’s Maximum Theorem (feasible set constant compact \(\mathbb A^i\); objective continuous in \((a^i,\mu^i,\sigma^{-i})\) by Step~3), the correspondence
\(F^i(\mu^i,\sigma^{-i})\) is upper hemicontinuous in \((\mu^i,\sigma^{-i})\).
\end{proof}


\subsection{Claim 1}

\begin{claim}
For any fixed $\theta^{i}\in\Theta^{i}$ and any $\varepsilon>0$,
\[
\sup_{a\in\mathbb A}\ \int_{\mathbb Y^{i}}
\Big|\sup_{\theta'\in O(\theta^{i},\varepsilon)} g(\theta',y,a)\Big|^{2}\,q^{i}(y\mid a)\,\nu^{i}(dy)\ <\ \infty .
\]
\end{claim}

\begin{proof}
By the LR condition (S3),
\[
q^{i}_{\theta'}(\cdot\mid a)\,M^{i}(\cdot)^{-1}\ \le\ q^{i}(\cdot\mid a)\ \le\ q^{i}_{\theta'}(\cdot\mid a)\,M^{i}(\cdot)
\quad\text{a.e.-}\nu^{i}\qquad(\forall\,\theta',a).
\]
Hence, for $\nu^{i}$-a.e.\ $y$ and all $(\theta',a)$,
\[
\big|g(\theta',y,a)\big|
=\left|\log\frac{q^{i}(y\mid a)}{q^{i}_{\theta'}(y\mid a)}\right|
\le \big|\log M^{i}(y)\big|.
\]
Taking the supremum over $\theta'\in O(\theta^{i},\varepsilon)$ preserves this bound:
\[
\Big|\sup_{\theta'\in O(\theta^{i},\varepsilon)} g(\theta',y,a)\Big|
\ \le\ \big|\log M^{i}(y)\big|.
\]
Therefore,
\[
\sup_{a}\int \Big|\sup_{\theta'} g(\theta',y,a)\Big|^{2}\,q^{i}(y\mid a)\,d\nu^{i}
\ \le\ \sup_{a}\int \big|\log M^{i}(y)\big|^{2}\,q^{i}(y\mid a)\,d\nu^{i}.
\]
Finally, by the elementary bound $\big|\log M^{i}\big|^{2}\le C\,(1+M^{i})$ (e.g.\ take $C=1$ using
$|\log t|^{2}\le t$ for all $t\ge 1$), we obtain
\[
\sup_{a}\int \big|\log M^{i}\big|^{2}\,q^{i}(\cdot\mid a)\,d\nu^{i}
\ \le\ C\,\sup_{a}\int \big(1+M^{i}\big)\,q^{i}(\cdot\mid a)\,d\nu^{i}
\ \le\ C\,(1+\tilde C)\ <\ \infty,
\]
because $\int q^{i}(\cdot\mid a)\,d\nu^{i}=1$ and
$\sup_{a}\int M^{i}\,q^{i}(\cdot\mid a)\,d\nu^{i}<\infty$ by (S4$'$).
This proves the claim.
\end{proof}




\subsection{Claim 2}

\paragraph{Step 2 (Uniform oscillation in $a$; explicit modulus and details).}
Fix $\theta^{i}\in\Theta^{i}$ and define, for $a\in\mathbb A$ and $\rho>0$,
\[
f_{(a,\rho)}(y)
:=\sup_{\theta'\in B(\theta^{i},\rho)}
\bigl|\,g(\theta',y,a)-g(\theta^{i},y,a)\,\bigr|\;\, q^{i}(y\mid a)\ \ \ge 0.
\]
We show that
\[
\sup_{a\in\mathbb A}\ \int_{\mathbb Y^{i}} f_{(a,\rho)}(y)\,\nu^{i}(dy)
\;\xrightarrow[\rho\downarrow0]{}\;0.
\]

\emph{(a) a.e.\ pointwise convergence for each fixed $a$.}
By a.e.-continuity (S2), for $\nu^{i}$-a.e.\ $y$ the map $(\theta,a)\mapsto q^{i}_{\theta}(y\mid a)$ is continuous, and LR (S3) implies
$q^{i}(y\mid a)=0\iff q^{i}_{\theta}(y\mid a)=0$ and $|g(\theta,y,a)|\le |\log M^{i}(y)|$.
If $q^{i}_{\theta^{i}}(y\mid a)>0$, continuity of $(\theta,a)\mapsto g(\theta,y,a)$ at $(\theta^{i},a)$ yields
$\sup_{\theta'\in B(\theta^{i},\rho)}|g(\theta',y,a)-g(\theta^{i},y,a)|\downarrow 0$ as $\rho\downarrow 0$.
If $q^{i}_{\theta^{i}}(y\mid a)=q^{i}(y\mid a)=0$, then the factor $q^{i}(y\mid a)$ in $f_{(a,\rho)}(y)$ kills the term, and the LR bound ensures the log–ratio is finite.
Hence, for each fixed $a$,
\[
f_{(a,\rho)}(y)\ \downarrow\ 0\quad\text{for $\nu^{i}$-a.e.\ }y\ \ \text{as }\rho\downarrow 0.
\]

\emph{(b) A uniform integrability modulus (independent of $(a,\rho)$).}
From LR (S3), for all $(a,\rho)$ and $\nu^{i}$-a.e.\ $y$,
\[
0\le f_{(a,\rho)}(y)\ \le\ 2\,|\log M^{i}(y)|\,q^{i}(y\mid a).
\]
Let $\delta>0$ be the one from (S4$'$). Using the elementary bound
$(|\log M^{i}(y)|)^{1+\delta}\le C_{\delta}\,(1+M^{i}(y))$ and Hölder/Markov,
\[
\begin{aligned}
\sup_{a,\rho}\ \int \bigl(f_{(a,\rho)}\bigr)^{1+\delta}\,d\nu^{i}
&\le (2^{1+\delta} C_{\delta})\,
\sup_{a}\ \int \bigl(1+M^{i}(y)\bigr)\, \bigl(q^{i}(y\mid a)\bigr)^{1+\delta}\,d\nu^{i}
\\[-1mm]
&<\infty
\qquad\text{by (S4$'$).}
\end{aligned}
\]
Therefore the family $\mathcal F:=\{f_{(a,\rho)}:(a,\rho)\in\mathbb A\times(0,\infty)\}$ is uniformly integrable with the **explicit tail modulus**
\[
\boxed{\ \ \Phi(K)\ :=\ \sup_{(a,\rho)}\ \int f_{(a,\rho)}\,\mathbf 1_{\{f_{(a,\rho)}>K\}}\,d\nu^{i}
\ \le\ K^{-\delta}\ \sup_{(a,\rho)}\ \int \bigl(f_{(a,\rho)}\bigr)^{1+\delta}\,d\nu^{i}
\ \le\ C\,K^{-\delta}\ ,\ }
\]
which satisfies $\Phi(K)\downarrow 0$ as $K\to\infty$, and is independent of $(a,\rho)$.

\emph{(c) Vitali and the uniform limit of integrals.}
Fix $a$. By (a) and uniform integrability (b), Vitali’s theorem gives
\[
J(a,\rho)\ :=\ \int f_{(a,\rho)}\,d\nu^{i}\ \xrightarrow[\rho\downarrow0]{}\ 0.
\]
To make this **uniform in $a$**, use the elementary limsup–sup inequality:
\[
\limsup_{\rho\downarrow0}\ \sup_{a\in\mathbb A} J(a,\rho)
\ \le\ \sup_{a\in\mathbb A}\ \limsup_{\rho\downarrow0} J(a,\rho)
\ =\ \sup_{a\in\mathbb A} 0
\ =\ 0.
\]
Hence $\sup_{a}\int f_{(a,\rho)}\,d\nu^{i}\to 0$ as $\rho\downarrow0$.

\smallskip
For completeness, here is an $\varepsilon$–$\eta$ decomposition using the explicit modulus.
Given $\varepsilon>0$, choose $K$ so large that $\Phi(K)\le \varepsilon/2$.
Then for all $(a,\rho)$,
\[
\int f_{(a,\rho)}\,d\nu^{i}
\ =\ \int f_{(a,\rho)}\mathbf 1_{\{f_{(a,\rho)}\le K\}}\,d\nu^{i}
\ +\ \int f_{(a,\rho)}\mathbf 1_{\{f_{(a,\rho)}> K\}}\,d\nu^{i}
\ \le\ \int f_{(a,\rho)}\mathbf 1_{\{f_{(a,\rho)}\le K\}}\,d\nu^{i}\ +\ \varepsilon/2.
\]
For the bounded part, $0\le f_{(a,\rho)}\mathbf 1_{\{f_{(a,\rho)}\le K\}}\le K$ and, by (a), it converges a.e.\ to $0$ as $\rho\downarrow0$ for each fixed $a$.
Dominated convergence yields, for each $a$, a $\rho_{a}$ with
$\int f_{(a,\rho)}\mathbf 1_{\{f_{(a,\rho)}\le K\}}\,d\nu^{i}\le \varepsilon/2$ for all $\rho<\rho_{a}$.
Taking limsup in $\rho$ and then supremum in $a$ gives
\[
\limsup_{\rho\downarrow0}\ \sup_{a}\int f_{(a,\rho)}\,d\nu^{i}\ \le\ \varepsilon,
\]
and since $\varepsilon>0$ was arbitrary, the uniform convergence follows.




@@@@@@@@@@@@ VITALI APPROACH @@@@@@@@@@@


\paragraph{Setup.}
Fix a reference measure $\nu$ on $\mathbb Y$. For each $x\in X$ and $\theta\in\Theta$ let
\[
q(y\mid x)=\frac{dQ(\cdot\mid x)}{d\nu}(y),\qquad
q_\theta(y\mid x)=\frac{dQ_\theta(\cdot\mid x)}{d\nu}(y),
\]
and define
\[
g(\theta,y,x):=\log\!\frac{q(y\mid x)}{q_\theta(y\mid x)},\qquad
K(\theta,x):=\int g(\theta,y,x)\,q(y\mid x)\,d\nu(y),
\]
with the boundary convention $0\log(0/p)=0$.

\begin{assumption}[B1: a.e.\ continuity of the densities]
For $\nu$-a.e.\ $y\in\mathbb Y$,
\[
x\mapsto q(y\mid x)\ \text{ is continuous on }X,
\qquad
(\theta,x)\mapsto q_\theta(y\mid x)\ \text{ is continuous on }\Theta\times X.
\]
\end{assumption}

\begin{assumption}[LR: two-sided domination by a measurable $M$]
There exists a measurable $M:\mathbb Y\to[1,\infty)$ such that, for all $(\theta,x)\in\Theta\times X$,
\[
q_\theta(y\mid x)\,M(y)^{-1}\ \le\ q(y\mid x)\ \le\ q_\theta(y\mid x)\,M(y)
\qquad\text{for $\nu$-a.e.\ }y\in\mathbb Y.
\]
In particular, $\bigl|\log\tfrac{q(y\mid x)}{q_\theta(y\mid x)}\bigr|\le |\log M(y)|$ and $q(y\mid x)>0$ iff $q_\theta(y\mid x)>0$ $\nu$-a.e.
\end{assumption}

\begin{assumption}[B2: uniform $L^2$ bound]
\[
\sup_{x,\theta}\ \int g(\theta,y,x)^{2}\,q(y\mid x)\,d\nu(y)\ <\ \infty.
\]
\end{assumption}

\begin{claim}[Joint continuity of $K$ (Vitali)]
If $(\theta_n,x_n)\to(\theta,x)$ in $\Theta\times X$, then $K(\theta_n,x_n)\to K(\theta,x)$.
\end{claim}

\begin{proof}
For $\nu$-a.e.\ $y$, Assumption~B1 yields
$q(y\mid x_n)\to q(y\mid x)$ and $q_{\theta_n}(y\mid x_n)\to q_\theta(y\mid x)$.
Set $f_n(y):=q(y\mid x_n)\,g(\theta_n,y,x_n)$ and $f(y):=q(y\mid x)\,g(\theta,y,x)$.

If $q_\theta(y\mid x)>0$, continuity of $(u,v)\mapsto u\log(u/v)$ on $\{u\ge0,\ v>0\}$ gives $f_n(y)\to f(y)$.
If $q(y\mid x)=q_\theta(y\mid x)=0$, then by \textsc{LR}, $|g(\theta_n,y,x_n)|\le |\log M(y)|$ while $q(y\mid x_n)\to0$, hence $f_n(y)\to 0=f(y)$.
Thus $f_n\to f$ $\nu$-a.e.

Assumption~B2 implies $\sup_n\int |f_n|^2\,d\nu <\infty$, so $\{f_n\}$ is uniformly integrable.
By Vitali's theorem, $\int f_n\,d\nu\to \int f\,d\nu$, i.e.\ $K(\theta_n,x_n)\to K(\theta,x)$.
\end{proof}

\begin{claim}[Lemma 2, Step 1: square integrability, uniformly in $x$]
\[
\sup_{x,\theta}\ \int g(\theta,y,x)^2\,Q(dy\mid x)\ <\ \infty .
\]
\end{claim}

\begin{proof}
Since $Q(dy\mid x)=q(y\mid x)\,d\nu(y)$, this is exactly Assumption~B2.
\end{proof}

\begin{claim}[Lemma 2, Step 2 / eq.\ (12): uniform in $x$]
Fix $\theta\in\Theta$. For every $\varepsilon>0$ there exists $\delta>0$ such that
\[
\sup_{x\in X}\ 
\mathbb E_{Q(\cdot\mid x)}\!\left[
\sup_{\theta'\in B(\theta,\delta)}
\bigl|g(\theta',Y,x)-g(\theta,Y,x)\bigr|
\right]\ <\ \varepsilon .
\]
\end{claim}

\begin{proof}
For $\delta>0$ define
\[
\Delta_\delta(y)\ :=\ \sup_{x\in X}\ \sup_{\theta'\in B(\theta,\delta)}
\bigl|g(\theta',y,x)-g(\theta,y,x)\bigr|.
\]
By Assumption~B1 and the ratio control in \textsc{LR}, $\Delta_\delta(y)\downarrow 0$ for $\nu$-a.e.\ $y$ as $\delta\downarrow0$:
continuity handles points with $q_\theta>0$, while \textsc{LR} bounds $|\log(q/q_\theta)|$ near joint zeros so the oscillation also vanishes there.

Let $S(y):=\sup_{x,\vartheta}|g(\vartheta,y,x)|$; by \textsc{LR}, $S(y)\le |\log M(y)|<\infty$ a.e., hence $0\le \Delta_\delta\le 2S$.
Then, by Assumption~B2,
\[
\sup_{x}\int (2S(y))^{2}\,q(y\mid x)\,d\nu(y)
\ \le\ 4\,\sup_{x,\vartheta}\int g(\vartheta,y,x)^{2}\,q(y\mid x)\,d\nu(y)\ <\ \infty,
\]
so $\{\Delta_\delta(\cdot)\,q(\cdot\mid x): x\in X\}$ is uniformly integrable for each $\delta$.
Since $\Delta_\delta\to 0$ a.e., Vitali's theorem yields
\[
\sup_{x\in X}\ \int \Delta_\delta(y)\,q(y\mid x)\,d\nu(y)\ \xrightarrow[\delta\downarrow 0]{}\ 0,
\]
which is the desired uniform version of (12).
\end{proof}

\paragraph{Remarks.}
(i) The function $M(y)$ may grow with $|y|$ (e.g., polynomial--exponential) and is used only to bound likelihood ratios and to control the oscillation at joint zeros.
(ii) If you prefer a dominated-convergence proof, strengthen \textsc{LR} with an envelope such as $(\max\{1,|\log M|\})^{2} q(\cdot\mid x)\le h\in L^{1}(\nu)$ (independent of $x$); then $|g|\,q\le h$ provides a pointwise $L^1$ dominator.




\begin{proposition}[Finiteness of $K$ and mutual absolute continuity]
Under \textnormal{B1}, \textnormal{LR}, and \textnormal{B2}, for every $(\theta,x)\in\Theta\times X$:
\begin{enumerate}
\item $K(\theta,x)$ is finite.
\item $Q(\cdot\mid x)\sim Q_\theta(\cdot\mid x)$ (mutual absolute continuity).
\end{enumerate}
\end{proposition}

\begin{proof}
(1) Write $g:=\log(q/q_\theta)$. By \textnormal{B2},
\[
\int g(\theta,y,x)^2\,q(y\mid x)\,d\nu(y)\ <\ \infty.
\]
Since $Q(\cdot\mid x)$ is a probability measure,
\[
|K(\theta,x)|
=\left|\int g\,q\,d\nu\right|
\le \Big(\int g^2\,q\,d\nu\Big)^{1/2}\Big(\int q\,d\nu\Big)^{1/2}
=\Big(\int g^2\,q\,d\nu\Big)^{1/2}<\infty,
\]
by Cauchy--Schwarz. Moreover, \textnormal{LR} ensures $|g|\le|\log M|$ $\nu$-a.e., so the integrand is finite a.e.

\smallskip
(2) From \textnormal{LR}, for $\nu$-a.e.\ $y$,
\[
q_\theta(y\mid x)=0 \ \Rightarrow\ q(y\mid x)=0,
\qquad
q(y\mid x)=0 \ \Rightarrow\ q_\theta(y\mid x)=0.
\]
Thus $q(\cdot\mid x)=0$ iff $q_\theta(\cdot\mid x)=0$ $\nu$-a.e., i.e.\ $Q(\cdot\mid x)$ and $Q_\theta(\cdot\mid x)$ have identical null sets; hence $Q(\cdot\mid x)\sim Q_\theta(\cdot\mid x)$.
\end{proof}




@@@@@@@@@@@@ END VITALI APPROACH @@@@@@@@@@@


\end{comment}

\subsection{OLD Relation to \citet{heidhues2018unrealistic}.}
This example is a special case of the returns-to-effort environment in \citet{heidhues2018unrealistic}, but it is used here to illustrate a different object. In the overconfidence case, HKS study a particular Bayesian learning process and show that, under their assumptions, behavior converges to the unique Berk--Nash equilibrium. In the notation of the present example, this corresponds to the case in which the overconfident justification map \(T\) selects a unique equilibrium action. Berk--Nash rationalizability recovers this point prediction: when \(T\) has a unique fixed point, the iterated rationalizable interval collapses to that point. Our learning foundation then shows that this point prediction is robust across the broader class of learning procedures considered here: convergence holds not only under myopic optimal behavior, but also when agents use selected samples and are only required to behave asymptotically optimally (forward looking behavior is a special case because the model is identified, see Section \ref{subsec:forward}).

An additional role of our solution concept appears when the overconfidence case admits multiple Berk--Nash equilibria. The HKS convergence result relies on uniqueness of the Berk--Nash equilibrium and therefore no longer yields a point prediction in this case. Berk--Nash rationalizability still provides a sharp set-valued prediction: since \(T\) is increasing, the rationalizable set is the interval between the smallest and largest Berk--Nash equilibrium actions. This interval preserves the economic content of self-defeating learning, because throughout the rationalizable range the agent infers a return to effort below the truth and therefore chooses inefficiently low effort relative to the correct-prior, no-learning benchmark. Our learning foundation gives the interval a further dynamic interpretation. If one takes the HKS learning process itself as the benchmark, every long-run limit action must lie in this interval, so the solution concept provides bounds even though point convergence is no longer available. The same bounds continue to hold for the broader class of learning procedures allowed here, including selected samples and asymptotically optimal behavior. Moreover, our converse result shows that this prediction is essentially tight: self-justified long-run ranges can be sustained by suitable admissible learning rules, so the rationalizable interval is not merely an outer bound on long-run behavior.


The underconfidence case illustrates a different use of the set-valued object. HKS identify the self-correcting logic of underconfidence, but they do not provide a parallel convergence theorem for this environment. In the present example, \(T\) is decreasing, so the Berk--Nash equilibrium is unique. The question is whether this unique equilibrium remains the robust prediction once one allows for different ways of learning from past data. Berk--Nash rationalizability answers this question through the interval map induced by \(T\). If \(T^2\) has a unique fixed point, then the rationalizable set collapses to the unique Berk--Nash equilibrium; by the learning foundation, actions converge almost surely to that equilibrium for the broad class of learning procedures covered by the theorem. If \(T^2\) has multiple fixed points, then the unique equilibrium is not the robust set-valued prediction. Berk--Nash rationalizability instead delivers the self-correcting interval \([a_{\min}^\infty,a_{\max}^\infty]\), whose endpoints form a two-cycle of the justification map. Thus, in the underconfidence case, the solution concept either strengthens the unique-equilibrium prediction into an almost-sure convergence result, or else explains why robustness requires a range rather than a point.

Thus Berk--Nash rationalizability is not merely a technique for analyzing one fully specified dynamic. For a given dynamic, it can be useful because it gives simple conditions under which convergence follows and, when convergence to a point is not guaranteed, provides bounds on the possible long-run range. But the solution concept also stands on its own. It is a set-valued analogue of Berk--Nash equilibrium: it describes which ranges of behavior are internally justified by the evidence generated within those ranges. The learning foundation explains why these self-justified sets are the relevant long-run objects for many learning procedures, not only for the particular dynamic studied in HKS.


\subsection{Returns to effort and misguided learning}

Following the returns-to-effort application in \cite{heidhues2018unrealistic}, we consider a simple single-agent environment in which the agent is misspecified about ability and learns about the return to effort. The agent chooses effort \(a\in\mathbb A=[0,\bar a]\), where \(\bar a\) is large enough that it never binds in the calculations below. Output is
\[
y=(\alpha^*+a)\theta^*+\varepsilon,\qquad \varepsilon\sim\mathcal N(0,1),
\]
where \(\alpha^*\geq0\) is true ability and \(\theta^*>0\) is the true return to effort. The agent's payoff is \(\pi(a,y)=y-c(a)\), where \(c\) is differentiable and strictly convex, \(c(0)=c'(0)=0\), and \(c'(a)\to\infty\). The agent is misspecified about ability. He believes that ability is \(\alpha>0\), which he holds fixed, and learns only the return parameter \(\theta\in[0,\overline\theta]\), where \(\overline\theta\) is large enough that it does not bind. His subjective model is
\[
y=(\alpha+a)\theta+\varepsilon,\qquad \varepsilon\sim\mathcal N(0,1).
\]
Overconfidence corresponds to \(\alpha>\alpha^*\), and underconfidence to \(\alpha<\alpha^*\).

The correct-prior, no-learning benchmark is the action the agent would choose if he held the correct belief \(\theta=\theta^*\) about the return to effort and did not update from feedback. In that case, the perceived expected payoff from effort \(a\) is \((\alpha+a)\theta^*-c(a)\). The false belief about ability affects the perceived level of output, but not the marginal perceived return to effort. Hence the benchmark action is the true optimal action \(a^{opt}=(c')^{-1}(\theta^*)\).

For an action distribution \(\sigma\in\Delta\mathbb A\), the KL-minimizing parameter value solves
\[
\theta^m(\sigma)\in\arg\min_{\theta\in[0,\overline\theta]}\frac12\int_{\mathbb A}\left((\alpha+a)\theta-(\alpha^*+a)\theta^*\right)^2\sigma(da).
\]
Because \(\alpha>0\), this quadratic objective is strictly convex in \(\theta\), so the minimizer is unique; we take \(\overline\theta\) large enough that the upper bound does not bind. For a degenerate selected sample at \(a\),
\[
\theta^m(\delta_a)=\theta^*+\theta^*\frac{\alpha^*-\alpha}{\alpha+a}=\theta^*\frac{\alpha^*+a}{\alpha+a}.
\]
More generally, \(\theta^m(\sigma)\) is a weighted average of the single-action minimizers \(\theta^m(\delta_a)\), with weights proportional to \((\alpha+a)^2\sigma(da)\).

Given a belief concentrated on \(\theta\), the agent chooses \(a\) to solve \(c'(a)=\theta\). Therefore, for any nonempty compact set \(A\subseteq\mathbb A\),
\[
\Gamma(A)=\left\{(c')^{-1}(\theta^m(\sigma)):\sigma\in\Delta A\right\}.
\]
Define
\[
T(a)=(c')^{-1}(\theta^m(\delta_a)).
\]
The Berk--Nash equilibrium actions are exactly the fixed points of \(T\). Indeed, if the long-run action is the singleton \(\{a\}\), then the evidence generated at \(a\) leads to the best-fitting return \(\theta^m(\delta_a)\), and optimality requires \(a=(c')^{-1}(\theta^m(\delta_a))=T(a)\).

The same map also determines \(\Gamma\) on intervals. If \(A=[L,H]\), then \(\theta^m(\sigma)\) ranges over the convex hull of the values \(\theta^m(\delta_a)\) for \(a\in A\). In particular, if \(T\) is increasing on \([L,H]\), then the lowest and highest justified actions are obtained from the endpoint samples \(\delta_L\) and \(\delta_H\), respectively, so
\[
\Gamma([L,H])=[T(L),T(H)].
\]
If \(T\) is decreasing on \([L,H]\), the order of the endpoints is reversed, so
\[
\Gamma([L,H])=[T(H),T(L)].
\]
Thus Berk--Nash equilibria are the fixed points of \(T\), while Berk--Nash rationalizability is characterized by iterating the induced interval map.

\emph{Overconfidence.} Suppose \(\alpha>\alpha^*\). Then \(\theta^m(\delta_a)<\theta^*\) for every \(a\), and \(\theta^m(\delta_a)\) is strictly increasing in \(a\), since
\[
\frac{d}{da}\theta^m(\delta_a)
=
\theta^*\frac{\alpha-\alpha^*}{(\alpha+a)^2}
>0.
\]
Since \((c')^{-1}\) is strictly increasing, \(T\) is also strictly increasing. Intuitively, because the agent overstates ability, he attributes disappointing output to a low return to effort. This bias is strongest when effort is low, since ability is then a larger share of the perceived productive input \(\alpha+a\); as effort rises, the ability mistake is diluted, so the inferred return moves closer to \(\theta^*\).

The left panel of Figure~\ref{fig:returns_effort} illustrates this case. The curve \(\theta^m(\delta_a)\) lies below the true return \(\theta^*\) and is increasing. Berk--Nash equilibrium actions are intersections of this curve with the marginal cost curve \(c'\). Since \(c'\) is strictly increasing and \(\theta^m(\delta_a)<\theta^*\), every fixed point of \(T\) lies below the correct-prior benchmark \(a^{opt}=(c')^{-1}(\theta^*)\). Thus every Berk--Nash equilibrium action involves inefficiently low effort.

Berk--Nash rationalizability extends this equilibrium prediction to sets. Starting from \(A^0=[0,\bar a]\), define \(A^{k+1}=\Gamma(A^k)\). Since \(T\) is increasing, if \(A^k=[a_{\min}^k,a_{\max}^k]\), then
\[
a_{\min}^{k+1}=T(a_{\min}^k),
\qquad
a_{\max}^{k+1}=T(a_{\max}^k).
\]
The lower endpoint increases, the upper endpoint decreases, and the limiting interval is \([a_{\min}^\infty,a_{\max}^\infty]\), where \(a_{\min}^\infty\) and \(a_{\max}^\infty\) are fixed points of \(T\). Equivalently, they are the smallest and largest Berk--Nash equilibrium actions. If \(T\) has a unique fixed point, Berk--Nash rationalizability collapses to that equilibrium. If \(T\) has multiple fixed points, as in the left panel of Figure~\ref{fig:returns_effort}, Berk--Nash rationalizability predicts the entire interval between the smallest and largest equilibrium actions.

This interval prediction captures a set-valued version of self-defeating learning. Overconfidence leads the agent to interpret output through an inflated estimate of ability, and hence to infer that the return to effort is low. Because the inferred return is lower when the selected sample contains lower effort levels, the inference and the behavior reinforce each other: low effort supports pessimistic beliefs about returns, and pessimistic beliefs about returns justify low effort. Relative to the correct-prior, no-learning benchmark, feedback worsens the agent's decision. Berk--Nash rationalizability shows that this mechanism does not depend on selecting a particular Berk--Nash equilibrium. It applies throughout the entire rationalizable range: every action in that range is justified by pessimistic beliefs about returns and involves inefficiently low effort.


\begin{figure}[htbp]
\hspace{-1cm}
  \centering
  \begin{subfigure}[b]{0.5\textwidth}
    \centering

\begin{tikzpicture}
\begin{axis}[
    width=8cm,
    height=5cm,
    xmin=0, xmax=3,
    ymin=0, ymax=1.5,
    samples=100,
    domain=0:3,
    axis lines=left,
    xtick=\empty,
    ytick={1},
    yticklabels={$\theta^*$},
    xlabel={$a$},
    xlabel style={anchor=north east, at={(1,0)}, xshift=5pt},
    ylabel style={at={(0,1)}, anchor=north, rotate=-90, xshift=-15pt, yshift=10pt}
]
\addplot[thick, red] {1 + (1)*(1 - 3)/(3 + x)};
\node[red] at (axis cs:2.35,0.5) {\scriptsize overconfident: $\theta^m(\delta_\cdot)$};
\node[black] at (axis cs:2,1.4) {\scriptsize mg cost: $c'(\cdot)$};

\addplot[only marks, mark=*, mark size=1.25pt, red] coordinates {
    (.27,.38)
    (.65,.45)
    (1.4,.54)
};
\addplot[only marks, mark=*, mark size=1.25pt, black] coordinates {
    (2.04,1)
};

\node at (axis cs:2,1.1) {\tiny $a^{opt}$};
\node at (axis cs:.23,.47) {\tiny $a_S$};
\node at (axis cs:.65,.4) {\tiny $a_M$};
\node at (axis cs:1.4,.62) {\tiny $a_L$};

\addplot[thick, black, domain=0:3, samples=300]
    {0.45 / (1 + exp(-25 * (x - 0.2))) + ln(1 + exp(5 * (x - 1.5))) / 5};

\addplot[dashed, black] coordinates {(0,1) (3,1)};

\end{axis}
\end{tikzpicture}
    
    \caption{Overconfident agent}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering

\begin{tikzpicture}
\begin{axis}[
    width=8cm,
    height=5cm,
    xmin=0, xmax=3,
    ymin=0, ymax=2.1,
    samples=100,
    domain=0:3,
    axis lines=left,
    xtick=\empty,
    ytick={1},
    yticklabels={$\theta^*$},
    xlabel={$a$},
    xlabel style={anchor=north east, at={(1,0)}, xshift=5pt},
    ylabel style={at={(0,1)}, anchor=north, rotate=-90, xshift=-15pt, yshift=10pt},
    xtick={0.22, 0.94},
    xticklabels={{\tiny\textcolor{blue}{$a^{\infty}_{\min}$}}, {\tiny\textcolor{blue}{$a^{\infty}_{\max}$}}},
]

\addplot[thick, blue] {1 + (1)*(1 - 0.5)/(0.5 + x)};
\node[blue] at (axis cs:2.2,1.35) {\scriptsize underconfident: $\theta^m(\delta_\cdot)$};

\addplot[thick, black, domain=0:3, samples=300]
  {1.5 * (1 - exp(-10*x)) + 0.5 * ln(1 + exp(10*(x - 1.0)))};
  
\node[black] at (axis cs:1.5,1.8) {\scriptsize mg cost: $c'(\cdot)$};  

\addplot[dashed, black] coordinates {(0,1) (3,1)};

\node at (axis cs:.2,.9) {\tiny $a^{opt}$};
\addplot[only marks, mark=*, mark size=1.25pt, black] coordinates {
    (.11,1)
};

\addplot[only marks, mark=*, mark size=1.25pt, black] coordinates {
    (0.511,1.495)
};

\node at (axis cs:0.511,1.608) {\tiny $a^*$};

\draw[dashed, darkgreen!70] (axis cs:.22,1.34) rectangle (axis cs:.94,1.7);
\draw[dashed, black!40] (axis cs:0.22,0) -- (axis cs:0.22,1.34);
\draw[dashed, black!40] (axis cs:0.94,0) -- (axis cs:0.94,1.34);

\end{axis}
\end{tikzpicture}
   
    \caption{Underconfident agent}
  \end{subfigure}
\caption{
\centering Returns to effort example.\\
\parbox{\linewidth}{\footnotesize
The optimal action \(a^{opt}\) is where the marginal cost curve \(c'\) intersects the true return \(\theta^*\). Berk--Nash equilibrium actions lie at intersections of \(c'\) and the KL-minimizing return curve \(\theta^m(\delta_\cdot)\). In the overconfident case, there may be multiple Berk--Nash equilibria, and Berk--Nash rationalizability gives the interval from the smallest to the largest equilibrium. In the underconfident case, the Berk--Nash equilibrium is unique, but Berk--Nash rationalizability may be a nontrivial interval whose endpoints form a two-cycle of the justification map \(T\).
}
}
  \label{fig:returns_effort}
\end{figure}



\emph{Underconfidence.} Suppose instead that \(\alpha<\alpha^*\). Then \(\theta^m(\delta_a)>\theta^*\) for every \(a\), and \(\theta^m(\delta_a)\) is strictly decreasing in \(a\). 
Since \((c')^{-1}\) is strictly increasing, \(T\) is strictly decreasing. Intuitively, because the agent understates ability, he attributes unexpectedly high output to a high return to effort. This bias is strongest when effort is low, since ability is then a larger share of the productive input; as effort rises, the ability mistake is diluted, so the inferred return moves closer to \(\theta^*\).

The right panel of Figure~\ref{fig:returns_effort} illustrates this case. The curve \(\theta^m(\delta_a)\) lies above the true return \(\theta^*\) and is decreasing. Berk--Nash equilibrium actions are intersections of this curve with the marginal cost curve \(c'\). Since \(T\) is strictly decreasing, there is at most one fixed point, and hence at most one Berk--Nash equilibrium action, denoted by $a^*$ in the figure. Moreover, since \(\theta^m(\delta_a)>\theta^*\), any such equilibrium lies above the correct-prior benchmark \(a^{opt}=(c')^{-1}(\theta^*)\). Thus the equilibrium prediction is over-effort: relative to the correct-prior, no-learning benchmark, the agent overestimates the return to effort and chooses effort that is too high.

The rationalizable prediction reflects the negative feedback in the justification map. Low sampled effort makes the ability mistake more important, leading the agent to infer a high return to effort; this high inferred return justifies high effort. But high sampled effort dilutes the ability mistake, leading the agent to infer a lower return and to justify lower effort. Thus underconfidence generates self-correcting rather than self-reinforcing mislearning.

Starting again from \(A^0=[0,\bar a]\), define \(A^{k+1}=\Gamma(A^k)\). Since \(T\) is decreasing, if \(A^k=[a_{\min}^k,a_{\max}^k]\), then
\[
a_{\min}^{k+1}=T(a_{\max}^k),
\qquad
a_{\max}^{k+1}=T(a_{\min}^k).
\]
The endpoints converge to limits \(a_{\min}^\infty\) and \(a_{\max}^\infty\) satisfying
\[
T(a_{\min}^\infty)=a_{\max}^\infty,
\qquad
T(a_{\max}^\infty)=a_{\min}^\infty.
\]
Thus the endpoints form a two-cycle of the justification map \(T\), or equivalently fixed points of \(T^2\).

The underconfidence case shows that a unique Berk--Nash equilibrium need not imply a singleton rationalizable prediction. Because \(T\) is continuous and decreasing, it has a unique fixed point, so there is a unique Berk--Nash equilibrium. But Berk--Nash rationalizability is governed by the interval map induced by \(T\), and hence by the fixed points of \(T^2\). If \(T^2\) has a unique fixed point, then \(a_{\min}^\infty=a_{\max}^\infty\), so Berk--Nash rationalizability collapses to the unique Berk--Nash equilibrium. If \(T^2\) has multiple fixed points, as in the right panel of Figure~\ref{fig:returns_effort}, then Berk--Nash rationalizability is the nontrivial interval \([a_{\min}^\infty,a_{\max}^\infty]\). The endpoints form a two-cycle of the justification map: low effort is justified by samples containing high effort, and high effort is justified by samples containing low effort.

\subsection{Strategic feedback and self-justification}

Consider two decision makers, indexed by $i=1,2$, whose actions interact through a feedback system. Two features of this setting will be central below. First, each player's action affects the payoff-relevant target faced by the other, so that actions generate strategic feedback across decision makers. Second, agents may interpret observed changes in these targets as information about an underlying environment without fully accounting for the extent to which the targets are themselves generated by past actions. Our misspecification below captures this idea in stark form: each player treats her observed target as a draw from an unknown stationary distribution rather than as the endogenous outcome of the feedback system. This reduced-form structure can arise in a variety of settings in which decision makers adjust to conditions that are partly created by one another's behavior, including supply-chain interactions, monetary and fiscal policy, organizational decision making, regulatory interactions, and firms adjusting prices, quantities, investment, or other strategic choices over time.\footnote{Supply-chain environments provide one particularly well-documented example of such feedback. \citet{lee1997information} emphasize the informational role of downstream orders for upstream production and inventory decisions, while \citet{sterman1989modeling} documents experimentally that decision makers in inventory systems systematically underappreciate endogenous feedback from their own decisions.}


Each player chooses an action $a^i\in[-1,1]$. The action is measured relative to a neutral benchmark, so that positive and negative values represent movements in opposite directions from that benchmark. Player $i$ observes a performance target $y^i$ and has payoff
\[
u^i(a^i,y^i)=-(a^i-y^i)^2.
\]
The true performance targets satisfy
\[
y^1=\gamma a^1-\omega a^2+\varepsilon^1,
\qquad
y^2=\omega a^1+\gamma a^2+\varepsilon^2,
\]
where $\varepsilon^1$ and $\varepsilon^2$ are independent standard normal random variables, $\gamma\geq 0$, and $\omega>0$. Thus $\gamma$ measures the strength of own-action feedback and $\omega$ the strength of cross-player feedback. The opposite signs of the two cross-effects generate a rotational component to the feedback: a change in one action induces a response in the other direction, which in turn feeds back to the first player.

Players neglect the dependence of performance targets on actions. Player $i$ believes instead that
\[
y^i=\theta^i+\varepsilon^i,
\]
where $\theta^i\in\Theta^i$ and $\Theta^i$ is a sufficiently large compact interval. Thus a player interprets changes in the observed target as information about an unknown underlying level $\theta^i$, rather than as the endogenous consequence of actions. Given a belief concentrated on $\theta^i$, player $i$ chooses
\[
a^i=\Pi(\theta^i),
\]
where $\Pi$ denotes projection onto $[-1,1]$.




For a fixed action profile $a$, the Gaussian KL divergence is uniquely minimized at
\[
\theta^{m,1}(a)=\gamma a^1-\omega a^2,
\qquad
\theta^{m,2}(a)=\omega a^1+\gamma a^2.
\]
Hence a Berk--Nash equilibrium satisfies
\[
a^1=\Pi(\gamma a^1-\omega a^2),
\qquad
a^2=\Pi(\omega a^1+\gamma a^2).
\]
We maintain throughout
\[
\gamma<1+\omega.
\]
Under this restriction, the unique Berk--Nash equilibrium is
\[
a^*=(0,0).
\]
Thus Berk--Nash equilibrium gives the same point prediction throughout the parameter region considered here.\footnote{Let
\[
B=
\begin{pmatrix}
\gamma & -\omega\\
\omega & \gamma
\end{pmatrix}.
\]
An equilibrium satisfies $a=\Pi(Ba)$. If $\gamma<1$, the projection inequality implies
\[
a'(Ba-a)\geq 0.
\]
But $a'Ba=\gamma\|a\|^2$, because the component of $B$ proportional to $\omega$ is skew-symmetric. Hence $(\gamma-1)\|a\|^2\geq0$, which is impossible for $a\neq0$. If $\gamma>1$, any nonzero fixed point must lie on the boundary. Using the $90^\circ$ rotational symmetry, suppose without loss that $a^1=1$. The first-coordinate condition implies $a^2\leq(\gamma-1)/\omega$. If the second coordinate is interior, its fixed-point condition gives $a^2=-\omega/(\gamma-1)$; if it is on the boundary, the corresponding projection inequalities also require $\omega\leq\gamma-1$. Thus $\omega>\gamma-1$, or equivalently $\gamma<1+\omega$, rules out every nonzero fixed point.}

The prediction is very different for Berk--Nash rationalizability. Let $S\subseteq[-1,1]^2$ be a nonempty compact set. Player $i$ may base her inference on a selected distribution $\sigma^i\in\Delta S$. Let
\[
\bar a^{\,i}=\int_S a\,\sigma^i(da)
\]
denote the mean action profile in player $i$'s selected sample, with components $\bar a^{\,i}_1$ and $\bar a^{\,i}_2$. The corresponding KL-minimizing parameters are
\[
\theta^{m,1}(\sigma^1)=\gamma \bar a^{\,1}_1-\omega \bar a^{\,1}_2,
\qquad
\theta^{m,2}(\sigma^2)=\omega \bar a^{\,2}_1+\gamma \bar a^{\,2}_2.
\]
Thus each player's fitted parameter depends on the mean action profile in her own selected sample. Because the two players may select different samples from $S$, the two coordinates of a candidate action profile can be justified using different distributions of observations generated within $S$.

The largest self-justified set has a particularly simple form:
\[
\mathcal{B}
=
\begin{cases}
\{(0,0)\}, & \gamma+\omega<1,\\[4pt]
[-1,1]^2, & \gamma+\omega\geq1.
\end{cases}
\]
To see the first claim, let $S$ be self-justified and define
\[
M=\max_{a\in S}\max_{i=1,2}|a^i|.
\]
Every mean action profile generated by a distribution supported on $S$ has coordinates bounded by $M$ in absolute value. Hence every parameter that can be fitted from such a sample has absolute value at most $(\gamma+\omega)M$, and every action that can be justified has absolute value at most $(\gamma+\omega)M$. Since some coordinate of some action in $S$ attains $M$, self-justification requires
\[
M\leq(\gamma+\omega)M.
\]
Thus, if $\gamma+\omega<1$, necessarily $M=0$.

Conversely, suppose $\gamma+\omega\geq1$ and take $S=[-1,1]^2$. As the mean of a selected sample ranges over $S$, the KL-minimizing parameter of either player ranges over
\[
[-(\gamma+\omega),\,\gamma+\omega].
\]
This interval contains $[-1,1]$. Hence, for every profile $a\in[-1,1]^2$, player 1 can select observations from $S$ that make $a^1$ optimal, while player 2 can select possibly different observations that make $a^2$ optimal. Therefore the entire action space is self-justified.

Notice that this characterization does not require iterating the operator $\Gamma$. When $\gamma+\omega<1$, the argument above applies to any self-justified set and shows directly that it must be the singleton $\{(0,0)\}$. When $\gamma+\omega\geq1$, the entire action space is itself self-justified and therefore must be the largest self-justified set.



The threshold $\gamma+\omega=1$ has a natural interpretation. When total feedback is weak, observations generated by a bounded range of actions cannot produce beliefs sufficiently extreme to reproduce that same range of actions. The only range that can justify itself is the singleton at zero. Once feedback is sufficiently strong, however, the data generated within the action space are rich enough that different samples can support every possible action. Notice that this conclusion is not reflected in Berk--Nash equilibrium: under our maintained assumption $\gamma<1+\omega$, the equilibrium remains uniquely $(0,0)$ on both sides of the threshold.

Next, we assess whether this conclusion survives the common-sample refinement. Under that refinement, both players must base their justification on the same distribution $\sigma\in\Delta S$. Let
\[
\bar a=\int_S a\,\sigma(da)
\]
denote the mean action profile in the common sample. The vector of KL-minimizing parameters is then
\[
\theta^m(\sigma)=B\bar a,
\qquad
B=
\begin{pmatrix}
\gamma & -\omega\\
\omega & \gamma
\end{pmatrix},
\]
and therefore
\[
\Gamma^{CS}(S)
=
\left\{
\Pi(B\bar a):
\bar a\in\operatorname{co}(S)
\right\}.
\]

The common-sample requirement can substantially sharpen the prediction. In particular, since $\|Bx\|=\sqrt{\gamma^2+\omega^2}\,\|x\|$, any common-sample self-justified set must collapse to $\{(0,0)\}$ whenever
\[
\gamma^2+\omega^2<1.
\]
Thus there are parameter values for which ordinary Berk--Nash rationalizability is the entire square, because $\gamma+\omega\geq1$, while common-sample Berk--Nash rationalizability is only the singleton $\mathcal{B}^{CS}=\{(0,0)\}$.\footnote{For example, if $\gamma=1/2$ and $\omega=3/4$, then $\gamma+\omega=5/4>1$, so the rationalizable set is $\mathcal{B}=[-1,1]^2$, whereas $\gamma^2+\omega^2=13/16<1$, so the common-sample rationalizable set is $\mathcal{B}^{CS}=\{(0,0)\}$.}

The refinement does not always have bite, however. If
\[
\gamma^2+\omega^2\geq\gamma+\omega,
\]
then the entire square is also common-sample self-justified, so
\[
\mathcal B^{CS}=[-1,1]^2.
\]
Indeed, for any profile $a\in[-1,1]^2$, one can choose a common sample whose mean is $\bar a=B^{-1}a$; the displayed inequality is exactly the condition ensuring that $B^{-1}$ maps the square into itself.\footnote{Since
\[
B^{-1}
=
\frac{1}{\gamma^2+\omega^2}
\begin{pmatrix}
\gamma & \omega\\
-\omega & \gamma
\end{pmatrix},
\]
we have $B^{-1}[-1,1]^2\subseteq[-1,1]^2$ iff
\[
\frac{\gamma+\omega}{\gamma^2+\omega^2}\leq1.
\]
For instance, $\gamma=1/2$ and $\omega=3/2$ satisfy this condition, so both the ordinary and common-sample rationalizable sets equal the entire action space.}


\paragraph{Comparison with a benchmark learning dynamic.}
The preceding analysis characterizes behavior that can be justified without specifying a particular learning procedure, and the common-sample refinement shows how this prediction can change when players are required to base their inferences on the same evidence. To put these set-valued predictions in perspective, we now compare them with one fully specified benchmark learning process. This comparison is not needed for the definition or characterization of Berk--Nash rationalizability; its purpose is simply to illustrate how the robustness captured by self-justification differs from the stability properties of a particular learning rule.

Suppose players use the entire history of their observations and have normal priors over $\theta^i$. In this case, standard stochastic-approximation arguments imply that if $\gamma<1$, play converges almost surely to the unique Berk--Nash equilibrium $(0,0)$. If $\gamma>1$, the equilibrium is unstable; moreover, in this Gaussian environment the probability that play converges to $(0,0)$ is zero.\footnote{With normal priors, the vector $m_t$ of posterior means obeys the exact recursion
\[
m_{t+1}
=
m_t+\alpha_{t+1}
\left[
B\Pi(m_t)-m_t+\varepsilon_{t+1}
\right],
\qquad
\alpha_t\sim t^{-1}.
\]
The associated ODE is
\[
\dot m=B\Pi(m)-m.
\]
For $\gamma<1$, let $\phi(x)=\int_0^x\Pi(s)\,ds$ and $V(m)=\phi(m^1)+\phi(m^2)$. Since $\nabla V(m)=\Pi(m)$ and the $\omega$ component of $B$ is skew-symmetric,
\[
\dot V(m)
\leq
-(1-\gamma)\|\Pi(m)\|^2,
\]
so zero is globally asymptotically stable. Standard stochastic approximation then yields almost-sure convergence. For $\gamma>1$, the local drift is $(B-I)m$, whose eigenvalues are $(\gamma-1)\pm i\omega$, so zero is a repeller. Instability of the limiting ODE alone does not generally imply that the stochastic process avoids the equilibrium. Here the stronger conclusion follows from the exact local linear recursion and the nondegenerate Gaussian innovations. See, for example, \citet{heidhues2021convergence} for the use of stochastic approximation in misspecified learning.}

When $\gamma+\omega<1$, all of the predictions considered above coincide. In this region $\gamma<1$, so the unique Berk--Nash equilibrium is $(0,0)$, the Berk--Nash rationalizable set is the singleton $\{(0,0)\}$, and full-history Bayesian learning converges almost surely to $(0,0)$. The common-sample refinement therefore does not alter the conclusion in this region.

More revealing is the region
\[
\gamma<1
\qquad\text{and}\qquad
\gamma+\omega\geq1.
\]
The unique Berk--Nash equilibrium remains $(0,0)$ and, under the full-history normal-prior learning process just described, play converges to it almost surely. Nevertheless, the rationalizable set is
\[
\mathcal{B}=[-1,1]^2.
\]
Thus the large rationalizable set cannot be attributed to instability of the equilibrium. Rather, the two approaches address different questions. Full-history Bayesian learning fixes a particular rule for how agents use past observations, whereas Berk--Nash rationalizability asks which behavior can be justified when the way in which experience is sampled is left unspecified. In this region, therefore, the equilibrium can be globally stable under a natural benchmark learning process while the baseline self-justification criterion allows the entire action space. As shown above, the common-sample refinement may sharpen this conclusion for some parameter values, but for others even the common-sample rationalizable set remains the whole square.

Finally, when
\[
1<\gamma<1+\omega,
\]
the unique Berk--Nash equilibrium is still $(0,0)$, but it is unstable under the full-history benchmark and the probability of convergence to it is zero. Since $\gamma+\omega>1$ in this region,
\[
\mathcal{B}=[-1,1]^2.
\]
Here the broad rationalizable prediction is consistent with the failure of the equilibrium to attract the benchmark learning dynamics. The preceding stable case is more informative for the purpose of the example, however, because it shows that a large self-justified set is not merely a consequence of dynamic instability. Rather, Berk--Nash rationalizability allows for substantial flexibility in how agents sample from their experience and requires only asymptotic optimality, while retaining the Bayesian and empirical-forecast structure underlying the learning foundation.


\subsection{A linear-quadratic network example}


We next show that the common-sample refinement can sharpen a familiar solution concept even when players know the game they are playing. We construct a simple three-player game in which correlated rationalizability allows a large set of action profiles, while imposing the common sample refinement reduces the prediction all the way to the unique Nash equilibrium.


We use a simple linear-quadratic network game. Linear-quadratic network games are a standard class of examples in economics, used to study peer effects, local public goods, crime, and network complementarities or substitutes; see, for example, \cite{ballester2006whos}, \cite{bramoulle2007public}, and \cite{bramoulle2014strategic}. The example is designed to isolate two forces behind the common-sample refinement. First, two players respond to the same third player's action, so requiring them to use a common empirical distribution restricts the actions they can jointly justify. Second, this restriction eliminates a source of disagreement that would otherwise sustain a large rationalizable set, leaving a dampened feedback loop that converges to the Nash equilibrium.


There are three players, \(i=1,2,3\). Each player chooses an action \(a^i\in[-1,1]\), and we write \(a=(a^1,a^2,a^3)\). Payoffs are
\[
u^1(a)=-\frac12(a^1-\lambda a^3)^2,
\]
\[
u^2(a)=-\frac12(a^2-\lambda a^3)^2,
\]
and
\[
u^3(a)=-\frac12\left(a^3+\mu\frac{a^1+a^2}{2}-\kappa\frac{a^1-a^2}{2}\right)^2.
\]
Assume \(0<\lambda\leq1\), \(\mu>0\), \(\lambda\mu<1\), and \(\kappa\lambda\geq1\). Players 1 and 2 choose actions that track the third player's action, with strength \(\lambda\). Player 3 responds both to the average action of players 1 and 2 and to the imbalance between them. The average term is stabilizing, while the imbalance term amplifies the flexibility allowed by rationalizability. Because players 1 and 2 may evaluate player 3 using different empirical distributions, they can justify different actions; the resulting imbalance between their actions, in turn, allows player 3 to justify a wide range of actions.


The model is correctly specified and identified, so we suppress \(\mu^i\) in this example and write best responses directly as functions of the empirical distribution used to evaluate payoffs. For \(\sigma\in\Delta\mathbb A\), let
\[
m_j(\sigma)=\int_{\mathbb A}a^j\,\sigma(da)
\]
denote the \(\sigma\)-mean of player \(j\)'s action. The best-response correspondences are single-valued:
\[
F^1(\sigma)=\{\lambda m_3(\sigma)\},
\qquad
F^2(\sigma)=\{\lambda m_3(\sigma)\},
\]
and \[ F^3(\sigma) = \left\{ \Pi\!\left( -\mu\frac{m_1(\sigma)+m_2(\sigma)}{2} +\kappa\frac{m_1(\sigma)-m_2(\sigma)}{2} \right) \right\}, \] where $\Pi$ denotes projection onto $[-1,1]$.

\paragraph{Nash equilibrium.}
At a Nash equilibrium,
\[
a^1=\lambda a^3,\qquad a^2=\lambda a^3,
\]
and
\[
a^3=
\Pi\!\left(
-\mu\frac{a^1+a^2}{2}
+\kappa\frac{a^1-a^2}{2}
\right).
\]

The first two equations imply \(a^1=a^2=\lambda a^3\). Hence the imbalance term in player 3's best response vanishes, and
\[
a^3=-\mu\lambda a^3.
\]
Since \(\lambda\mu>0\), this implies \(a^3=0\), and therefore \(a^1=a^2=0\). Thus the game has a unique Nash equilibrium,
\[
a^*=(0,0,0).
\]

\paragraph{Rationalizable profiles.}
Under the baseline operator \(\Gamma\), different players may use different distributions over the candidate set. Starting from \(\mathbb A=[-1,1]^3\), players 1 and 2 can justify precisely actions in \([-\lambda,\lambda]\), since their best responses are \(\lambda m_3(\sigma)\) and \(m_3(\sigma)\in[-1,1]\). Player 3 can justify every action in \([-1,1]\), because the imbalance term can vary over an interval containing \([-1,1]\) when \(\kappa\geq1\). Thus
\[
\Gamma(\mathbb A)=[-\lambda,\lambda]\times[-\lambda,\lambda]\times[-1,1].
\]
This set is fixed under \(\Gamma\). Indeed, if \(S=[-\lambda,\lambda]\times[-\lambda,\lambda]\times[-1,1]\), then players 1 and 2 again justify exactly \([-\lambda,\lambda]\), and player 3 can again justify every action in \([-1,1]\), because \(\kappa\lambda\geq1\). Therefore
\[
\mathcal B=[-\lambda,\lambda]\times[-\lambda,\lambda]\times[-1,1].
\]
Rationalizability is permissive because players 1 and 2 may justify different actions using different empirical distributions over player 3's behavior.\footnote{The argument does not rely on correlation: only opponents' marginal means matter, so the same set obtains under independent-beliefs rationalizability.}

\paragraph{Common-sample rationalizable profiles.}
Because the game is correctly known, the common-sample operator takes a particularly simple form. For any $S\subseteq\mathbb A$,
\[
\Gamma^{CS}(S)
=
\left\{
a\in\mathbb A:
\exists\,\sigma\in\Delta S
\text{ such that }
a^i\in BR^i(\sigma^{-i})
\text{ for every }i
\right\}.
\]
Thus, in contrast to classical rationalizability, all players must justify their actions using marginals of the same joint distribution $\sigma$.

Starting from $C^0=\mathbb A$, define
\[
C^{k+1}=\Gamma^{CS}(C^k).
\]
Consider the first round. If $a\in C^1$, then there is a single $\sigma\in\Delta C^0$ such that
\[
a^1=\lambda m_3(\sigma),
\qquad
a^2=\lambda m_3(\sigma).
\]
The same mean of player 3's action therefore determines both best responses, so
\[
a^1=a^2.
\]
Moreover, as $m_3(\sigma)$ ranges over $[-1,1]$, their common action ranges over $[-\lambda,\lambda]$. Player 3 can still justify any action in $[-1,1]$. Hence
\[
C^1
=
\{(q,q,r):q\in[-\lambda,\lambda],\ r\in[-1,1]\}.
\]


From the second round onward, every common sample is supported on profiles satisfying $a^1=a^2$. Hence, for any such sample,
\[
m_1(\sigma)=m_2(\sigma),
\]
so player 3's imbalance term vanishes. Writing profiles as $(q,q,r)$, a common-sample update therefore satisfies
\[
q=\lambda m_3(\sigma),
\qquad
r=-\mu m_1(\sigma).
\]

Consider two successive applications of $\Gamma^{CS}$. In the first, the new first coordinate is $\lambda$ times the previous mean third coordinate; in the second, the new third coordinate is $-\mu$ times the previous mean first coordinate. Thus, after two rounds, the ranges of both relevant coordinates are multiplied by $\lambda\mu$. Since
\[
\lambda\mu<1,
\]
repeated application of $\Gamma^{CS}$ contracts these ranges to zero. Therefore
\[
\bigcap_{k=0}^{\infty} C^k=\{(0,0,0)\},
\]
and hence
\[
\mathcal B^{CS}=\{(0,0,0)\}.
\]



Thus this example has
\[
NE=\mathcal B^{CS}=\{(0,0,0)\},
\]
whereas
\[
\mathcal B=[-\lambda,\lambda]\times[-\lambda,\lambda]\times[-1,1].
\]
The common-sample refinement has two effects. First, because players 1 and 2 must use the same empirical distribution over player 3's action, it imposes \(a^1=a^2\). Second, once \(a^1=a^2\) is imposed, player 3's imbalance term vanishes, and the remaining feedback loop has strength \(\lambda\mu\). When \(\lambda\mu<1\), this feedback is dampened, and the common-sample refinement selects the unique Nash equilibrium.


\subsection{Self-Synchronized Behavior}

We introduce a refinement that focuses on actions that persist together with the empirical distributions used to justify them. For a nonempty set $S\subseteq\mathbb A$, define
\[
\Gamma^{+}(S)
=
\left\{
a\in\mathbb A:
\begin{array}{l}
\text{for every }i\in I\text{ there exist }\sigma^i\in\Delta S
\text{ and }\mu^i\in\Delta\Theta^{m,i}(\sigma^i)\\
\text{such that }
a\in\operatorname{supp}(\sigma^i)
\text{ and }
a^i\in F^i(\mu^i,(\sigma^i)^{-i})
\end{array}
\right\}.
\]
The common-sample refinement $\Gamma^{CS+}$ is defined analogously by requiring a single $\sigma\in\Delta S$, with $a\in\operatorname{supp}(\sigma)$, to justify all players. We call $S$ \emph{$+$-self-justified} if $S\subseteq\Gamma^+(S)$, and \emph{common-sample $+$-self-justified} if $S\subseteq\Gamma^{CS+}(S)$.

Because $a\in\Gamma^+(S)$ requires $a\in\operatorname{supp}(\sigma^i)\subseteq S$, we have $\Gamma^+(S)\subseteq S$. Hence $+$-self-justified sets are exactly the fixed points of $\Gamma^+$. Since $\Gamma^+$ is monotone, the union of all fixed points is itself a fixed point, so a largest fixed point always exists. The same holds for $\Gamma^{CS+}$. Unlike the baseline operator $\Gamma$, however, these refined operators need not be nonempty-valued on nonempty sets, so their largest fixed points may be empty. When $\mathbb A$ is finite, the decreasing sequence of iterates stabilizes after finitely many steps and yields the usual iterative characterization.\footnote{In infinite action spaces, the iterative characterization need not hold because the condition $a\in\operatorname{supp}(\sigma)$ is not preserved under weak convergence.}

We next provide a learning foundation for these refinements. A nonempty set $S\subseteq\mathbb A$ is \emph{self-synchronized} along a realized path if, for every $a\in S$, there exists a subsequence $(t_k)_k$ and distributions $\sigma^i\in\Delta S$, $i\in I$, such that
\[
a_{t_k}\to a,
\qquad
\hat\sigma_{t_k}^i\Rightarrow\sigma^i,
\qquad
a\in\operatorname{supp}(\sigma^i)
\quad\text{for every }i\in I.
\]
Thus self-synchronization strengthens recurrence by requiring the limiting empirical distributions along the same subsequence to continue to represent the recurrent action. It excludes actions that are revisited only along exceptional dates while the samples used for learning converge to a different empirical regime. This also suggests a robustness interpretation: actions supported only by an asymptotically negligible set of dates may disappear under small perturbations of the realized history, whereas synchronized actions remain represented in the limiting empirical distribution. We leave a fuller exploration of this notion to future work. In finite action spaces, however, self-synchronization has an immediate frequency interpretation.

\begin{proposition}[Frequency interpretation]\label{prop:synchronization-frequency}
Suppose that $\mathbb A$ is finite and all players use the same selected sample. Then the largest self-synchronized set is
\[
\left\{
a\in\mathbb A:
\limsup_{t\to\infty}\hat\sigma_t(a)>0
\right\},
\]
where $\hat\sigma_t$ is the empirical distribution of the common selected sample. In particular, under full-history learning, this is the set of action profiles played with nonvanishing empirical frequency.
\end{proposition}

\begin{proof}
See the Appendix.

\begin{proof}
Let
\[
P:=\left\{a\in\mathbb A:\limsup_{t\to\infty}\hat\sigma_t(a)>0\right\}.
\]
We first show that $P$ is self-synchronized. Fix $a\in P$ and let
$\ell=\limsup_t\hat\sigma_t(a)>0$. Since $|H_t|\to\infty$, the change in
$\hat\sigma_t(a)$ generated by adding one selected observation converges to
zero. Moreover, the frequency of $a$ can increase only when an observation
with $a_t=a$ is selected. It follows that there are infinitely many selected
dates $t_k$ with $a_{t_k}=a$ such that
$\liminf_k\hat\sigma_{t_k}(a)>0$. Indeed, otherwise every sufficiently late
increase in the frequency of $a$ would start from a value bounded away from
$\ell$, and the vanishing size of a single update would contradict
$\limsup_t\hat\sigma_t(a)=\ell$.

Since $\Delta\mathbb A$ is compact, after passing to a subsequence we have
$\hat\sigma_{t_k}\to\sigma$ for some $\sigma\in\Delta\mathbb A$. Then
$\sigma(a)>0$, so $a\in\operatorname{supp}(\sigma)$. If
$b\in\operatorname{supp}(\sigma)$, then
$\limsup_t\hat\sigma_t(b)\geq\sigma(b)>0$, and hence $b\in P$. Thus
$a\in\operatorname{supp}(\sigma)\subseteq P$, so $P$ is self-synchronized.

Conversely, let $S$ be any self-synchronized set and fix $a\in S$. There
exist a subsequence $(t_k)_k$ and $\sigma\in\Delta S$ such that
$a_{t_k}\to a$, $\hat\sigma_{t_k}\to\sigma$, and
$a\in\operatorname{supp}(\sigma)$. Since $\mathbb A$ is finite,
$\sigma(a)>0$, and therefore
$\limsup_t\hat\sigma_t(a)\geq\sigma(a)>0$. Hence $a\in P$. Since $a\in S$
was arbitrary, $S\subseteq P$. Therefore $P$ is the largest
self-synchronized set. Under full-history learning, $\hat\sigma_t$ is the
usual empirical distribution of play, which gives the final claim.
\end{proof}
\end{proof}
 
Because self-synchronization focuses on a stronger notion of long-run persistence, we can correspondingly weaken the behavioral requirement. We say that behavior is \emph{synchronized asymptotically myopic} if, whenever for some player $i$ and some subsequence $(t_k)_k$,
\[
a_{t_k}\to a,
\qquad
\hat\sigma_{t_k}^i\Rightarrow\sigma^i,
\qquad
a\in\operatorname{supp}(\sigma^i),
\]
there exists $\varepsilon_k\downarrow0$ such that
$a_{t_k}^i\in F_{\varepsilon_k}^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})$
for all $k$. The asymptotically myopic behavior imposed in Section \ref{sec:foundations} clearly implies synchronized asymptotic myopia.

The forward-looking interpretation from the preceding subsection extends to this weaker requirement under correspondingly weaker identification. In particular, under the weak-identification condition of EP16, Appendix C, the same argument implies that forward-looking Bayesian behavior is synchronized asymptotically myopic: along a synchronized subsequence, best-fitting models agree on the consequence distribution generated by the limiting action, so dynamic optimality implies myopic optimality in the limit.

\begin{theorem}[Self-synchronized behavior is \(+\)-self-justified]
\label{theo:self-synchronized}
Consider a game with Bayesian players, selected samples, consistent forecasts, and synchronized asymptotically myopic behavior. With probability one, every self-synchronized set $S$ satisfies
$S\subseteq\Gamma^+(S)$. If the selected sample is common across players, then every self-synchronized set satisfies
$S\subseteq\Gamma^{CS+}(S)$.
\end{theorem}

\begin{proof}
See the Appendix.

Fix a realization in the $\mathbf P$-probability-one event on which Lemma \ref{lemm:Berk-selected} holds simultaneously for every player, and let $S$ be self-synchronized. Pick $a\in S$. By self-synchronization, there exists a subsequence $(t_k)_k$ and, for every player $i$, a distribution $\sigma^i\in\Delta S$ such that $a_{t_k}\to a$, $\hat\sigma_{t_k}^i\Rightarrow\sigma^i$, and $a\in\operatorname{supp}(\sigma^i)$. Passing to a further subsequence if necessary, let $\mu_{t_k}^i\Rightarrow\mu^i$ for every $i$. Lemma \ref{lemm:Berk-selected} then implies $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$.

By forecast consistency, $\tilde\sigma_{t_k}^{-i}\Rightarrow(\sigma^i)^{-i}$. Since $a\in\operatorname{supp}(\sigma^i)$, synchronized asymptotic myopia applies along this subsequence, so there exists $\varepsilon_k^i\downarrow0$ such that $a_{t_k}^i\in F_{\varepsilon_k^i}^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})$. The closed-graph property of $F_\varepsilon^i$ therefore yields $a^i\in F^i(\mu^i,(\sigma^i)^{-i})$.

Thus, for every player $i$, $\sigma^i\in\Delta S$, $a\in\operatorname{supp}(\sigma^i)$, $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$, and $a^i\in F^i(\mu^i,(\sigma^i)^{-i})$. Hence $a\in\Gamma^+(S)$. Since $a\in S$ was arbitrary, $S\subseteq\Gamma^+(S)$.

If the selected sample is common across players, the synchronizing subsequence has a common limiting distribution $\sigma\in\Delta S$, and the same argument gives $S\subseteq\Gamma^{CS+}(S)$.
\end{proof}

In particular, when $\mathbb A$ is finite, Proposition \ref{prop:synchronization-frequency} and Theorem \ref{theo:self-synchronized} imply the existence of a nonempty $+$-self-justified set; under a common sample they likewise imply the existence of a nonempty common-sample $+$-self-justified set. Hence the largest fixed points of $\Gamma^+$ and $\Gamma^{CS+}$ are nonempty in the finite-action case.

We illustrate the distinction between the original and refined concepts with the following example.

\begin{example}[Vanishing-frequency experimentation]
Consider a single-agent problem with action set $\mathbb A=\{a,b\}$ and consequence space $\mathbb Y=\{0,1\}$. The true consequence distribution satisfies $Q(1\mid a)=q$ and $Q(1\mid b)=q+d$, where $0<q<q+d<1$. The agent's misspecified model ignores the effect of the action and assumes $Q_\theta(1\mid a)=Q_\theta(1\mid b)=\theta$. Payoffs are $\pi(a,y)=0$ and $\pi(b,y)=q-y$.

Let $\sigma(b)=p$. The unique KL-minimizing parameter is $\theta(\sigma)=q+pd$. Hence the subjective expected payoff from $a$ is $0$, while that from $b$ is $-pd$.

Under the original operator $\Gamma$, both actions are rationalizable. Action $a$ is optimal for every $p\geq0$, while $b$ is optimal when $p=0$, since under $\sigma=\delta_a$ the agent is indifferent between $a$ and $b$. Thus the Berk--Nash rationalizable set is $\{a,b\}$.

The refinement eliminates $b$. To justify $b$ under $\Gamma^+$, the rationalizing distribution must satisfy $\sigma(b)>0$. But then $b$ yields strictly lower subjective expected payoff than $a$. Hence the $+$-rationalizable set is $\{a\}$.

The two concepts therefore distinguish two notions of long-run relevance. Under the original concept, both $a$ and $b$ can be sustained as actions played infinitely often. Under the refinement, the only $+$-self-justified set is $\{a\}$. With finite actions and full-history learning, Proposition \ref{prop:synchronization-frequency} implies that only $a$ can be played with nonvanishing frequency. Thus $b$ may still be played infinitely often, but its frequency must converge to zero, and the empirical distribution converges to $\delta_a$.
\end{example}

The refinement has bite here because $b$ is only weakly optimal under the distribution $\delta_a$. This illustrates a more general feature of the $+$ refinement. If an action is strictly optimal under a rationalizing distribution that excludes it from its support, then, under the usual continuity conditions, it remains optimal after modifying that distribution to place an arbitrarily small positive probability on the action. The action therefore also survives the $+$ refinement. Thus the additional bite of the support requirement comes primarily from actions whose justification is not locally robust. This logic applies in both finite and continuous action spaces.

\subsection{General formulation}

XXXX

General formulation? 

Let
\[
\Sigma(S)\subseteq(\Delta S)^I
\]
denote the set of admissible profiles of player-specific conjectures
\(\boldsymbol{\sigma}=(\sigma^i)_{i\in I}\). Each $\sigma^{i} \in \Delta S$ and $(\sigma^{i})^{-i} \in \Delta S^{-i}$ is the marginal over $S^{-i}$ of $\sigma^{i}$. Define
\begin{equation}
\Gamma_{\Sigma}(S)
:=
\bigcup_{\boldsymbol{\sigma}\in\Sigma(S)}
\prod_{i\in I}
\left[
\bigcup_{\mu^i\in\Delta\Theta^{m,i}(\sigma^i)}
F^i\bigl(\mu^i,(\sigma^i)^{-i}\bigr)
\right].
\label{eq:Gamma-Sigma}
\end{equation}
Equivalently,
\[
\Gamma_{\Sigma}(S)
=
\left\{
a\in\mathbb A:
\begin{array}{l}
\exists\,\boldsymbol{\sigma}\in\Sigma(S)
\text{ such that, for every }i\in I,\\[2pt]
\exists\,\mu^i\in\Delta\Theta^{m,i}(\sigma^i)
\text{ with }
a^i\in F^i\bigl(\mu^i,(\sigma^i)^{-i}\bigr)
\end{array}
\right\}.
\]

The union over \(\boldsymbol{\sigma}\) must appear outside the product over
players. Otherwise, a different profile
\(\boldsymbol{\sigma}\in\Sigma(S)\) could be selected for each player,
thereby eliminating the cross-player restrictions imposed by
\(\Sigma(S)\).

The unrestricted operator is obtained by setting $\Sigma(S)=(\Delta S)^I$, in which case $\Gamma_{\Sigma}(S)=\Gamma(S)$. 
By contrast, define the diagonal restriction
\[
\mathcal D(S)
:=
\left\{
\boldsymbol{\sigma}\in(\Delta S)^I:
\sigma^i=\sigma^j
\text{ for all }i,j\in I
\right\}.
\]
Setting $\Sigma(S)=\mathcal D(S)$ yields the common-support operator: $\Gamma_{\Sigma}(S)=\Gamma^{CS}(S)$. The operator $\Gamma^{CS_{+}}$ can be obtained similarly.

With this notation:

1. the order between operators is immediate.

2. There all operators are treated symmetrically.

\subsection{OLD. PUT IN OTHER. Self-Synchronized Behavior and Forward-Looking Learning}

We introduce a refinement that focuses on actions that persist together with the empirical distributions used to justify them. For a nonempty compact set \(S\subseteq\mathbb A\), define
\[
\Gamma^{+}(S)
=
\left\{
a\in\mathbb A:
\begin{array}{l}
\text{for every }i\in I\text{ there exist }\sigma^i\in\Delta S
\text{ and }\mu^i\in\Delta\Theta^{m,i}(\sigma^i)\\
\text{such that }
a\in\operatorname{supp}(\sigma^i)
\text{ and }
a^i\in F^i(\mu^i,(\sigma^i)^{-i})
\end{array}
\right\}.
\]
The common-sample refinement \(\Gamma^{CS+}\) is defined analogously by requiring a single \(\sigma\in\Delta S\), with \(a\in\operatorname{supp}(\sigma)\), to justify all players. We call \(S\) \(+\)-self-justified if \(S\subseteq\Gamma^{+}(S)\), and common-sample \(+\)-self-justified if \(S\subseteq\Gamma^{CS+}(S)\). 

Because $a\in\Gamma^+(S)$ requires $a\in\operatorname{supp}(\sigma^i)\subseteq S$ for every player, we always have $\Gamma^+(S)\subseteq S$. Hence $S$ is $+$-self-justified if and only if it is a fixed point of $\Gamma^+$. Since $\Gamma^+$ is monotone, the union of all fixed points is itself a fixed point and therefore is the largest fixed point. Unlike for $\Gamma$, however, the iterative characterization from $\mathbb A$ need not extend to infinite action spaces, because the condition $a\in\operatorname{supp}(\sigma)$ is not preserved under weak convergence. When $\mathbb A$ is finite, the decreasing sequence of iterates stabilizes after finitely many steps, so the iterative characterization again holds. Moreover, $\Gamma^+$ need not be nonempty-valued on nonempty sets, so its largest fixed point may be empty in general; below we show that it is nonempty in the finite-action common-sample case. The same observations apply to $\Gamma^{CS+}$.

We next provide a learning foundation for these refined self-justification concepts. The relevant long-run object strengthens the ordinary limit set by requiring current play to remain synchronized with the empirical distributions that support it. A nonempty compact set \(S\subseteq\mathbb A\) is \emph{self-synchronized} along a realized path if, for every \(a\in S\), there exists a subsequence \((t_k)_k\) and distributions \(\sigma^i\in\Delta S\), \(i\in I\), such that
\[
a_{t_k}\to a,
\qquad
\hat\sigma_{t_k}^i\Rightarrow\sigma^i,
\qquad
a\in\operatorname{supp}(\sigma^i)
\quad\text{for every }i\in I.
\]
Thus current play and the empirical distributions supporting it recur together. Self-synchronization excludes actions that are revisited only at exceptional dates while the samples used for learning converge toward a different empirical regime. In this sense, self-synchronized sets capture behavior that is both recurrent and empirically entrenched. Intuitively, self-synchronized actions are robust to perturbations that affect only an asymptotically negligible fraction of the realized history. Actions that occur only along exceptional dates may disappear when those dates are deleted, whereas an action synchronized with a limiting empirical distribution that assigns positive mass to each of its neighborhoods remains represented after such a perturbation.

We leave a fuller exploration of this notion to future work. We note, however, that in finite action spaces self-synchronization has a particularly simple interpretation.

\begin{proposition}[Frequency interpretation]\label{prop:synchronization-frequency}
Suppose that $\mathbb A$ is finite and all players use the same selected sample. Then the largest self-synchronized set is
\[
\left\{
a\in\mathbb A:
\limsup_{t\to\infty}\hat\sigma_t(a)>0
\right\},
\]
where $\hat\sigma_t$ is the empirical distribution of the common selected sample. In particular, under full-history learning, this is the set of action profiles played with nonvanishing empirical frequency.
\end{proposition}
\begin{proof} See the Appendix.
CHECK XXX Let
\[
P:=\left\{a\in\mathbb A:\limsup_{t\to\infty}\hat\sigma_t(a)>0\right\}.
\]
We first show that \(P\) is self-synchronized. Fix \(a\in P\), and let
\(\ell=\limsup_t\hat\sigma_t(a)>0\). Since the selected sample is persistent and
\(|H_t|\to\infty\), the change in \(\hat\sigma_t(a)\) generated by adding one
selected observation converges to zero. Moreover, \(\hat\sigma_t(a)\) can
increase only at a date \(t\) at which \(a_t=a\) and that observation is
selected. It follows that there is a sequence \(t_k\to\infty\) such that
\[
a_{t_k}=a
\qquad\text{and}\qquad
\liminf_{k\to\infty}\hat\sigma_{t_k}(a)>0.
\]
Since \(\Delta\mathbb A\) is compact, after passing to a subsequence,
\[
\hat\sigma_{t_k}\to\sigma
\]
for some \(\sigma\in\Delta\mathbb A\). Then \(\sigma(a)>0\), so
\(a\in\operatorname{supp}(\sigma)\). Moreover, if
\(b\in\operatorname{supp}(\sigma)\), then
\[
\limsup_{t\to\infty}\hat\sigma_t(b)\geq \sigma(b)>0,
\]
and hence \(b\in P\). Thus
\[
a\in\operatorname{supp}(\sigma)\subseteq P,
\]
so \(P\) is self-synchronized.

Conversely, let \(S\) be any self-synchronized set and \(a\in S\). By
self-synchronization, there is a subsequence \(t_k\) and a distribution
\(\sigma\) such that
\[
a_{t_k}\to a,\qquad
\hat\sigma_{t_k}\to\sigma,\qquad
a\in\operatorname{supp}(\sigma).
\]
Since \(\mathbb A\) is finite, \(a\in\operatorname{supp}(\sigma)\) implies
\(\sigma(a)>0\), and therefore
\[
\limsup_{t\to\infty}\hat\sigma_t(a)\geq\sigma(a)>0.
\]
Hence \(a\in P\), so \(S\subseteq P\). Therefore \(P\) is the largest
self-synchronized set. The full-history case is the special case in which
the common selected sample contains every observation.
\end{proof}

Because self-synchronization restricts attention to a stronger notion of long-run persistence, we can correspondingly weaken the behavioral requirement imposed above. We say that behavior is \emph{synchronized asymptotically myopic} if, whenever for some player $i$ and some subsequence $(t_k)_k$,
\[
a_{t_k}\to a,
\qquad
\hat\sigma_{t_k}^i\Rightarrow\sigma^i,
\qquad
a\in\operatorname{supp}(\sigma^i),
\]
there exists a sequence $\varepsilon_k\downarrow0$ such that
\[
a_{t_k}^i\in
F_{\varepsilon_k}^i
\bigl(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i}\bigr)
\]
for all $k$. The asymptotically myopic behavior imposed in Section \ref{sec:foundations} clearly implies synchronized asymptotic myopia, but the converse need not hold.

The weaker condition also accommodates forward-looking behavior. Following EP16, suppose player \(i\) evaluates actions according to the discounted Bayesian value function \(V^i\), defined recursively by the Bellman equation
\[
V^i(\mu^i,\beta^{-i})
=
\sup_{a^i\in\mathbb A^i}
\left\{
\int_{\Theta^i}U^i(a^i,\beta^{-i},\theta^i)\,\mu^i(d\theta^i)
+
\delta^i
\int V^i\!\left(B^i(\mu^i,a^i,y^i),\beta^{-i}\right)
\,\bar Q_{\mu^i}^i(dy^i\mid a^i,\beta^{-i})
\right\},
\]
where \(B^i(\mu^i,a^i,y^i)\) denotes the Bayesian posterior following consequence \(y^i\), and
\[
\bar Q_{\mu^i}^i(\cdot\mid a^i,\beta^{-i})
:=
\int_{\Theta^i}
\int_{\mathbb A^{-i}}
Q_{\theta^i}^i(\cdot\mid a^i,a^{-i})\,
\beta^{-i}(da^{-i})\,
\mu^i(d\theta^i)
\]
is the predictive distribution over consequences induced by belief $\mu^i$ and forecast $\beta^{-i}$. Let \(\Phi^i(\mu^i,\beta^{-i})\) denote the set of actions attaining the supremum. We say that player \(i\) is \emph{forward looking} if \(a_t^i\in\Phi^i(\mu_t^i,\tilde\sigma_t^{-i})\) at every date \(t\).

Following EP16, we say that the model is \emph{weakly identified} if, for every player $i$, every $\sigma\in\Delta\mathbb A$, every $\theta^i,\theta^{i\prime}\in\Theta^{m,i}(\sigma)$, and every $a\in\operatorname{supp}(\sigma)$, the reduced-form predictive distributions coincide:
\[
\bar Q_{\theta^i}^i(\cdot\mid a^i,\sigma^{-i})
=
\bar Q_{\theta^{i\prime}}^i(\cdot\mid a^i,\sigma^{-i}).
\]
Thus, best-fitting models may differ in their parameters, but they agree on the distribution of consequences induced by every own action that occurs in the support of the empirical distribution.

\begin{proposition} \label{prop:synchronized-optimality}
Under weak identification, if player $i$ is forward looking, then her behavior is synchronized asymptotically myopic, provided that payoffs are bounded and the value function and optimal-policy correspondence satisfy the usual continuity properties.
\end{proposition}
\begin{proof} See the Supplemental Appendix.

The proof uses the argument in Theorem 4 of Appendix C in EP16. Fix player $i$ and a subsequence $(t_k)_k$ such that
\[
a_{t_k}\to a,
\qquad
\hat\sigma_{t_k}^i\Rightarrow\sigma^i,
\qquad
a\in\operatorname{supp}(\sigma^i).
\]
Passing to a further subsequence if necessary, let
$\mu_{t_k}^i\Rightarrow\mu^i$. By Lemma \ref{lemm:Berk-selected},
$\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$, and forecast consistency implies
$\tilde\sigma_{t_k}^{-i}\Rightarrow(\sigma^i)^{-i}$. Since player $i$ is
forward looking, $a_{t_k}^i\in\Phi^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})$.
Continuity of the dynamic problem therefore implies
\[
a^i\in\Phi^i(\mu^i,(\sigma^i)^{-i}).
\]

By weak identification and $a\in\operatorname{supp}(\sigma^i)$, all
parameters in $\operatorname{supp}(\mu^i)$ induce the same reduced-form
predictive distribution under $a^i$. Hence Bayesian updating following
$a^i$ leaves $\mu^i$ unchanged, and the continuation value from choosing
$a^i$ is $\delta^i V^i(\mu^i,(\sigma^i)^{-i})$. For any alternative
$x^i$, the posterior is a martingale with mean $\mu^i$. Since the value
function is convex in beliefs, Jensen's inequality implies
\[
E\!\left[
V^i\!\left(B^i(\mu^i,x^i,Y^i),(\sigma^i)^{-i}\right)
\right]
\geq
V^i(\mu^i,(\sigma^i)^{-i}).
\]
Dynamic optimality of $a^i$ then implies that its current expected payoff
is at least that of every $x^i$, and therefore
\[
a^i\in F^i(\mu^i,(\sigma^i)^{-i}).
\]
By continuity of expected payoffs, the myopic payoff loss of
$a_{t_k}^i$ converges to zero. Hence there exists
$\varepsilon_k\downarrow0$ such that
\[
a_{t_k}^i\in
F_{\varepsilon_k}^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})
\]
for every $k$. Thus player $i$'s behavior is synchronized asymptotically
myopic.
\end{proof}

The proof uses the argument in Appendix C of EP16; we provide it here in the Supplemental Appendix. Along a synchronized subsequence, limiting posterior beliefs are supported on the best-fitting models for the limiting empirical distribution. Weak identification implies that these models agree on the consequences of the limiting action. Hence that action has no limiting informational advantage, and dynamic optimality implies myopic optimality along the subsequence.

In particular, under weak identification, forward-looking behavior does not enlarge the set of actions that can persist in a self-synchronized long-run regime. Proposition \ref{prop:synchronized-optimality} therefore allows the self-justification result below to apply directly to forward-looking Bayesian agents.

We now state the analogue of the learning-foundation result.

\begin{theorem}[Self-synchronized behavior is \(+\)-self-justified]
\label{theo:self-synchronized}
Consider a game with Bayesian players, selected samples, consistent forecasts, and synchronized asymptotically optimal behavior. With probability one, every self-synchronized set \(S\) satisfies $S\subseteq\Gamma^{+}(S)$. If the selected sample is common across players, then every self-synchronized set satisfies $S\subseteq\Gamma^{CS+}(S)$.
\end{theorem}

\begin{proof}
Fix a realization in the $\mathbf P$-probability-one event on which Lemma \ref{lemm:Berk-selected} holds simultaneously for every player, and let $S$ be self-synchronized. Pick $a\in S$. By self-synchronization, there exists a subsequence $(t_k)_k$ and, for every player $i$, a distribution $\sigma^i\in\Delta S$ such that $a_{t_k}\to a$, $\hat\sigma_{t_k}^i\Rightarrow\sigma^i$, and $a\in\operatorname{supp}(\sigma^i)$. Passing to a further subsequence if necessary, let $\mu_{t_k}^i\Rightarrow\mu^i$ for every $i$. Lemma \ref{lemm:Berk-selected} then implies $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$.

By forecast consistency, $\tilde\sigma_{t_k}^{-i}\Rightarrow(\sigma^i)^{-i}$. Since $a\in\operatorname{supp}(\sigma^i)$, synchronized asymptotic myopia applies along this subsequence, so there exists $\varepsilon_k^i\downarrow0$ such that $a_{t_k}^i\in F_{\varepsilon_k^i}^i(\mu_{t_k}^i,\tilde\sigma_{t_k}^{-i})$. The closed-graph property of $F_\varepsilon^i$ therefore yields $a^i\in F^i(\mu^i,(\sigma^i)^{-i})$.

Thus, for every player $i$, $\sigma^i\in\Delta S$, $a\in\operatorname{supp}(\sigma^i)$, $\mu^i\in\Delta\Theta^{m,i}(\sigma^i)$, and $a^i\in F^i(\mu^i,(\sigma^i)^{-i})$. Hence $a\in\Gamma^+(S)$. Since $a\in S$ was arbitrary, $S\subseteq\Gamma^+(S)$.

If the selected sample is common across players, the synchronizing subsequence has a common limiting distribution $\sigma\in\Delta S$, and the same argument gives $S\subseteq\Gamma^{CS+}(S)$.
\end{proof}

The proof differs from that of Theorem \ref{theo:limit-self-justified} in two respects. First, self-synchronization directly provides limiting sample distributions whose supports are contained in $S$. This is needed to use those distributions as witnesses in $\Gamma^+(S)$; stronger asymptotic myopia alone (or even perfect optimality) would not imply this support restriction. Second, self-synchronization requires $a\in\operatorname{supp}(\sigma^i)$. This is what permits us to apply synchronized asymptotic myopia along the subsequence approaching $a$. Without the first condition we could not conclude $a\in\Gamma^+(S)$, and without the second the weaker behavioral assumption would not apply.

\begin{corollary}[Existence in finite action spaces]
\label{cor:plus-existence}
Suppose that $\mathbb A$ is finite. Then there exists a nonempty
$+$-self-justified set and a nonempty common-sample $+$-self-justified set.
Consequently, the largest fixed points of $\Gamma^+$ and $\Gamma^{CS+}$
are nonempty.
\end{corollary}

\begin{proof}
Consider full-history learning. By Proposition
\ref{prop:synchronization-frequency}, the largest self-synchronized set is the
set of action profiles played with nonvanishing empirical frequency, and is
therefore nonempty. By Theorem \ref{theo:self-synchronized}, this set is both
$+$-self-justified and common-sample $+$-self-justified. Hence each operator
has a nonempty fixed point, so its largest fixed point is nonempty.
\end{proof}


We illustrate the distinction between the original and refined concepts with the following example.

\begin{example}[Vanishing-frequency experimentation]
Consider a single-agent problem with action set $\mathbb A=\{a,b\}$ and consequence space $\mathbb Y=\{0,1\}$. The true consequence distribution satisfies $Q(1\mid a)=q$ and $Q(1\mid b)=q+d$, where $0<q<q+d<1$. The agent's misspecified model ignores the effect of the action and assumes $Q_\theta(1\mid a)=Q_\theta(1\mid b)=\theta$. Payoffs are $\pi(a,y)=0$ and $\pi(b,y)=q-y$.

Let $\sigma(b)=p$. The unique KL-minimizing parameter is $\theta(\sigma)=q+pd$. Hence the subjective expected payoff from $a$ is $0$, while that from $b$ is $-pd$.

Under the original operator $\Gamma$, both actions are rationalizable. Action $a$ is optimal for every $p\geq0$, while $b$ is optimal when $p=0$, since under $\sigma=\delta_a$ the agent is indifferent between $a$ and $b$. Thus the Berk--Nash rationalizable set is $\{a,b\}$.

The refinement eliminates $b$. To justify $b$ under $\Gamma^+$, the rationalizing distribution must satisfy $\sigma(b)>0$. But then $b$ yields strictly lower subjective expected payoff than $a$. Hence the $+$-rationalizable set is $\{a\}$.

The two solution concepts therefore distinguish two notions of long-run relevance. Under the original concept, $\{a,b\}$ is self-justified, so both actions can be sustained as actions played infinitely often. Under the refinement, the only $+$-self-justified set is $\{a\}$. With finite actions and full-history learning, the actions played with nonvanishing frequency form a self-synchronized set and hence must be $+$-self-justified. It follows that $b$ must have vanishing frequency, while $a$ has frequency converging to one. Thus the empirical distribution converges to $\delta_a$, even though $b$ may continue to be played infinitely often.

\end{example}

The refinement has bite here because $b$ is only weakly optimal under the distribution $\delta_a$. This illustrates a more general feature of the $+$ refinement. If an action is strictly optimal under a rationalizing distribution that excludes it from its support, then, under the usual continuity conditions, it remains optimal after modifying that distribution to place an arbitrarily small positive probability on the action. The action therefore also survives the $+$ refinement. Thus the additional bite of the support requirement comes primarily from actions whose justification is not locally robust. This logic applies in both finite and continuous action spaces.


\subsection{Old material Proof of ``converse''}

\medskip
\noindent
\emph{XXX NEW DEMIAN XXX Step 4: Show that the target actions are asymptotically optimal along the target path.}

Let $\mathbf Q \in \Delta (\prod_{t}^{\infty} \mathbb Y_{t} )$ denote the probability law over infinite histories of outcomes generated by the outcome kernel $Q$ when the action rule is degenerate at the target path $z^\infty$ and the sampling array is the deterministic array constructed in Step 3. As shown in Step 3, this array satisfies
\[
\frac{|H_t^i|}{\log t}\to\infty
\]
for every player $i$, and, being deterministic ex ante, it also satisfies the sampling-timing requirement. Hence the target-path process is an admissible learning process. 


For each player $i$, let $\mu_t^{i,z}$, $\hat\sigma_t^{i,z}$, and $\tilde\sigma_t^{-i,z}$ denote player $i$'s posterior, selected empirical distribution, and forecast under this process. Also, define the payoff loss from playing the target action $z_t^i$ at date $t$ by
\[
\ell_t^i
:=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}
U^i(x^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i)
-
\int_{\Theta^i}
U^i(z_t^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i),
\]

Finally, let 
\[
\ell_t:=\max_{i\in I}\ell_t^i.
\]

Observe that for each player $i$, $\mu_t^{i,z}$, $\hat\sigma_t^{i,z}$, and $\tilde\sigma_t^{-i,z}$ are measurable with respect to $(y_{\tau})_{\tau \in H^{i}_{t}}$ (recall that the action and sampling paths are taken to be fixed). Thus, so is $\ell^{i}_{t}$. When needed, to make this dependence explicit, we will add $(y^{t})$ to these quantities.  
 
We claim that
\begin{align*}
    \mathbf Q \left( \lim_{t \to \infty} \ell_{t}(y^{t}) = 0  \right) = 1
\end{align*}


XXXX How do we know that the action sequence, sampling sequence, and outcome sequence are in $\Omega^{\ast}$... A version of Lemma for fixed actions/sampling should hold too; this issue (if an issue) is a presentational one XXX

XXX Rest of step 4 ok 

\medskip
\noindent
\emph{Step 5: Choose tolerances and define the actual process.}

Since
\[
\ell_t\to0
\qquad
\mathbf Q\text{-almost surely},
\]
Lemma~\ref{lem:deterministic-tolerance} implies that there exists a deterministic sequence $\varepsilon_t\downarrow0$ such that
\[
\mathbf Q
\left(
\ell_t\leq\varepsilon_t
\text{ for every }t
\right)
>
1-\alpha.
\]
Let
\[
G
:=
\left\{
\ell_t\leq\varepsilon_t
\text{ for every }t
\right\},
\]
so that
\[
\mathbf Q(G)>1-\alpha.
\]

We now define the action rule of the actual process. At date $t$, given the posterior $\mu_t^i$ and forecast $\tilde\sigma_t^{-i}$ induced by the deterministic sampling array constructed in Step 3, player $i$ chooses the target action $z_t^i$ whenever
\[
z_t^i
\in
F_{\varepsilon_t}^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right).
\]
Otherwise, she chooses an arbitrary exact best response in
\[
F^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right),
\]
which is nonempty by Lemma~\ref{lem:basic-properties}(ii), using any fixed measurable selection. Hence, at every history,
\[
a_t^i
\in
F_{\varepsilon_t}^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right),
\]
so the resulting action rule is asymptotically myopic.

Together with the full-support priors, the deterministic sampling array constructed in Step 3, Bayesian updating, and the empirical forecasts
\[
\tilde\sigma_t^{-i}
=
(\hat\sigma_t^i)^{-i},
\]
this action rule defines an admissible learning process with consistent forecasts.

For each $T\geq1$, let
\[
F_T
:=
\left\{
a_t=z_t
\text{ for every }t\leq T
\right\}
\]
and
\[
G_T
:=
\left\{
\ell_t\leq\varepsilon_t
\text{ for every }t\leq T
\right\}.
\]
We claim that, for every finite $T$, 
\begin{align}
    \mathbf Q (G_{T} ) = \mathbf P (F_{T}).
\end{align}

We prove this by induction. 

For \(T=1\), the posterior and forecast do not depend on any preceding
consequence. By construction of the action rule,
\[
a_1=z_1
\quad\Longleftrightarrow\quad
\ell_1^z\leq\varepsilon_1.
\]
and thus the rule prescribe that each players indeed plays $z^{i}_{1}$. Conditional
on \(a_1=z_1\), the distribution of \(y_1\) is \(Q(\cdot\mid z_1)\), which
is also its distribution under \(\mathbf Q \). Hence the desired result holds.


XXXXXXX

Now suppose that, for some \(T\geq2\),
\[
E_P\!\left[
\mathbf 1_{F_{T-1}}\psi(y^{T-1})
\right]
=
E_{P^z}\!\left[
\mathbf 1_{G_{T-1}}\psi(y^{T-1})
\right]
\]
for every bounded measurable function
\(\psi:Y^{T-1}\to\mathbb R\). On \(F_{T-1}\), the actual action history
through date \(T-1\) is \(z^{T-1}\). Because the sampling array is fixed,
the actual process and the target-path process therefore use the same
selected observations and have the same posterior and forecast at date
\(T\). Consequently, on \(F_{T-1}\),
\[
\mathbf 1\{a_T=z_T\}
=
\mathbf 1\!\left\{
\ell_T^z(y^{T-1})\leq\varepsilon_T
\right\}.
\]

Let \(\varphi:Y^T\to\mathbb R\) be bounded and measurable. Because the
date-\(T\) consequence is drawn after \(a_T\), and its conditional
distribution on \(\{a_T=z_T\}\) is \(Q(\cdot\mid z_T)\), it follows that
\begin{align*}
E_P\!\left[
\mathbf 1_{F_T}\varphi(y^T)
\right]
&=
E_P\!\left[
\mathbf 1_{F_{T-1}}
\mathbf 1\!\left\{
\ell_T^z(y^{T-1})\leq\varepsilon_T
\right\}
\int_Y
\varphi(y^{T-1},y_T)\,
Q(dy_T\mid z_T)
\right].
\end{align*}
Define
\[
\psi(y^{T-1})
:=
\mathbf 1\!\left\{
\ell_T^z(y^{T-1})\leq\varepsilon_T
\right\}
\int_Y
\varphi(y^{T-1},y_T)\,
Q(dy_T\mid z_T).
\]
Applying the induction hypothesis to this function gives
\begin{align*}
E_P\!\left[
\mathbf 1_{F_T}\varphi(y^T)
\right]
&=
E_{P^z}\!\left[
\mathbf 1_{G_{T-1}}
\mathbf 1\!\left\{
\ell_T^z(y^{T-1})\leq\varepsilon_T
\right\}
\int_Y
\varphi(y^{T-1},y_T)\,
Q(dy_T\mid z_T)
\right] \\
&=
E_{P^z}\!\left[
\mathbf 1_{G_T}\varphi(y^T)
\right],
\end{align*}
where the second equality uses the fact that, under \(P^z\), the
conditional distribution of \(y_T\) given \(y^{T-1}\) is
\(Q(\cdot\mid z_T)\). This completes the induction.

Taking \(\varphi\equiv1\), we conclude that, for every \(T\geq1\),
\[
P(F_T)=P^z(G_T).
\]


XXXX OLD STEP 4 and STEP 5 XXX

\medskip
\noindent
\emph{Step 4: Show that the target actions are asymptotically optimal along the target path.}

Let $\mathbf P^z$ denote the probability law generated when the action rule is degenerate at the target path $z^\infty$ and the sampling array is the deterministic array constructed in Step 3. As shown in Step 3, this array satisfies
\[
\frac{|H_t^i|}{\log t}\to\infty
\]
for every player $i$, and, being deterministic ex ante, it also satisfies the sampling-timing requirement. Hence the target-path process is an admissible learning process. Let $\mu_t^{i,z}$, $\hat\sigma_t^{i,z}$, and $\tilde\sigma_t^{-i,z}$ denote player $i$'s posterior, selected empirical distribution, and forecast under this process.

For each player $i$, define the payoff loss from playing the target action $z_t^i$ at date $t$ by
\[
\ell_t^i
:=
\sup_{x^i\in\mathbb A^i}
\int_{\Theta^i}
U^i(x^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i)
-
\int_{\Theta^i}
U^i(z_t^i,\tilde\sigma_t^{-i,z},\theta^i)\,
\mu_t^{i,z}(d\theta^i),
\]
and let
\[
\ell_t:=\max_{i\in I}\ell_t^i.
\]
We claim that
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely}.
\]

Let $\Omega^\ast$ be the probability-one event on which Lemma~\ref{lemm:Berk-selected} holds simultaneously for every player under the target-path process. Suppose, toward a contradiction, that $\ell_t\not\to0$ on a set of positive $\mathbf P^z$-probability. Since the player set is finite, there exist a player $i$, a number $\eta>0$, and an event $A\subseteq\Omega^\ast$ with $\mathbf P^z(A)>0$ such that
\[
\limsup_{t\to\infty}\ell_t^i(\omega)>\eta
\qquad
\text{for every }\omega\in A.
\]

Fix $\omega\in A$. Then there exists a subsequence $(t_m)_m$ such that
\[
\ell_{t_m}^i(\omega)\geq\eta
\qquad
\text{for every }m.
\]
By compactness, passing to a further subsequence if necessary, we may assume
\[
z_{t_m}\to a\in S,
\]
\[
\rho_{t_m}^i\Rightarrow\rho^i\in\Delta S,
\]
and
\[
\mu_{t_m}^{i,z}(\omega)\Rightarrow\mu^i.
\]

By Step 3,
\[
d_\Delta
\left(
\hat\sigma_{t_m}^{i,z},
\rho_{t_m}^i
\right)
\to0.
\]
Together with
\[
\rho_{t_m}^i\Rightarrow\rho^i,
\]
this implies
\[
\hat\sigma_{t_m}^{i,z}
\Rightarrow
\rho^i.
\]
Since
\[
\tilde\sigma_t^{-i,z}
=
(\hat\sigma_t^{i,z})^{-i},
\]
we also have
\[
\tilde\sigma_{t_m}^{-i,z}
\Rightarrow
(\rho^i)^{-i}.
\]

Because $\omega\in\Omega^\ast$, Lemma~\ref{lemm:Berk-selected} applies to the subsequence $(t_m)_m$. Hence
\[
\mu^i
\in
\Delta\Theta^{m,i}(\rho^i).
\]
By identification,
\[
\Theta^{m,i}(\rho^i)
=
\{\theta^i(\rho^i)\},
\]
so necessarily
\[
\mu^i
=
\delta_{\theta^i(\rho^i)}.
\]

On the other hand, by the choice of the supporting distributions in Step 2,
\[
z_{t_m}^i
\in
F^i
\left(
\delta_{\theta^i(\rho_{t_m}^i)},
(\rho_{t_m}^i)^{-i}
\right)
\qquad
\text{for every }m.
\]
Identification and Lemma~\ref{lem:basic-properties}(iv) imply that the map
\[
\rho\mapsto\theta^i(\rho)
\]
is continuous. Hence
\[
\delta_{\theta^i(\rho_{t_m}^i)}
\Rightarrow
\delta_{\theta^i(\rho^i)}.
\]
Together with
\[
z_{t_m}^i\to a^i
\]
and
\[
(\rho_{t_m}^i)^{-i}
\Rightarrow
(\rho^i)^{-i},
\]
the closed-graph property of $F^i$ implies
\[
a^i
\in
F^i
\left(
\delta_{\theta^i(\rho^i)},
(\rho^i)^{-i}
\right).
\]

By continuity of the value function and expected payoffs, the payoff loss from $z_{t_m}^i$ under
\[
\left(
\mu_{t_m}^{i,z},
\tilde\sigma_{t_m}^{-i,z}
\right)
\]
converges to the payoff loss from $a^i$ under
\[
\left(
\delta_{\theta^i(\rho^i)},
(\rho^i)^{-i}
\right).
\]
The latter loss is zero because
\[
a^i
\in
F^i
\left(
\delta_{\theta^i(\rho^i)},
(\rho^i)^{-i}
\right).
\]
Therefore
\[
\ell_{t_m}^i(\omega)\to0,
\]
contradicting
\[
\ell_{t_m}^i(\omega)\geq\eta
\qquad
\text{for every }m.
\]
Hence
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely}.
\]

\medskip
\noindent
\emph{Step 5: Choose tolerances and define the actual process.}

Since
\[
\ell_t\to0
\qquad
\mathbf P^z\text{-almost surely},
\]
Lemma~\ref{lem:deterministic-tolerance} implies that there exists a deterministic sequence $\varepsilon_t\downarrow0$ such that
\[
\mathbf P^z
\left(
\ell_t\leq\varepsilon_t
\text{ for every }t
\right)
>
1-\alpha.
\]
Let
\[
G
:=
\left\{
\ell_t\leq\varepsilon_t
\text{ for every }t
\right\},
\]
so that
\[
\mathbf P^z(G)>1-\alpha.
\]

We now define the action rule of the actual process. At date $t$, given the posterior $\mu_t^i$ and forecast $\tilde\sigma_t^{-i}$ induced by the deterministic sampling array constructed in Step 3, player $i$ chooses the target action $z_t^i$ whenever
\[
z_t^i
\in
F_{\varepsilon_t}^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right).
\]
Otherwise, she chooses an arbitrary exact best response in
\[
F^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right),
\]
which is nonempty by Lemma~\ref{lem:basic-properties}(ii), using any fixed measurable selection. Hence, at every history,
\[
a_t^i
\in
F_{\varepsilon_t}^i
\left(
\mu_t^i,
\tilde\sigma_t^{-i}
\right),
\]
so the resulting action rule is asymptotically myopic.

Together with the full-support priors, the deterministic sampling array constructed in Step 3, Bayesian updating, and the empirical forecasts
\[
\tilde\sigma_t^{-i}
=
(\hat\sigma_t^i)^{-i},
\]
this action rule defines an admissible learning process with consistent forecasts.

For each $T\geq1$, let
\[
F_T
:=
\left\{
a_t=z_t
\text{ for every }t\leq T
\right\}
\]
and
\[
G_T
:=
\left\{
\ell_t\leq\varepsilon_t
\text{ for every }t\leq T
\right\}.
\]
We claim that, for every finite $T$, whenever the realized consequence history belongs to $G_T$, the actual process follows the target path through date $T$.

The claim follows by induction. At date $1$, the actual and target histories are both empty, so the posterior and forecast coincide with those used to compute $\ell_1$. Since $G_T$ implies
\[
\ell_1\leq\varepsilon_1,
\]
the target action $z_1^i$ is $\varepsilon_1$-optimal for every player $i$, and therefore the action rule prescribes $z_1$.

Now suppose that
\[
a_s=z_s
\qquad
\text{for every }s<t,
\]
where $t\leq T$. Because the sampling array $W$ is deterministic ex ante, the actual process and the target-path process use exactly the same selected dates at date $t$. Since the realized action history also coincides with the target history through date $t-1$, the selected observations, posterior beliefs, and forecasts coincide with those used to compute $\ell_t$. Since $G_T$ implies
\[
\ell_t\leq\varepsilon_t,
\]
the target action $z_t^i$ is $\varepsilon_t$-optimal for every player $i$. Hence the action rule prescribes $z_t$, completing the induction.

It remains to compare probabilities under the actual process and the target-path process. Up to any date at which the actual action path coincides with the target path, both processes use the same deterministic sampling array and the same consequence kernel
\[
Q(\cdot\mid z_t).
\]
Therefore, for every finite $T$,
\[
\mathbf P(F_T)
\geq
\mathbf P^z(G_T).
\]

The events $(F_T)_T$ are decreasing, with
\[
\bigcap_{T=1}^{\infty}F_T
=
\left\{
a_t=z_t
\text{ for every }t
\right\},
\]
and $(G_T)_T$ decreases to $G$. Hence, by continuity of probability from above,
\[
\mathbf P
\left(
\bigcap_{T=1}^{\infty}F_T
\right)
=
\lim_{T\to\infty}
\mathbf P(F_T)
\geq
\lim_{T\to\infty}
\mathbf P^z(G_T)
=
\mathbf P^z(G)
>
1-\alpha.
\]

On the event
\[
\bigcap_{T=1}^{\infty}F_T,
\]
the realized action path coincides with the target path $z^\infty$. Therefore,
\[
L(a^\infty)
=
L(z^\infty)
=
S.
\]
Hence
\[
\mathbf P
\bigl(
L(a^\infty)=S
\bigr)
>
1-\alpha.
\]
\end{proof}

\end{proof}



\section{Deterministic tolerance lemma not using Egorov}

\begin{lemma}[Deterministic tolerance]\label{lem:deterministic-tolerance}
Let \((\ell_t)_{t\geq1}\) be a sequence of nonnegative random variables on a probability space \((\Omega,\mathcal F,P)\). Suppose that \(\ell_t\to0\), \(P\)-almost surely, and that \(\sup_t \ell_t\leq M\) for some finite constant \(M\). Then, for every \(\alpha>0\), there exists a deterministic sequence \(\varepsilon_t\downarrow0\) such that
\[
P\left(\ell_t\leq\varepsilon_t\text{ for every }t\right)>1-\alpha.
\]
\end{lemma}
\begin{proof}
Let \(C:=\max\{M,1\}\). For each \(T\), let \(R_T:=\sup_{t\geq T}\ell_t\). Since \(\ell_t\to0\) almost surely, \(R_T\to0\) almost surely as \(T\to\infty\). Hence, for each \(k\geq1\), we can choose \(N_k\) increasing such that \(P(R_{N_k}>C/k)<\alpha 2^{-k}\).

Define
\[
\varepsilon_t
:=
\begin{cases}
C, & t<N_1,\\
C/k, & N_k\leq t<N_{k+1}.
\end{cases}
\]
Then \(\varepsilon_t\downarrow0\).

For each \(k\), let \(E_k:=\{R_{N_k}>C/k\}\). By construction, \(P(E_k)<\alpha2^{-k}\), so the union bound implies
\[
P\left(\bigcup_{k=1}^\infty E_k\right)
\leq
\sum_{k=1}^\infty P(E_k)
<
\alpha.
\]
Thus, with probability greater than \(1-\alpha\), none of the events \(E_k\) occurs. On this event, \(R_{N_k}\leq C/k\) for every \(k\).

It remains to check that \(\ell_t\leq\varepsilon_t\) for every \(t\). If \(t<N_1\), then \(\ell_t\leq M\leq C=\varepsilon_t\). If \(N_k\leq t<N_{k+1}\), then \(t\geq N_k\), so \(\ell_t\leq R_{N_k}\leq C/k=\varepsilon_t\). Therefore \(P(\ell_t\leq\varepsilon_t\text{ for every }t)>1-\alpha\).
\end{proof}


